To Err is Machine: Vulnerability Detection Challenges LLM Reasoning

In this paper, we present a challenging code reasoning task: vulnerability detection. Large Language Models (LLMs) have shown promising results in natural-language and math reasoning, but state-of-the-art (SOTA) models reported only 54.5% Balanced Accuracy in our vulnerability detection evaluation, even those models pre-trained on large amounts of source code. Our error analysis on LLM responses shows that the models struggle to reason about the code semantics relevant to identifying vulnerabilities, especially subtle semantic differences caused by small textual changes. We explored prominent models and training settings to understand their effects on vulnerability detection performance -- including better prompts, larger models, more pre-training data, and fine-tuning -- but none led to significant improvements. This raises the question of whether simply scaling training data and model size will allow us to "solve" complex code reasoning tasks like vulnerability detection, or if a fundamental shift in modeling and training techniques is required. We also explored adding domain knowledge to prompts; although it helped certain models understand some code semantics, vulnerability detection requires multi-step reasoning, and these models still failed in steps, such as reasoning about variable relations. Our results suggest that new models, new training methods, or more execution-specific pretraining data may be needed to conquer vulnerability detection. We speculate that auto-regressive pre-training on source code may not effectively extract code semantics, especially on the current pretraining mixtures, in which execution data is scarce. Success on vulnerability detection as a code reasoning task can benefit many areas of software engineering such as debugging, test input generation, and program repair. Our code and data are available at https://doi.org/10.6084/m9.figshare.27368025.

==> ErrorExamples/hmr-hallucination.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Hallucination}.} \label{fig:hallucination-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 30/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
static int __get_data_block(struct inode *inode, sector_t iblock, struct buffer_head *bh, int create, int flag, pgoff_t *next_pgofs)
{
  struct f2fs_map_blocks map;
  int err;
  map.m_lblk = iblock;
  map.m_len = bh->b_size >> inode->i_blkbits;
  map.m_next_pgofs = next_pgofs;
  err = f2fs_map_blocks(inode, &map, create, flag);
  if (!err) {
    map_bh(bh, inode->i_sb, map.m_pblk);
    bh->b_state = (bh->b_state & ~F2FS_MAP_FLAGS) | map.m_flags;
    bh->b_size = (u64)map.m_len << inode->i_blkbits;
  }
  return err;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
    % Sure! The function \texttt{\_\_get\_data\_block} takes a \texttt{sector\_t} parameter \texttt{iblock} and uses it to calculate the block number for the input \texttt{inode} and \texttt{bh} using the formula \texttt{iblock * (inode->i\_blkbits / 512)}
    
    \ldots
    \hl{if \texttt{iblock} is set to this maximum value, the calculation \texttt{iblock * (inode->i\_blkbits / 512)} will result in a large integer overflow}, causing the calculation to wrap around to a small value.
    \end{tcolorbox}
\end{figure}

==> ErrorExamples/hmr-repetition.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Repetition} (code not shown).} \label{fig:repetition-example}
%     \begin{tcolorbox}[title=\textbf{Source code} (Example 49/vulnerable),colframe=Periwinkle]
%     \begin{minted}
%     [
%     frame=lines,
%     numbersep=2mm,
%     breaklines=true,
%     fontsize=\footnotesize,
%     highlightlines={},
%     highlightcolor=yellow,
%     linenos,
%     tabsize=2,
%     ]
%     {c}
% void * CAPSTONE_API cs_winkernel_malloc(size_t size)
% {
%   // Disallow zero length allocation because they waste pool header space and,
%   // in many cases, indicate a potential validation issue in the calling code.
%   NT_ASSERT(size);

%   // FP; a use of NonPagedPool is required for Windows 7 support
% #pragma prefast(suppress : 30030)		// Allocating executable POOL_TYPE memory
%   CS_WINKERNEL_MEMBLOCK *block = (CS_WINKERNEL_MEMBLOCK *)ExAllocatePoolWithTag(
%     NonPagedPool, size + sizeof(CS_WINKERNEL_MEMBLOCK), CS_WINKERNEL_POOL_TAG);
%   if (!block) {
%     return NULL;
%   }
%   block->size = size;

%   return block->data;
% }
%     \end{minted}
%     \end{tcolorbox}
    \begin{tcolorbox}[title={\textbf{Model response} (StarCoder, Example 49/vulnerable)}]
1. The function is buggy because it is not checking for a null pointer.

2. The function is buggy because it is not checking for a null pointer.

\ldots

10. The function is buggy because it is not checking for a null pointer.
    \end{tcolorbox}
\end{figure}

==> ErrorExamples/logical-contradiction.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Logical Contradiction}.} \label{fig:contradiction-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 38/vulnerable),colframe=Periwinkle]
% int ecall_restore(const char *input, uint64_t input_len, char **output,
%                   uint64_t *output_len) {
%   if (!asylo::primitives::TrustedPrimitives::IsOutsideEnclave(input,
%                                                               input_len) ||
%       !asylo::primitives::TrustedPrimitives::IsOutsideEnclave(
%           output_len, sizeof(uint64_t))) {
%     asylo::primitives::TrustedPrimitives::BestEffortAbort(
%         "ecall_restore: input/output found to not be in untrusted memory.");
%   }
%   int result = 0;
%   size_t tmp_output_len;
%   try {
%     result = asylo::Restore(input, static_cast<size_t>(input_len), output,
%                             &tmp_output_len);
%   } catch (...) {
%     LOG(FATAL) << "Uncaught exception in enclave";
%   }

%   if (output_len) {
%     *output_len = static_cast<uint64_t>(tmp_output_len);
%   }
%   return result;
% }
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    breakanywhere=true,
    % breakanywheresymbolpre=\tiny\ensuremath{\hookleftarrow},
    % breakanywheresymbolpre=-,
    breakanywheresymbolpre={},
    fontsize=\footnotesize,
    highlightlines={3,9},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
int ecall_restore(const char *input, uint64_t input_len, char **output, uint64_t *output_len) {
  if (!IsOutsideEnclave(input, input_len) ||
      !IsOutsideEnclave(output_len, sizeof(uint64_t)))
    BestEffortAbort("ecall_restore: input/output found to not be in untrusted memory.");
  // ...
  result = Restore(input, static_cast<size_t>(input_len), output, &tmp_output_len);
  // ...
  if (output_len)
    *output_len = static_cast<uint64_t>(tmp_output_len);
  return result;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (Code LLAMA)]
    \ldots
    % 
    \hl{The function then checks if the \texttt{output\_len} pointer is located in untrusted memory}, and if it is not, it aborts the execution.

    \ldots
    % 
    The function is vulnerable to CWE-787: Out-of-bound Write because \hl{the \texttt{output\_len} pointer is not checked to ensure that it is located in untrusted memory} before it is used to store the restored enclave state.
    This could allow an attacker to write to the \texttt{output\_len} pointer, which could lead to a buffer overflow or other security vulnerabilities.
    \end{tcolorbox}
\end{figure}

==> ErrorExamples/logical-implication.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Faulty Logical Implication}.} \label{fig:logical-implication-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 11/non-vulnerable),colframe=Periwinkle]
% int avpriv_ac3_parse_header(AC3HeaderInfo **phdr, const uint8_t *buf,
%                             size_t size)
% {
%   GetBitContext gb;
%   AC3HeaderInfo *hdr;
%   int err;

%   if (!*phdr)
%     *phdr = av_mallocz(sizeof(AC3HeaderInfo));
%   if (!*phdr)
%     return AVERROR(ENOMEM);
%   hdr = *phdr;

%   err = init_get_bits8(&gb, buf, size);
%   if (err < 0)
%     return AVERROR_INVALIDDATA;
%   err = ff_ac3_parse_header(&gb, hdr);
%   if (err < 0)
%     return AVERROR_INVALIDDATA;

%   return get_bits_count(&gb);
% }
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={3,6},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
int avpriv_ac3_parse_header(AC3HeaderInfo **phdr, const uint8_t *buf, size_t size) {
  // ...
  err = init_get_bits8(&gb, buf, size);
  if (err < 0)
    return AVERROR_INVALIDDATA;
  err = ff_ac3_parse_header(&gb, hdr);
  if (err < 0)
    return AVERROR_INVALIDDATA;
  return get_bits_count(&gb);
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
    \ldots{}if the input \texttt{buf} is null, then \hl{the \texttt{init\_get\_bits8} call will return a negative value, and the \texttt{ff\_ac3\_parse\_header} call will attempt to access the null pointer \texttt{hdr}}, which will result in a null pointer dereference.
    
    Therefore, the function is vulnerable to a null pointer dereference if the input \texttt{buf} is null.
    \end{tcolorbox}
\end{figure}

==> ErrorExamples/understanding-control-flow.tex <==
\begin{figure}[htbp]
    \centering
    % \benjamin{Could be macro, not as typical as the other example. Make sure we know what list\_for\_each\_entry\_safe does. Have some discussion why the error might happen.}
    \caption{Example of \textbf{Incorrect Control-flow}.} \label{fig:control-flow-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 17/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={12,14},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
static void regulator_ena_gpio_free(struct regulator_dev *rdev)
{
	struct regulator_enable_gpio *pin, *n;
	if (!rdev->ena_pin) return;
	/* Free the GPIO only in case of no use */
	list_for_each_entry_safe(pin, n, &regulator_ena_gpio_list, list) {
		if (pin->gpiod == rdev->ena_pin->gpiod) {
			if (pin->request_count <= 1) {
				pin->request_count = 0;
				gpiod_put(pin->gpiod);
				list_del(&pin->list);
				kfree(pin);
				rdev->ena_pin = NULL;
				return;
			} else {
				pin->request_count--;
			}
		}
	}
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (StarChat-$\beta$)]
    The function \hl{dereferences \texttt{`rdev->ena\_pin`} after freeing it}, which is a use after free. This can lead to memory corruption or other unexpected behavior.
    \end{tcolorbox}
\end{figure}

==> ErrorExamples/understanding-integer-math.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of Incorrect Understanding of \textit{Integer Math}.} \label{fig:integer-math-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 5/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={4},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
long WebPImage::getHeaderOffset(byte* data, long data_size, byte* header, long header_size) {
  if (data_size < header_size) { return -1; }
  long pos = -1;
  for (long i=0; i < data_size - header_size; i++) {
    if (memcmp(header, &data[i], header_size) == 0) {
      pos = i;
      break;
    }
  }
  return pos;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
The issue is that the comparison loop can cause an integer overflow if the \texttt{data\_size} is large and the \texttt{header\_size} is small\ldots
% This can happen because the loop iterates \texttt{data\_size}-\texttt{header\_size} times, which can result in a large number of iterations if \texttt{data\_size} is large.

For example, \hl{if \texttt{data\_size} is 1000 and \texttt{header\_size} is 10, the loop will iterate 900 times (1000 - 10). This can cause an integer overflow} if the loop counter is not properly initialized or if it is not properly checked for overflow.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.FSE25/abstract.tex <==
\begin{abstract}
Vulnerability detection is of crucial importance to maintaining the security, integrity, and trustworthiness of software systems.
Large Language Models (LLMs) have demonstrated great potential for software engineering tasks such as code generation and program repair, making them a promising approach for vulnerability detection.
Precise vulnerability detection requires reasoning about the code, making it a good case study for exploring the limits of LLMs' reasoning capabilities.
Although recent work has applied LLMs to vulnerability detection using generic prompting techniques, their full capabilities for this task and the types of factual and reasoning errors they make remain unclear.

In this paper, we surveyed eleven LLMs that are state-of-the-art in code generation and commonly used as coding assistants, and evaluated their capabilities for vulnerability detection.
We systematically searched for the best-performing prompts, incorporating techniques such as in-context learning and retrieval-augmented generation.
Our results show that while baseline prompting methods improved the models' performance, LLMs generally struggled with vulnerability detection. They reported performance close to a random-guess baseline and failed to distinguish between buggy and fixed versions of programs in the majority of cases.
Through an in-depth analysis of hundreds of model reasoning instances, we found that more than half of LLM responses contained errors in key areas like code understanding, hallucination, and logical reasoning. For example, the models frequently missed bounds and NULL-pointer checks, referred to code that didn't exist, or made faulty or inconsistent logical inferences. They also often misjudged the locations of buggy code and misidentified bug types, reducing the accuracy and value of their explanations.
These findings suggest that despite their potential for other tasks, LLMs may fail to properly comprehend critical code structures and security-related concepts.
Based on our error analysis, we propose four novel prompting methods based on incorporating bug semantics into LLM prompts, leveraging information from bug-fixing changes, CVE bug reports, and static analysis tools.
Our results show that bug semantic-based prompting is a promising approach for improving vulnerability detection performance, and highlight the need for further research to improve the vulnerability detection, factual, and reasoning capabilities of LLMs.
Our data and code are available at \url{https://figshare.com/s/78fe02e56e09ec49300b}.
\end{abstract}


==> _OldVersion.FSE25/content.tex <==
\section{Introduction}

Large Language Models (LLMs) have demonstrated impressive capabilities across various software engineering tasks, such as code generation~\cite{humaneval}, test generation~\cite{lemieux_testgen}, and code summarization~\cite{ahmed2024automatic}. Their versatile capabilities, along with their novel ability to explain their predictions in plain-text, make LLMs worthwhile subjects of investigation for detecting security vulnerabilities.
In static analysis and human inspection, vulnerability detection requires code understanding and reasoning. Pattern-matching on code structures is insufficient to produce precise analyses~\cite{flawfinder,rats}, especially for real-world code. For example, to precisely detect a buffer overflow, we cannot only scan for {\tt strcpy} or {\tt malloc} statements. We need to identify the statements that update the strings and buffers, reason about the lengths of the strings after the changes at these statements, and also understand the bounds-check code to judge whether the protection is sufficient. 

LLMs have shown limited ability for complex reasoning~\cite{hooda_large_2024}, and a recent survey calls for more challenging tasks to evaluate their reasoning abilities~\cite{reasoning_survey}; this calls into question whether LLMs possess the capabilities to perform effective vulnerability detection. This capability has profound implications for the potential applications of LLMs in other tasks which require understanding and reasoning about semantics of code, e.g., fault localization, program repairs, debugging and code generation for non-trival tasks.  Studying LLMs for vulnerability detection also shed lights for the industry practitioners on whether LLMs can be considered as their software assurance tools. 

Several studies have shown that LLMs struggle to attain high performance on vulnerability detection~\cite{fu2023chatgpt,ullah2023large,nong2024chainofthought,zhang2023prompt}.
LLMs generally underperformed with basic prompts~\cite{fu2023chatgpt}, which motivated the use of in-context examples~\cite{ullah2023large}, chain-of-thoughts~\cite{nong2024chainofthought} and static analysis~\cite{zhang2023prompt}.
Prior studies primarily evaluate vulnerability detection performance. The very recent work (to the best of our knowledge, these papers are still in arXiv but not yet published) highlight broad errors in the models' vulnerability detection responses~\cite{yu2024security,nong2024chainofthought,sun2024llm4vuln,ullah2023large}, but do not comprehensively investigate the LLM errors from the perspective of detecting vulnerabilities.

Our studies, which are concurrently developed with these works, aim for (1) {\it comprehensiveness} --- we surveyed a wider variety of models and prompts in different scenarios of vulnerability detection, and analyzed more LLM responses with multiple raters, compared to prior work; and
(2) {\it usefulness} --- beyond evaluating ``Yes/No'' predictions, we studied whether LLMs can correctly report the types, locations and causes of a vulnerability, as done in industry-standard static analysis-based detectors~\cite{fbinfer,codeql,sonarqube}, and point out capabilities and code structures which LLMs struggled with, highlighting future research directions.
In that regard, we also compared the capabilities of LLMs with human performance for understanding vulnerabilities.
Specifically, we designed the following four questions to guide our research:

\begin{itemize}
    % \item \textbf{RQ1:} What are the most successful and least successful prompt designs for LLM-based vulnerability detection?
    % \item \textbf{RQ2:} How well do state-of-the-art LLMs perform on vulnerability detection?
    % \item \textbf{RQ3:} What kinds of errors do LLMs make when explaining the vulnerabilities?
    % \item \textbf{RQ4:} How do LLMs compare to human developers for localizing vulnerabilities?
    \item \textbf{RQ1:} How well do state-of-the-art LLMs and prompts perform on vulnerability detection?
    \item \textbf{RQ2:} Why do LLMs underperform on vulnerability detection? What kinds of errors do LLMs make when detecting vulnerabilities?
    \item \textbf{RQ3:} How can we improve LLMs for vulnerability detection?
    \wei{bug semantics and self-consistency check can all be added here}
    \ben{Expands scope, only include if we have time --- \textbf{RQ4:} Can integrating self-consistency help LLMs perform better for vulnerability detection?}
\end{itemize}

To thoroughly investigate these RQs, we evaluated 11 SOTA LLMs using five distinct prompt templates, including developing three novel techniques for generating prompts. We systematically searched among the prompts to draw out the best performance from each model (\Cref{sec:rq1}). We investigated their empirical performance and their capability to distinguish buggy code from the corresponding fixed versions (\Cref{sec:rq2}).
% 
We rigorously analyzed 287 LLM responses explaining their vulnerability predictions and categorized them into 4 comprehensive error categories specifically tailored for vulnerability detection, revealing the ways in which the LLMs frequently failed and which code structures the models struggled with, as well as the effects of such errors on the models' explanation quality (\Cref{sec:rq3}).
% 
We evaluated the models' fault localization abilities on DbgBench, comparing their performance and difficulties with those of professional human software engineers to understand their similarities and differences (\Cref{sec:dbgbench}).

Our results show the following:
most models performed best with Basic and In-Context prompting. Our proposed CoT-SA and Contrastive Pairs, used with In-Context prompting, were beneficial for some models. 
LLMs performed within 0.5-0.63 Balanced Accuracy, close to a random-guess baseline, and failed to distinguish buggy and fixed versions of code in 76\% of cases on average.
57\% of LLM responses contained errors in {\it Code Understanding}, {\it Hallucination}, {\it Logic}, and/or {\it Commonsense Knowledge}, and among others, LLMs especially struggled with correctly identifying bounds/null checks. Furthermore, LLMs frequently predicted erroneous location, type, or root cause of vulnerabilities, in spite of the correct binary label.
LLMs correctly located 6/27 bugs in DbgBench~\cite{dbgbench}, all of which were correctly diagnosed by at least one human. GPT-3 performed the best among all the models and correctly located 4/27 bugs.

In summary, we make the following contributions:
\wei{draft the contribution, need to fine tune it 
\begin{itemize}
    \item We did a comprehensive study on prompting LLMs for vulnerability detection, to the best of our knowledge, our study integrates the most recent models (12 models), used most clean dataset (1028 datapoints), and tested various scenarios of vulnerability detection (including test them on pair/unpair data.
    \item We analyzed 287 LLM responses to break down the errors which LLMs made, and provide insights and a dataset for future research on vulnerability detection using LLMs.    
    \item Based on our study results, we designed new prompt methods and significantly improve the performance of LLMs on vulnerability detection. It provides insights on how we should integrate LLMs for the challenge tasks of vulnerability detection.
\end{itemize}
}

\mycomment{
\begin{itemize}
    \item We designed 3 new prompt templates for vulnerability detection, integrating information from bug-fixing patches, CVE descriptions, and static analyzers.
    \item We comprehensively evaluated the vulnerability detection capabilities of state-of-the-art LLMs, including testing them on pairs of buggy/fixed code.
    \item We analyzed 287 LLM responses to break down the errors which LLMs made, and provide insights and a dataset for future research on vulnerability detection using LLMs.
   \item We evaluated LLMs' debugging abilities in comparison with humans on the DbgBench vulnerability benchmark.
\end{itemize}
}

\section{How well do state-of-the-art LLMs and prompts perform on vulnerability detection?}
We designed a comprehensive study to evaluate how existing LLMs perform on this task. Compared to previous studies~\cite{XXX}, our work integrates the newest model, used the cleanest datasets (\wei{please copy over the rebuttal content}. We present our study setup in Section~\cite{setup} and we report our results in Section~\ref{results}.

\subsection{Study Setup}~\label{setup}
\subsubsection{Dataset}
\label{sec:dataset}
% \ben{Make more straightforward and concise, remove stuff about cost and portion of dataset.}
We evaluated the models' vulnerability detection capabilities mainly using the SVEN dataset released by \citet{sven}. This dataset was collected from CVE records reporting real-world vulnerabilities from the CrossVul~\cite{crossvul}, BigVul~\cite{bigvul}, and VUDENC~\cite{vudenc} datasets and has 93\% accurate labels~\cite{primevul}, making it suitable for our detailed evaluation.
% 
SVEN is made of the source code of functions that were changed in vulnerability-fixing commits, where the version of the code before the commit is considered vulnerable and the version after the commit is considered non-vulnerable.
The authors curated the dataset by manually inspecting the commits based on their domain expertise to ensure that the data includes true security vulnerabilities/fixes and excludes data quality issues, including spurious commit message matches, tangled commits, and project-specific APIs.
Leveraging these labels, we focus on the \textit{binary classification} setting: given a prompt containing a function's source code, models predict whether the function belongs in the positive (vulnerable) or negative (non-vulnerable) class.


% The entire SVEN dataset comprises 846 C/C++ functions. We used 100 functions (50 pairs of a vulnerable function and its corresponding fixed version) to perform the study. This is because (1) many real-world functions are very long and do not fit the context window of the LLMs under study; (2) running LLM queries is very costly. It takes an average of 2 GPU-minutes per query, totaling 3.4 GPU-hours for 100 functions for each prompt method per model, and about \$180 of OpenAI credits in total. We studied a total of 11 models and for each model, we used 5 prompt methods (\S \Cref{}).
% In addition, the models’ responses tended to vary when sampled multiple times. To address this variance, we ran the model inference 3 times with different random seeds and report the aggregated results.

We also used the Big-Vul~\cite{bigvul} and D2A~\cite{d2a} datasets to source in-context examples and extra metadata to generate our prompts (see \Cref{sec:prompt-design}).
% We used DbgBench~\cite{dbgbench} to compare the performances of LLMs and human for vulnerability detection (see  \Cref{sec:dbgbench}).


\subsubsection{Models}

\begin{table}[htbp]
\centering
\caption{11 models we studied, HumanEval $Pass@1$ is reported by \citet{paperswithcode-humaneval} or the source papers.}
\label{tab:humaneval}
\begin{tabular}{lrrrrr}
\toprule
Model   & Parameters & Context Length & \makecell[r]{Code completion\\score (HumanEval)}              \\
\midrule
GPT-4~\citet{gpt4}       & - & 128k & 86.6 \\
Gemini 1.0 Pro~\citet{gemini} & - & 32k & 67.7 \\
WizardCoder~\citet{wizardcoder} & 15B & 2k                   & 57.3                 \\
Code LLAMA~\citet{codellama}  & 34B & 16k$\sim$100k                   & 48.8                    \\
GPT-3.5~\citet{gpt3.5}     & - & 4k & 48.1 \\
Mixtral-MoE~\citet{mixtral} & 45B & 8k$\sim$128k & 40.2 \\
Mistral~\citet{mistral} & 7B & 8k$\sim$128k & 30.5 \\
StarCoder~\citet{starcoder} & 15B & 8k & 30.4 \\
LLAMA 2~\citet{llama2} & 70B & 4k & 29.9 \\
StarChat-$\beta$~\citet{starchat} & 15B & 8k & - \\
MagiCoder~\citet{magicoder} & 7B & 16k$\sim$100k & - \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{Text generation parameters we used.}
    \label{tab:parameters}
    \begin{tabular}{lccc}
    \toprule
        Parameter & HuggingFace & OpenAI & Google \\
    \midrule
        Top-$p$ & 0.9 & 1.0 & 1.0 \\
        Temperature & 0.1 & 0.1 & 0.1 \\
        Max. tokens generated & 512 & 512 & 512 \\
    \bottomrule
    \end{tabular}
\end{table}

% \ben{Make more simple and concise}
We collected a list of large language models from two benchmark surveys~{\cite{zhao_survey_2023, liuAgentBenchEvaluatingLLMs2023}} as well as the highest-performing models from \citet{paperswithcode-humaneval}. We added several notable open-source models (e.g. StarCoder~\cite{starcoder}) and excluded the models for which inference was not available via API (e.g. Bard~\cite{bard}), not trained on source code (e.g. Pythia~\cite{pythia}), were trained only on distillations from ChatGPT (e.g. Vicuna~\cite{vicuna}), or were superseded by later iterations on the same project (e.g. LlaMA 1~\cite{llama1}).
In \Cref{tab:humaneval}, we list the \textcolor{red}{11} models used in our study, including the number of parameters (if it is an open source model), the length of the {\it context window}, i.e., the maximum number of input tokens, and HumanEval $Pass@1$ score~\cite{humaneval}, a metric that can somewhat reflect the models' capabilities in generating source code.

\subsubsection{Implementation of Automatic Evaluation}
% \ben{Make more concise, describing just the most important settings and parser.}
To evaluate many models on a large dataset, we wrote scripts to automatically query the models and parse the model output. For the open-source models, we used HuggingFace~\cite{huggingface_generation} and ollama~\cite{ollama} local text generation APIs. For GPT-3.5, GPT-4, and Gemini, we used the APIs hosted by the corresponding organizations~\cite{openai,googleai}.
\Cref{tab:parameters} shows the text generation parameters we used for the models.
We selected parameter values intended to make their responses more deterministic, without sampling greedily (which can substantially reduce the performance).
To address variance caused by the non-deterministic sampling process, we ran the model inference 3 times with different random seeds and report the aggregated results.

% StarCoder is the base model of StarChat-$\beta$.
% For model survey Table
% \url{https://huggingface.co/blog/starcoder}
% \footnotetext[1]{StarCoder is the base model of StarChat-$\beta$ ~\cite{starchat}.}
% \footnotetext[2]{We used the next-largest 13B version of LLAMA 2 because we lacked the resources to run the 70B version.}
% % \footnotetext[2]{We used the next-largest 13B version of LLAMA 2 because we lacked the resources to run the 70B version.}
% % % For inference parameter table
% \footnotetext[3]{
% % \url{https://github.com/facebookresearch/codellama/blob/main/example\_completion.py\#L15}
% Code LLAMA's example scripts set \texttt{top\_p} to 0.9~\cite{codellama-temperature}. }
% \footnotetext[4]{OpenAI recommends to alter either temperature or 
% % \url{https://platform.openai.com/docs/api-reference/chat/create}
% \texttt{top\_p}, but not both, for their models~\cite{openai-temperature}.}
% \footnotetext[4]{OpenAI recommends to alter either temperature or \texttt{top\_p}, but not both, for their models. \url{https://platform.openai.com/docs/api-reference/chat/create}}
We wrote a custom framework to assemble the prompts (including in-context example selection and embedding retrieval) and parse the responses.
The models generally replied with plain-text sentences. We developed a regular expression-based method to extract categorical vulnerable/non-vulnerable responses; in cases where the models had no categorical response, we considered the prediction incorrect.
In order to ensure the correctness of our extraction method, we selected 10\% of the responses for manual observation and found that our extraction procedure had an error rate of less than 0.5\%.
For future reuse, we open-source our code and document further implementation details in our data package~\cite{data-package-figshare}.


\subsubsection{Metrics for Evaluation}
\label{sec:metrics}

We evaluated the models using the following four metrics: \textit{Accuracy}, the proportion of correct predictions on all examples, \textit{Precision}, the proportion of correct predictions out of the examples on which the model predicted vulnerable, \textit{Recall}, the proportion of correct predictions out of the examples which are labeled vulnerable, and \textit{Balanced Accuracy}, the mean of per-class accuracy for both vulnerable and non-vulnerable classes.

    \begin{equation*}     
        \text{BalancedAccuracy} = \frac{ \frac{correct_{negative}}{examples_{negative}} + \frac{correct_{positive}}{examples_{positive}} }{2}
    \end{equation*}
    
We observed that LLMs often produced predictions that are highly imbalanced, such as labeling every example as vulnerable (see \Cref{sec:rq2}), and that conventional metrics such as F1 and MCC tend to favor these severely-imbalanced classifiers (see our data package for details~\cite{data-package-figshare}).
We argue that an imbalanced classifier that pathologically predicts only one class is less desirable than one that demonstrates some ability to differentiate between classes. In order to reflect this, {we primarily used Balanced Accuracy~\cite{brodersen_balanced_2010} to compare model performance}.

%\section{Study Designs and Results of RQs}

%\subsection{RQ1: How well do state-of-the-art LLMs and prompting techniques perform on vulnerability detection?}
%\label{sec:rq1}

\subsubsection{Prompting Methods Studied}\label{sec:prompt-design}

We evaluated several existing prompting methods~\cite{fu2023chatgpt,liuGptandIncontext2023,zhou2024large} as baselines, which can be grouped into {\it Basic (zero-shot)} and {\it In-context ($n$-shot)} prompts~\cite{liu_pre-train_2021}.
We also designed three new prompting methods, namely \textit{In-context prompting based on contrastive pair}, \textit{Chain-of-Thought from CVE descriptions}, and {\it Chain-of-Thought from static analysis}.
There are many ways to phrase a given prompt, which can strongly influence performance~\cite{state_of_what_art}. To remove confounding variables between different prompt designs, we implemented the prompts using consistent phrasing which consistently produced valid results for most models, and cited the prior work which applied each method prominently.
% \ben{There are lots of ways to phrase the prompts, so we roughly used the simplest phrasing that worked best out of the ones we tried, and match up with the method proposed by related works.}
% \ben{Make the case that these prompting methods are prominently used and fundamental in the sense that more advanced methods will build on top of them, so our error analysis on them can generalize its implications.}
% \ben{Although many prompting methods exist which differ in slight details~\cite{liu_pre-train_2021}, we focused on evaluating the prominently used prompting techniques, which are foundational to more advanced techniques.}
% \ben{These prompting methods are foundational to more advanced prompting techniques, so we believe that our results will generalize.}

\noindent\textbf{Basic (zero-shot) prompting}~\cite{fu2023chatgpt}: 
We used a system prompt to set the context: \prompt{I want you to act as a vulnerability detection system}, and we explored a variety of natural language descriptions:
(a) \underline{Basic query}: \prompt{Is the following function buggy? Please answer Yes or No.}\footnote{We also tried \prompt{Is the following function vulnerable?}; however, our pilot study shows that it did not perform as well.}
(b) \underline{CWE list}: This prompt starts with \prompt{Does the following function contain one of the following bug types?}, followed by a fixed list of bug types, e.g., \prompt{CWE-190: Integer Overflow};
(c) \underline{Q/A}: Begin the query with \prompt{Question:} and begin the model's response with \prompt{Answer:}. This conditions the model to respond in a question-answering mode~\cite{gpt3}.

\noindent\textbf{In-context ($n$-shot) prompting}~\cite{liuGptandIncontext2023,zhou2024large}:
Before the basic prompt, we provide examples of inputs and responses for in-context (IC) learning which condition the model to reply in the same format as the example responses~\cite{gpt3,stanford_incontext}.
We selected the in-context examples from other data points in the SVEN dataset, excluding the corresponding bug-fix pair to prevent data leakage.
The selection of in-context examples can heavily impact the performance~\cite{incontext_number}, so we studied three popularly-used settings:
(a) \underline{IC-Random}~\cite{zhou2024large}: randomly selected examples;
(b) \underline{IC-Retrieval}~\cite{zhou2024large}: examples similar to the query example, measured by cosine similarity between their embeddings generated by a neural network\footnote{We tried several embedding models in a pilot study~\cite{reimers2019sentencebert,openai_embeddings,codebert} as well as sparse retrieval methods such as BM25~\cite{bm25} and TF-IDF~\cite{tfidf} and reported CodeBERT~\cite{codebert} as the best-performing model.}; and
% \footnote{We tried several embedding models~\cite{reimers2019sentencebert,openai_embeddings,codebert} and sparse retrieval metrics~\cite{tfidf,bm25} and report the best-performing methods: CodeBERT~\cite{codebert} and BM25~\cite{bm25}.}
% (c) \underline{IC-BM25}~\cite{liuGptandIncontext2023}: examples that were similar to the query example as measured by BM25~\cite{bm25}; and
(c) \underline{IC-Contrastive}: examples from {\it contrastive pairs} (see below for details).

\noindent\textbf{In-context prompting with contrastive pairs}: 
We leveraged \textit{contrasting pairs} by providing the vulnerable version of the code (before the bug-fixing commit) and the fixed version (after the commit) as in-context examples in the same prompt.
Since these two versions of the source code differ primarily in the portion related to the bug-fix, we intend for this prompt template to highlight the cause of the bug and instruct the model that small differences in code can introduce or mitigate vulnerabilities.
\ben{We should draw up the pair analysis table for contrastive and non-contrastive in-context prompts to see if contrastive prompts helped the model differentiate buggy from fixed examples.}

\ben{TODO: Search comprehensively for related works in this area.}
\ben{TODO: Integrate all the new wacky methods, like CFG-based, incontext with second-guess, etc. Include as appropriate.}

% \begin{figure}[htbp]
%     \centering
% \begin{minipage}{0.35\textwidth}
% \begin{mdframed}
% \small{\texttt{The crypto\_skcipher\_init\_tfm function in crypto/skcipher.c in the Linux kernel through 4.11.2 relies on a setkey function that lacks a key-size check, which allows local users to cause a denial of service (NULL pointer dereference) via a crafted application.}}
% \end{mdframed}
% \end{minipage}
% \quad% 
% \begin{minipage}{0.6\textwidth}
% \begin{mdframed}
% \small{\texttt{%
% 1. A buffer buf of size 10 is {allocated} at line 1.\\
% 2. An index i is {initialized to a value} in the range [0, 100] at line 2.\\
% 3. The index {i is used to access buf} at line 3. 
% {This may exceed the bounds of buf.}\\
% }}
% \end{mdframed}
% \end{minipage}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

\noindent\textbf{Chain-of-thoughts from CVE descriptions} (\underline{CoT-CVE}):
We designed chain-of-thought (CoT) prompts~\cite{cot} by incorporating intermediate reasoning steps that lead to the answer. We drew in-context examples from the Big-Vul dataset~\cite{bigvul}, which includes links to the CVE bug reports. For vulnerable examples, we adapted the bug report descriptions into in-context responses explaining the vulnerability.
% For non-vulnerable examples (which lack descriptions in CVE reports), we provided the default query and response.
% https://nvd.nist.gov/vuln/detail/CVE-2013-6051
For example, the prompt below is based on CVE-2017-9211~\cite{CVE-2017-9211}, detailing the vulnerability, including symptoms, attack surface, and related variables.
\ben{Tie it to the error analysis: did these CoT prompts make fewer factual errors or explain the bug better?}

\begin{promptblock}
\small{\texttt{The crypto\_skcipher\_init\_tfm function in crypto/skcipher.c in the Linux kernel through 4.11.2 relies on a setkey function that lacks a key-size check, which allows local users to cause a denial of service (NULL pointer dereference) via a crafted application. Therefore, the example is buggy.}}
\end{promptblock}

\noindent\textbf{Chain-of-thoughts from static analysis} (\underline{CoT-SA}):
We used created CoT prompts using \textit{buggy paths} reported by static analysis tool --- lists of statements that lead to a bug.
We drew in-context examples from the D2A dataset~\cite{d2a}, which lists buggy paths identified by the Infer static analyzer~\cite{fbinfer} for various open-source C++ projects.
For vulnerable examples, we converted the buggy paths into natural language descriptions and used them as responses.
% For non-vulnerable examples, we provided the default response.
The example below is a prompt based on a buffer overflow detected by Infer.
\ben{Tie it to the error analysis: did these CoT prompts make fewer factual errors or explain the bug better?}

\begin{promptblock}
\small{\texttt{%
1. A buffer buf of size 10 is {allocated} at line 1.\\
2. An index i is {initialized to a value} in the range [0, 100] at line 2.\\
3. The index {i is used to access buf} at line 3. 
{This may exceed the bounds of buf.}\\
4. Therefore, the example is buggy.
}}
\end{promptblock}

% Considering the numerous ways the above prompting techniques can be combined, we systematically searched for high-performing prompts for each model.
% For the basic prompting method, we evaluated four ``modes'' ---
% (1) basic query, (2) Q/A, (3) CWE list, and (4) both Q/A and CWE list --- and designated the best-performing mode as the \textbf{Basic} prompting approach.

% For the in-context prompting methods, we evaluated random selection \textbf{(IC-Random)}, embedding similarity search \textbf{(IC-Embedding)}, chain-of-thought from CVE descriptions \textbf{(CoT-CVE)}, and chain-of-thought from static analysis \textbf{(CoT-SA)}.
% For each approach, we used two configurations: (1) 6 randomly-selected examples as well as (2) 3 contrastive pairs. We then selected the best outcome for each model and prompting method.
In a pilot study (\S~\ref{sec:discussion}), we found that 6 in-context examples performed best across most models and was the maximum number that fit within their context sizes. Therefore, we used 6-shot prompts, evaluating both (a) 6 selected examples in a non-contrastive setting and (b) 3 selected contrastive pairs. Examples and implementation details of the prompts are provided in our data package~\cite{data-package-figshare}.
% \ben{Move most implementation details of the prompts and evaluations into here, like random seeds.}
% \ben{Before running all the models, let's do some more rigorous/reportable trials of the variables we tried: buggy/vulnerable, number of shots, and retrieval method.}
\ben{Let's add some comparison of the model size with the prediction and reasoning quality, if it's interesting.}

\subsection{Results}
\label{sec:rq1}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{Images/performance_paired_mean.png}
        \caption{Paired data}
        \label{fig:best-prompts}
    \end{subfigure}

    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{Images/performance_unpaired_mean.png}
        \caption{Unpaired data}
        \label{fig:best-prompts-unpaired}
    \end{subfigure}
    
    \caption{Performance of various prompting methods on the SVEN dataset. Bar height shows the Balanced Accuracy averaged over three random seeds, with error bars indicating one standard deviation, and stars show the best-performing prompt for each model.}
\end{figure}

\Cref{fig:best-prompts} shows the performance of baseline prompting methods on all models, compared to a hypothetical random-guess baseline.
Our results show that the Embedding retrieval performed the best overall, eliciting the best performance from 4 models. \ben{Why?}

\ben{Contrastive vs. non-contrastive}

\ben{CoT-SA and CoT-CVE}

\ben{Best model overall}

We evaluated the models on a dataset containing pairs of vulnerable and fixed programs.
This represents a use-case such as using LLMs to detect vulnerabilities, and then checking again for the vulnerability after applying a bug-fixing patch.
While this aspect is shared with other benchmarks based on bug reports, like Big-Vul~\cite{bigvul} and CVEFixes~\cite{cvefixes}, it may not represent all vulnerability detection settings.
To represent an alternative scenario of scanning new procedures for vulnerabilities, we also plotted results on a random sample of 50\% vulnerable and 50\% non-vulnerable functions from SVEN that were unrelated in terms of bug fixes and show the results in \Cref{fig:best-prompts-unpaired} (bottom).
\ben{Talk about results.}

% Pair table

\begin{table}[t]
    \centering
    \caption{Further analysis on 50 pairs of vulnerable and non-vulnerable examples. Cell values display the number and percentage of pairs in each category
    % \benjamin{TODO: Replace GPT-3.5 line.}
    }
    \label{tab:pair-performance}
    \begin{tabular}{lrrr}
    \toprule
        Model & Can't Distinguish & Both Correct & Both Wrong \\
       \midrule
        StarChat-Beta & 24 (48\%) & 18 (36\%) & 8 (16\%) \\
        GPT-4 & 36 (72\%) & 9 (18\%) & 5  (10\%)\\
        StarCoder & 35 (70\%) & 10 (20\%) & 5 (10\%) \\
        Mixtral-MoE & 36 (72\%) & 10 (20\%) & 4 \myspace(8\%) \\
        MagiCoder & 42 (84\%) & 6 (12\%) & 2 \myspace(4\%) \\
        GPT-3.5 & 40 (80\%) & 7 (14\%) & 3 \myspace(6\%) \\
        LLAMA 2 & 41 (82\%) & 6 (12\%) & 3 \myspace(6\%) \\
        WizardCoder & 21 (42\%) & 17 (34\%) & 12 (24\%) \\
        Code LLAMA & 44 (88\%) & 5 (10\%) & 1 \myspace(2\%) \\
        Mistral & 47 (94\%) & 3 \myspace(6\%) & 0 \myspace(0\%) \\
        Gemini & 49 (98\%) & 1 \myspace(2\%) & 0 \myspace(0\%)\\
        \midrule
        Average & 38 (76\%) & 8 (16\%) & 4 \myspace(8\%) \\
        \bottomrule
    \end{tabular}
\end{table}

\Cref{tab:pair-performance} presents a further analysis on the models' capabilities of distinguishing pairs of vulnerable and nonvulnerable code. In the table, under Column {\it Can't Distinguish}, we show that on average, 76\% of pairs cannot be distinguished. Under {\it Both Correct} and {\it Both Wrong} columns, our results indicate that the models can predict both versions correctly in some instances (16\% of pairs), but there are also cases (8\% of pairs) where the models can predict both versions incorrectly.

\begin{summarybox}
\textbf{Summary:}
The SOTA LLMs performed poorly at vulnerability detection, with Balanced Accuracy ranging from 0.5 to 0.63.
All models frequently failed to distinguish the buggy and fixed versions of programs --- in 76\% of cases on average.
\end{summarybox}

\begin{summarybox}
\textbf{Summary (merge with the above)}
Across two vulnerability detection settings,
Basic or IC-Random prompts performed the best for 7-8 models.
Integrating Q/A and CWE-list were useful for improving model performance.
IC-Embedding and CoT-SA performed best for 3-4 models. Contrastive Pairs were useful for predicting unpaired data.
\end{summarybox}


\section{Why do existing LLMs underperform on vulnerability detection?}
\label{sec:rq3}

We have performed an error analysis to understand why LLMs fail. Compared to existing studies~\cite{}, our approach \wei{show how we different} 

\ben{Include analysis on a sampling of new data, including data which uses chains of thought to reason about bugs.}

\subsection{Study Setup} 

For a vulnerability detection tool to be useful, we hope it can present further vulnerability information such as its cause, types and locations. We prompted the LLMs to explain all predictions that they identified as vulnerable and analyzed their responses.
The prompt consists of three parts:
(1) the original prompt described in \Cref{sec:rq1}, applying the best-case prompt for each model noted in \Cref{fig:model-performance},
(2) the model's original prediction, e.g., ``Yes/No'' for basic prompts or ``Yes, the vulnerability is \textit{CWE-XXX: Description}'' for prompts with CWE information, and
(3) ``Please explain the reasoning for this answer''. We manually inspected the results and found that the models generally make four types of errors:


\begin{figure}[htbp]
    \centering
    \small{Does the response contain an error?\\
    \begin{tabular}{ll}
    \mbox{\cblock{58}{146}{58} No} &
    \mbox{\cblock{192}{61}{62} Yes}
    \end{tabular}}

    \includegraphics[width=0.5\linewidth]{Images/error-analysis_categories.pdf}
    \caption{Error categories observed in responses from all LLMs.
    Bar width shows the number of errors observed in each category. Bar labels show the percentage of responses containing each category of error. Responses can contain more than one error.}
    \label{fig:error-categories}
\end{figure}


\begin{table}[htbp]
\centering
    \centering
    \caption{Fine-grained errors across 287 responses to 100 programs.
    For select \textit{Code understanding} errors related to specific code structures, the total number of responses containing those structures and the percentage with an error are shown.
    }
    \label{tab:fine-grained}
\begin{tabular}{llr}
\toprule
Error category & Error & Count \\
\midrule
\multirow[t]{10}{*}{Code understanding} & Bounds/NULL check & 76/159 (48\%) \\
 & String operation & 3/29 (10\%) \\
 & Integer math & 8/96 \myspace(8\%) \\
 & Pointer operation & 9/147 \myspace(6\%) \\
 & Alloc/Free operation & 4/81 \myspace(5\%) \\
 & Index operation & 1/60 \myspace(2\%) \\
 & Control flow & 11 \\
 & Syntax & 5 \\
 & Data type & 1 \\
 \cmidrule{2-3}
 & Total & 118 \\
 \midrule
\multirow[t]{4}{*}{Hal/Mem/Rep} & Hallucination & 15 \\
 & Memorization & 11 \\
 & Repetition & 5 \\
 \cmidrule{2-3}
 & Total & 31 \\
 \midrule
\multirow[t]{3}{*}{Logic error} & Implication & 14 \\
 & Inconsistent & 13 \\
 \cmidrule{2-3}
 & Total & 27 \\
 \midrule
Common knowledge & Total & 8 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{\textit{Code understanding errors}} LLMs produce incorrect assertions about programming language semantics or code structures, including inferences about the effects of statements.
For instance, sometimes an LLM incorrectly claims that a pointer is accessed without being checked, when the code contains the check; sometimes an LLM claims an integer operation will overflow when, considering the size of the integer and possible values of the operation implied by the prior code context, an overflow is impossible.
\paragraph{\textit{Common knowledge errors}} LLMs make incorrect assumptions about the applications, environment, or code conventions.
For example, an LLM may claim that if a variable \texttt{N\_FDC} is negative, an error will occur. However, a developer could reasonably interpret the all-capitalized \texttt{N\_FDC} as a configuration variable representing the number of a certain resource (floppy-disk controllers), and assume it to be a non-negative integer by definition.
\paragraph{\textit{Logic errors}} LLMs produce statements that are logically contradictory or make incorrect logical implications when reaching the conclusions of vulnerability.
For example, sometimes an LLM correctly claims that a variable \texttt{x} is checked, then later contradicts itself by stating, ``since \texttt{x} \textit{is not checked}, it will overflow...''.
\paragraph{\textit{Hallucination/Memorization/Repetition errors}} LLMs produce {\it hallucination} (stating information that sounds correct but is not present in the prompt, such as pointing out a potential integer overflow in an arithmetic operation that doesn't appear in the code), {\it memorization} (memorizing information from the training data),
and {\it repetition} (infinitely repeating  certain text sequences, for instance: ``1. The function is buggy because it is not checking for a null pointer. 2. The function is buggy because it is not checking for a null pointer. 3\ldots'').


We collected quantitative data by analyzing  a total of 287 eligible LLM responses to understand how often LLMs make such mistakes.
To mitigate subjectivity, we used independent ratings from three authors, similar to \citet{empiricalstudy-deeplearningbugs}.
The raters independently identified the errors in the LLM responses, meeting to refine the protocol after processing \sfrac{1}{3}, \sfrac{1}{2}, and all of the data.
We measured inter-rater agreement using \textit{Fleiss' kappa ($\kappa$)~\cite{fleiss}}, ranging from -1 to 1 with higher values indicating more agreement.
We resolved disagreements by siding with the majority when two raters differed from the third, resulting in $\kappa=0.75$ with 83\% of responses classified identically. We then discussed the remaining disagreements until reaching a final categorization for each response.


\input{ErrorExamples/understanding-missing-check}

\input{ErrorExamples/understanding-integer-math-2}


\subsection{Results}
\Cref{fig:error-categories} reports how often each type of error occurred in LLM responses. We found that LLMs were somewhat useful for explaining vulnerabilities as 43\% responses contain no errors. Improving Code Understanding will help LLMs to better explain vulnerabilities, as 41\% responses contained code understanding errors. Our results also demonstrate that LLMs still cannot perfectly solve reasoning problems, as some of the incorrect code understanding is due to not being able to
reason about the values across several statements, and there are 9\% Logic errors and 3\% Common Knowledge errors, which can affect the reasoning. We  observed that LLMs tended towards Hallucination, Memorization, and Repetition (11\% of errors) during vulnerability detection.


In \Cref{tab:fine-grained}, we show the specific code structures that affected the correctness of the explanations as well as the fine-grained classifications for Logic errors and Hallucination/Memorization/Repetition errors. For example, out of 159 responses explaining bounds checks, 76 are incorrect. \Cref{fig:bounds-check-example} shows an example of a model response which flags an unchecked null-pointer dereference, presumably at line 5 (\texttt{p->lineinfo[oldpc]}), even though \texttt{p->lineinfo} is checked at line 2.
This error can lead to false positives, especially after the bug is fixed by adding a check.

\Cref{fig:integer-math-example} shows an example of an \textit{integer math} error.  From the model response,  the LLM correctly identified that there is a bounds-check at line~6 (it was in fact added by the developers to prevent overflows~\cite{CVE-2018-16435}). Given the upper bound of \texttt{0x7fff} for \texttt{nSamples+1} and \texttt{nPatches+1}, even the maximum values would not cause an overflow in an unsigned integer ($\texttt{0x7fff} * \texttt{0x7fff} * \texttt{8} = \texttt{0xfff80008}$) at line~9; however, the LLM was not able to understand and reason about such math.


\begin{figure}[t]
    \centering
    \small{
    \begin{tabular}{ll}
    \mbox{\cblock{192}{61}{62} Prediction + Bug Type} & \mbox{\cblock{50}{116}{161} Prediction} \\
    \mbox{\cblock{169}{170}{53}  Prediction + Location} & \mbox{\cblock{147}{114}{178} Prediction + Cause} \\
    \mbox{\cblock{225}{129}{44}  Prediction + Bug Type + Location} &
    \end{tabular}
    }
    \includegraphics[width=0.5\linewidth]{Images/error-analysis_strict_performance.pdf}
    \caption{Performance of the best prompting method/seed.
    \textit{Prediction} displays binary prediction accuracy; bars with \textit{Bug Type}, \textit{Location}, and \textit{Cause} display correct predictions for explaining a vulnerability.
    GPT-3.5, GPT-4, and Gemini each produced fewer than 5 eligible explanations each and are excluded.
    % \benjamin{TODO: Check against Precision results in above figures.}
    }
    \label{fig:strict-performance}
\end{figure}


\Cref{fig:strict-performance} presents the second part of the results of RQ3. Here, we provide a summary of the models' capability of reporting the type, the location and the root cause of a vulnerability. The results show that although most LLMs correctly predicted up to 79\% of vulnerable examples (blue bar), correctness dropped substantially when we consider the predicted location, bug type, and causes.
Considering both bug types and locations (orange bar), all models dropped in correctness, decreasing by 18-67\%, with Mistral failing on all examples.
Considering root-cause explanations (purple bar), model correctness decreased by 24-50\%.

\begin{summarybox}
\textbf{Summary:}
57\% of LLM responses contained errors when explaining the cause of vulnerabilities.
The most common error categories were ``Code understanding'' (41\% of responses, especially missing Bounds/NULL Checks) and ``Hallucination/Memorization/Repetition'' (11\% of responses).
All LLMs experienced a substantial (18-100\%) drop in correctness when considering their predictions of bug location, type and causes.
\end{summarybox}


\section{How to Improve Existing LLMs for Vulnerability Detection}

\ben{TODO: Explain cot-explanation prompts (as well as contrastive and Cot-sa, Cot-CVE if they end up here)}

\subsection{Performance evaluation}

\begin{table}[htbp]
\centering
\caption{Performance of baseline approaches vs. our proposed prompting methods.}
\label{tab:our-approach-performance}
\begin{tabular}{l rl rl rrr}
\toprule
    \textbf{Model} & \multicolumn{2}{c}{\textbf{Best baseline}} & \multicolumn{2}{c}{\textbf{Contrastive}} & \textbf{CoT-SA} & \textbf{CoT-CVE} & \textbf{CoT-explanation} \\
    \midrule
    LLAMA 2 & 0.7 & (IC-Random) & 0.8 & (Random) & xxx & xxx & xxx \\
    Code LLAMA & x & x & x & x & x & x & x \\
    Mistral & x & x & x & x & x & x & x \\
    Mixtral & x & x & x & x & x & x & x \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Error analysis on CoT prompts}

\mycomment{
\subsection{RQ4: How do LLMs compare to human developers for localizing vulnerabilities?}
\label{sec:dbgbench}

\ben{Merge this section's results with RQ1, it is not interesting enough to deserve its own section.}

% dbgbench includes one buffer overflow, https://dbgbench.github.io/find.c8491c11.diagnosis.txt
\subsubsection{Study setup} We are interested in how LLMs' performance compares to human's. To set up the experiments, we used DbgBench~\cite{dbgbench}, where the detailed human performance is reported. In their study~\cite{dbgbench}, 12 professional software engineers were given the source code, bug reports, and test cases related to 27 bugs in the \texttt{find} and \texttt{grep} utilities, such as null-pointer dereferences, buffer overflows, resource leaks, and infinite loops.  They reported a diagnosis with fault locations, rated their perception of the difficulty, and provided a patch. To match the human setting, we gave each LLM prompts containing the bug report, test case, the source code of the files containing the faults, and instructions ``Given the above bug report, test case which reproduces the bug, and source code, provide the line numbers of all fault locations in the code in the following format: \texttt{* file.c:line number}.''
These prompts (averaging 19-25k tokens) exceeded the context length of 4 models, which we excluded.
We extracted fault locations from the outputs of the remaining 7 LLMs and compared them with the correct fault locations from DbgBench, considering a prediction correct if at least one fault location matched the ground truth.


\begin{table}[htbp]
    \centering
    \caption{LLMs correctly located 6 out of 27 DbgBench bugs.
    \textit{Human performance} reports the average perceived difficulty and time to diagnosis, and the percentage of human participants which correctly localized each bug.
    2 models failed to localize any bugs (not shown), including GPT-4.
    }
    \label{tab:dbgbench-correct}

\colorlet{myGray}{gray!25!}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrl}
\toprule
 & \multicolumn{3}{c}{Human performance} \\
 \cmidrule{2-4}

%%%% AUTOGENERATED
Total 6 Bugs & \makecell[r]{Human\\Correct} & \makecell[r]{Diagnosis\\Time (min.)} & \makecell[r]{Difficulty\\Rating (1-5)} & Model \\
\midrule
\rowcolor{myGray} & & & & GPT-3.5 \\
\rowcolor{myGray} \multirow{-2}{*}{find.24bf33c0} & \multirow{-2}{*}{71\%} & \multirow{-2}{*}{31} & \multirow{-2}{*}{Moderate (3)} & Mixtral-MoE \\
\multirow{2}{*}{grep.2be0c659} & \multirow{2}{*}{78\%} & \multirow{2}{*}{29} & \multirow{2}{*}{Moderate (3)} & Gemini \\
& & & & MagiCoder \\
\rowcolor{myGray} grep.c96b0f2c & 80\% & 50 & Very Difficult (4) & GPT-3.5 \\
\multirow{2}{*}{grep.3220317a} & \multirow{2}{*}{100\%} & \multirow{2}{*}{42} & \multirow{2}{*}{Very Difficult (4)} & Code LLAMA \\
& & & & Mixtral-MoE \\
\rowcolor{myGray} & & & & Code LLAMA \\
\rowcolor{myGray} & & & & Gemini \\
\rowcolor{myGray} & & & & GPT-3.5 \\
\rowcolor{myGray} \multirow{-4}{*}{grep.5fa8c7c9} & \multirow{-4}{*}{100\%} & \multirow{-4}{*}{26} & \multirow{-4}{*}{Moderate (3)} & MagiCoder \\
grep.55cf7b6a & 100\% & 15 & Slight (2) & GPT-3.5 \\
%%%% AUTOGENERATED

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


\subsubsection{RQ4 Results}
\Cref{tab:dbgbench-correct} shows that among the 7 models, 5 models produced correct output for 6 bugs and made a total of 11 correct predictions (some models predict correctly on the same bug). GPT-3.5 performed the best and correctly located 4 bugs. Interestingly, the newer model, GPT-4, did not match the ground-truth fault locations on any examples, and neither did Mistral. These bugs took humans 15 to 50 minutes to diagnose, with difficulty ratings ranging from slightly to very difficult (2-4 on a scale of 1 to 5).
\Cref{fig:dbgbench-distribution} shows where these bugs located in the entire dataset in terms of perceived difficulty and diagnostic time given by DbgBench.


\begin{figure}[htbp]
    \centering
    \begin{tabular}{ll}
    \mbox{\cboxfill{53}{53}{53}{166}{206}{227} Human Time/Difficulty} &
    \mbox{\cboxfill{53}{53}{53}{31}{120}{180} Correct LLM prediction}
    \end{tabular}
    \includegraphics[width=0.5\linewidth]{Images/dbgbench_distribution.pdf}
    \caption{The distribution of time and difficulty reported by humans in DbgBench, and the portion of examples predicted correctly by at least one LLM.
    }
    \label{fig:dbgbench-distribution}
\end{figure}



In \Cref{fig:dbgbench-performance}, we visualize individual bugs and rank them based on the ``easiness'' of diagnosis for humans. To do so, we first rank the bugs based on the correctness achieved among the developers who diagnosed the bug, and to break ties, we compared the diagnosis time. Here, we can see that LLMs failed to correctly predict the examples which were the hardest for humans (rightmost dots), as well as many of the easiest examples (missing 4 out of 7 leftmost dots which were localized by 100\% of humans). Overall,  LLMs performed substantially worse than humans. Most of the correct predictions were among those already correctly diagnosed by 70-100\% of human study participants. These findings suggest that current LLMs still have significant limitations in localizing software bugs in a real-world setting.


\begin{figure}[htbp]
    \centering
    \small{\begin{tabular}{ll}
\mbox{\ccircle{31}{119}{180} Human diagnosis} &
\mbox{\cex{34}{30}{31} All models incorrect} \\
\addlinespace[1ex]
\multicolumn{2}{c}{Correct LLM Localizations} \\
\midrule
\mbox{\cplus{44}{160}{44} GPT-3.5} &
\mbox{\cplus{31}{119}{180} GPT-3.5 + Mixtral-MoE} \\
\mbox{\cplus{255}{127}{14} Gemini + MagiCoder} &
\mbox{\cplus{214}{39}{40} Mixtral-MoE + Code LLAMA} \\
\multicolumn{2}{l}{\mbox{\cplus{148}{103}{189} GPT-3.5 + Gemini + Code LLAMA + MagiCoder}}
    \end{tabular}}

    \includegraphics[width=0.5\linewidth]{Images/dbgbench.pdf}

    \caption{Comparison of Human and LLM performance on all bugs in DbgBench.
    Bugs are ordered along the X-axis by human performance/diagnostic time.
    Y-axis indicates the percentage of humans or LLMs that correctly localized the bug.
    }
    \label{fig:dbgbench-performance}
\end{figure}

\begin{summarybox}
\textbf{Summary for RQ4:}
LLMs correctly located 6/27 bugs from DbgBench, while at least one human correctly located 27/27 bugs. GPT-3.5 performed the best and correctly located 4 bugs. GPT-4 and Mistral failed to locate any bugs correctly.
\end{summarybox}

}
\section{Threats to Validity}
Better prompts than those we evaluated may exist.
To draw out the best model performance, we systematically explored several prominent prompting techniques and introduced three new approaches motivated by our domain knowledge (\Cref{sec:rq1}).
Model performance can be reduced by irrelevant context~\cite{distractibility}, or the order~\cite{incontext_order} and quality~\cite{incontext_number} of in-context examples. To alleviate these potential issues, we reported the best-case performance among various prompt orderings and varying amounts and sources of context, and tried different number of shots (\Cref{sec:discussion}).

We queried 100 functions due to the cost of LLMs (see \Cref{sec:dataset}), which may seem limited. However, we note that our dataset originates from 36 open-source projects with diverse applications, including databases, servers, and interpreters.
The vulnerabilities represent important issues, all featuring in the top-25 most dangerous CWEs for the past five years~\cite{cwe_stubborn}, and were manually curated to ensure quality~\cite{croft_quality} and focus on real-world use cases~\cite{sven}. We performed a pilot study which suggests that the models did not memorize the labels (\Cref{sec:discussion}).

To mitigate potential biases from the experimental setup and metrics, we evaluated the LLMs in two distinct scenarios: ``paired'' and ``unpaired'' (\Cref{sec:rq2}), and aggregated results across 3 different random seeds. We justify our choice of metrics in \Cref{sec:metrics}.

The analysis of the LLMs errors can involve subjective judgments. To ensure confident classifications, we rigorously designed the categories to be unambiguous and confirmed agreement among multiple raters (\Cref{sec:rq3}).

Our fault localization setting for DbgBench does not perfectly match the human debugging scenario, as the LLMs could not run tests or use debuggers. While such tools could aid LLMs in making a diagnosis, we focused on a direct use of LLMs in this study. Investigating long-context integration and interactive agent environments is an interesting direction for future work. 

\section{Discussions}
\label{sec:discussion}

Because SVEN is open-source, the labels may be inside the training dataset of recent LLMs. To test if LLMs memorized vulnerability labels, we refactored the code (using NatGen~\cite{chakraborty2022natgen}) while preserving the vulnerability labels and evaluated the models.
If the models simply memorized the vulnerability labels, we would expect performance to be substantially reduced on the refactored code. We saw both improvements and reductions in performance and only small differences in Balanced Accuracy (0.02-0.09), even with extensive refactoring.

As a pilot study, we tried using 2, 4, 6, or 8 in-context examples for the models which performed best with in-context prompts and found that 6-shots performed best for most models.
Extended results for both experiments can be found in our data package~\cite{data-package-figshare}.

\section{Related Work}
\label{sec:related-work}

LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been applied in various software engineering tasks, such as code generation~\cite{humaneval}, test generation~\cite{lemieux_testgen}, and code summarization~\cite{ahmed2024automatic}
through the use of prompting.
Effective prompts can condition the model for a specific task like Question/Answer~\cite{gpt3}, provide additional information through in-context examples~{\cite{rag}} and elicit step-by-step reasoning through chain-of-thought examples~{\cite{cot,kojima2022large}}.
We have surveyed these state-of-the-art prompting methods and applied them to the vulnerability detection task.

Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as zero-shot prompting ~{\cite{vulDetIssrew-2023, fu2023chatgpt}}, in-context learning~{\cite{gao2023far,liuGptandIncontext2023,chan2023transformerbased}}, and fine-tuning~{\cite{shestov2024finetuning, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized chain-of-thoughts (CoT), such as ``Let's think step-by-step''~{\cite{li2023hitchhikers, automatedbugreplay-icse2024,sun2023gptscan}}, multi-step prompts~{\cite{ullah2023large,yu2024security}}, and generic information such as CFG, DFG, PDG, and API calls~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.
In this work, we propose three novel prompt approaches tailored for vulnerability detection, integrating information from bug-fix commits (contrastive pairs), CVE descriptions (CoT-CVE), and static analysis reports (CoT-SA). We reported the capabilities of LLMs to distinguish buggy and patched versions of code.

Several concurrent papers have taken initial steps to analyze errors in LLM-generated vulnerability detection responses (to the best of our knowledge, the papers are in arXiv but not yet published).
\citet{yu2024security} analyzed 82 responses and identified problems based a taxonomy of errors in ChatGPT responses to StackOverflow and general-purpose queries, corroborating our findings that the models struggled with  correctness, logic and consistency.
\citet{nong2024chainofthought} categorized 100 incorrect predictions from GPT-3.5 into {\it Insufficient Context}, {\it CWE Oblivion}, {\it Incomplete Control Flow/Data Flow}; similarly, \citet{sun2024llm4vuln} used an LLM guided by 300 human annotations to categorize incorrect predictions into  {\it Wrong Reasoning}, {\it Need Detailed Analysis}, {\it Need Other Code}, and {\it Other}.
\citet{ullah2023large} automatically compared GPT-4's summarization of LLM reasoning with human-generated reasoning based on BLEU, ROUGE, and GPT-4.

Our error classifications provide more fine-grained categories than prior work (see \Cref{tab:fine-grained}) and allow us to analyze the code structures which affected the correctness of explanations, and thus potentially provide better guidance for future improvement of LLMs for vulnerability detection. We provide a quantitative comparison of LLMs and human's performance on locating bugs. To the best of our knowledge, our work is the most comprehensive: compared to prior works, we analyzed more models (11), and used multiple raters with a rigorous agreement protocol based on Fleiss' $\kappa$ to manually annotate a larger set of 287 LLM responses.

\section{Conclusions}
We comprehensively evaluated the vulnerability detection capabilities of LLMs from the standpoint of their performance as well as their errors.
We found that they performed only slightly better than random guessing (0.5-0.63 Balanced Accuracy), and that they struggled to differentiate buggy and fixed code versions, making the same prediction for 76\% of pairs.
We proposed CoT from Static Analysis and Contrastive pairs, which improved the performance of some models.
LLMs frequently made Code Understanding, Common Knowledge, Hallucination, and Logic errors when explaining vulnerabilities, with 57\% of responses containing errors.
On complex debugging tasks from DbgBench, LLMs performed far worse than humans, correctly localizing only 6/27 bugs.
These findings highlight LLMs' limitations in vulnerability detection and our dataset of LLM errors provides guidance for future improvement of LLM-based vulnerability detection.


==> _OldVersion.FSE25/prompt-design.tex <==
% \begin{outdated}
% % \begin{flushleft}
% \subsection{RQ1: What are the most successful and least successful prompt designs for LLM-based vulnerability detection?}
% \label{sec:rq1}
% \end{flushleft}

% \subsubsection{Prompting methods}\label{sec:prompt-design}
% We used three existing prompting methods~\cite{liu_pre-train_2021}, including
% {\it Basic (zero-shot) prompting}, {\it In-context ($n$-shot) prompting}, and {\it In-context prompting based on embedding similarity}. 
% We also designed three new prompting methods, namely \textit{In-context prompting based on contrastive pair}, \textit{Chain-of-Thought from CVE descriptions}, and {\it Chain-of-Thought from static analysis}.

% \ben{There are lots of ways to phrase the prompts, so we roughly used the simplest phrasing that worked best out of the ones we tried, and match up with the method proposed by related works.}

% https://tex.stackexchange.com/a/461533
% https://tex.stackexchange.com/a/96298
\begin{description}[leftmargin=0pt,style=unboxed]
\item [Basic (zero-shot) prompting~\citep{fu2023chatgpt}:] 
We first designed a system prompt to set the context: ``I want you to act as a vulnerability detection system'', along with natural-language instructions:
(1) \textit{Basic query}: ``Is the following function buggy? Please answer Yes or No.'' (We also tried ``Is the following function vulnerable?"; however, our pilot study shows that it did not perform as well.)
(2) \textit{CWE list}: This prompt starts with ``Does the following function contain one of the following bug types?'', followed by a fixed list of bug types, e.g., ``CWE-190: Integer Overflow'';
(3) \textit{Q/A}: Begin the query with ``Question:'' and begin the model's response with ``Answer:''. This conditions the model to respond in a question-answering mode.

\item[In-context ($n$-shot) prompting\citep{liuGptandIncontext2023,zhou2024large}:]
% \ben{Merge with below to discuss random (no retrieval), TF-IDF/BM25, and CodeBERT retrieval.}
In this prompt, we provide examples of inputs and responses for in-context learning~\citep{gpt3}.
The in-context examples condition the model to reply in the same format as the example responses~\citep{stanford_incontext}. The selection of in-context examples can impact the performance. We studied three settings: (1) randomly selected examples, (2) the examples that had similar embeddings to the query example, and (3) the examples from {\it contrastive pairs} (see below for details).

% \item[In-context prompting based on embedding similarity:] Choose the in-context examples which are most similar to the code in the query, where ``similar'' is approximated by the vector proximity between code embeddings.
% Examples which are closer in embedding space can be more relevant to the query code~\cite{rag}.
% We surveyed several embedding models~\citep{reimers2019sentencebert,openai_embeddings,codebert} and chose CodeBERT~\citep{codebert} because it
% performed best. We searched the SVEN dataset (the 100 examples we used) for similar examples.

\item[In-context prompting based on contrastive pairs:] 
We formed \textit{contrasting pairs} of in-context examples by providing the vulnerable version of the code (before the bug-fixing commit) and the fixed version (after the commit) as in-context examples in the same prompt. Since these two versions of the source code differ primarily in the portion related to the bug-fix, our intention is that this prompt template would highlight the cause of the bug and instruct the model to learn that the small differences in code can lead to different labels.

\item[In-context prompting based on CoT from CVE descriptions:]
We designed ``chain-of-thought'' prompts by providing intermediate reasoning steps which lead to the answer, inspired by \citet{cot}. We use in-context examples from the Big-Vul dataset~\citep{bigvul}, which includes the CVE bug reports. For vulnerable examples,  we used the default in-context query and provide the chain-of-thought response. To produce such response, we adapt the descriptions in these bug reports to describe how the bug manifests.
% https://nvd.nist.gov/vuln/detail/CVE-2013-6051
For example, CVE-2017-9211~\cite{CVE-2017-9211} describes the vulnerability, including the symptoms, attack surface, and variable involved:

\begin{flushleft}
\small{\texttt{The crypto\_skcipher\_init\_tfm function in crypto/skcipher.c in the Linux kernel through 4.11.2 relies on a setkey function that lacks a key-size check, which allows local users to cause a denial of service (NULL pointer dereference) via a crafted application.}}
% \small{{\tt The {bgp\_attr\_unknown} function in bgp\_attr.c in {Quagga~0.99.21} {does not properly initialize the {total} variable}, which allows remote attackers to cause a {denial of service} (bgpd crash) via a {crafted BGP update}}}.
% A NULL pointer dereference vulnerability in the function nfc_genl_deactivate_target() in net/nfc/netlink.c in the Linux kernel before 5.1.13 can be triggered by a malicious user-mode program that omits certain NFC attributes, leading to denial of service.
% \small{\texttt{The matchCurrentInput function inside lou\_translateString.c of Liblouis prior to 3.7 does not check the input string's length, allowing attackers to cause a denial of service (application crash via out-of-bounds read) by crafting an input file with certain translation dictionaries.}}
\end{flushleft}

We use this description as the CoT response and  append ``Therefore, the example is buggy'' to complete the response.
For non-vulnerable examples, we provide the default in-context example query/response.

\item[In-context prompting based on CoT from static analysis:] We also used the output buggy paths reported by static analysis tools to prepare the chains of thought prompt. The buggy path consists of a list of statements that can lead to the bug. We use in-context examples from the D2A dataset~\cite{d2a}, which lists buggy paths from the Infer static analyzer~\cite{fbinfer} for several open-source C++ projects.
We convert the buggy paths to natural language descriptions and use them as the response. This is an example COT response for a buffer overflow vulnerability:

\begin{flushleft}
\small{\texttt{%
1. A buffer buf of size 10 is {allocated} at line 1.\\
2. An index i is {initialized to a value} in the range [0, 100] at line 2.\\
3. The index {i is used to access buf} at line 3. 
{This may exceed the bounds of buf.}\\
}}
\end{flushleft}

We append ``Therefore, the example is buggy'' to complete the response.
For non-vulnerable examples, we provide the default response.

\end{description}

Considering the numerous ways the above prompting techniques can be combined, we systematically searched for high-performing prompts for each model.
For the basic prompting method, we evaluated four ``modes'' ---
(1) basic query, (2) Q/A, (3) CWE list, and (4) both Q/A and CWE list --- and designated the best-performing mode as the \textbf{Basic} prompting approach.

For the in-context prompting methods, we evaluated random selection \textbf{(IC-Random)}, embedding similarity search \textbf{(IC-Embedding)}, chain-of-thought from CVE descriptions \textbf{(CoT-CVE)}, and chain-of-thought from static analysis \textbf{(CoT-SA)}.
We did a pilot study (\S~\ref{sec:discussion}) and found that 6 shots performed the best for most models and was the maximum number of examples that fit within most models' context sizes. Thus, we used 6 shots for all in-context prompts.
For each approach, we used two configurations: (1) 6 randomly-selected examples as well as (2) 3 contrastive pairs. We then selected the best outcome for each model and prompting method.
We list examples of the prompts and more details in our data package~\cite{data-package-figshare}.

% \end{outdated}

==> _OldVersion.ICSE25/Figures/dbgbench/difficulty-time.tex <==
\begin{figure}[t]
    \centering
    % Correct Localizations
    
    % \begin{tabular}{lll}
    % \mbox{\ccircle{31}{119}{180} GPT-3.5} &
    % \mbox{\ccircle{255}{127}{14} Gemini} &
    % \mbox{\ccircle{44}{160}{44} MagiCoder} \\
    % \mbox{\ccircle{214}{39}{40} Mixtral-MoE} &
    % \mbox{\ccircle{148}{103}{189} Code LLAMA} \\
    \begin{tabular}{ll}
    % \mbox{\cboxfill{53}{53}{53}{128}{128}{128} LLM} &
    % \mbox{\cbox{34}{30}{31} Human}
    % rgb(166, 206, 227)
    % rgb(31, 120, 180)
    
    \mbox{\cboxfill{53}{53}{53}{166}{206}{227} Human Time/Difficulty} &
    \mbox{\cboxfill{53}{53}{53}{31}{120}{180} Correct LLM prediction}
    
    % \mbox{\cboxfill{53}{53}{53}{166}{206}{227} Human Time} &
    % \mbox{\cboxfill{53}{53}{53}{166}{206}{227} Human Difficulty}\\
    % \multicolumn{2}{c}{\cboxfill{53}{53}{53}{31}{120}{180} Correct LLM prediction}
    
    %&
    % \mbox{\colorline{} Mean}
    \end{tabular}
    % \includegraphics[width=0.49\linewidth]{Images/dbgbench/LLMVsDifficulty.png}%
    % \includegraphics[width=0.49\linewidth]{Images/dbgbench/LLMVsTime.png}
    \includegraphics[width=\linewidth]{Images/dbgbench/dbgbench_distribution.pdf}
    \caption{The distribution of time and difficulty reported by humans in DbgBench, and the portion of examples predicted correctly by at least one LLM.
    % The X-axis positions of the points are arbitrary and used to avoid overlap.
    }
    % Demo figures for DbgBench.
    % LLMs correctly predicted 4 examples which humans tended to rate ``Moderate'' difficulty and took 25-45 minutes to debug.}
    \label{fig:dbgbench-distribution}
\end{figure}


==> _OldVersion.ICSE25/Figures/dbgbench/performance-figure.tex <==


%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \small{\begin{tabular}{ll}
% \mbox{\ccircle{34}{30}{31} Human diagnosis} &
\mbox{\ccircle{31}{119}{180} Human diagnosis} &
\mbox{\cex{34}{30}{31} All models incorrect} \\
\addlinespace[1ex]
\multicolumn{2}{c}{Correct LLM Localizations} \\
\midrule
\mbox{\cplus{44}{160}{44} GPT-3.5} &
\mbox{\cplus{31}{119}{180} GPT-3.5 + Mixtral-MoE} \\
\mbox{\cplus{255}{127}{14} Gemini + MagiCoder} &
\mbox{\cplus{214}{39}{40} Mixtral-MoE + Code LLAMA} \\
\multicolumn{2}{l}{\mbox{\cplus{148}{103}{189} GPT-3.5 + Gemini + Code LLAMA + MagiCoder}}
    \end{tabular}}

    \includegraphics[width=0.8\linewidth]{Images/dbgbench/dbgbench.pdf}

% \tikz\draw[thick, color=red] (-0.3,0) -- (0.3,0.6) (-0.3,0.6) -- (0.3,0);
% \tikz[baseline]\draw[line width=2.5pt, color=red] (-0.1,0) -- (0.1,0.2) (-0.1,0.2) -- (0.1,0);
    
    \caption{Comparison of Human and LLM performance on all bugs in DbgBench.
    Bugs are ordered along the X-axis by human performance/diagnostic time.
    Y-axis indicates the percentage of humans or LLMs that correctly localized the bug.
    % Points are ordered by human performance along the X axis and their height shows the percentage of humans or LLMs which correctly localized the bug.
    % \benjamin{
    % TODO: Add summary of all model performance, including models that didn't correctly predict any.
    % TODO: Add bug type and other interesting metadata.
    % TODO: Add the bug labels on the X axis.
    % }
    % \wei{TODO: Make human dots blue}
    % \benjamin{TODO: Fix overlap in x axis tick labels.}
    }
    \label{fig:dbgbench-performance}
\end{figure}


==> _OldVersion.ICSE25/Figures/dbgbench/performance-table.tex <==
\begin{table}[t]
    \centering
    \caption{LLMs correctly located 6 out of 27 DbgBench bugs.
    \textit{Human performance} reports the average perceived difficulty and time to diagnosis, and the percentage of human participants which correctly localized each bug.
    2 models failed to localize any bugs (not shown), including GPT-4.
    % \wei{TODO: Update all rows, sort bugs by difficulty, can we merge the bugs}
    }
    \label{tab:dbgbench-correct}

\colorlet{myGray}{gray!25!}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrl}
\toprule
 & \multicolumn{3}{c}{Human performance} \\
 \cmidrule{2-4}

%%%% AUTOGENERATED
Total 6 Bugs & \makecell[r]{Human\\Correct} & \makecell[r]{Diagnosis\\Time (min.)} & \makecell[r]{Difficulty\\Rating (1-5)} & Model \\
\midrule
\rowcolor{myGray} & & & & GPT-3.5 \\
\rowcolor{myGray} \multirow{-2}{*}{find.24bf33c0} & \multirow{-2}{*}{71\%} & \multirow{-2}{*}{31} & \multirow{-2}{*}{Moderate (3)} & Mixtral-MoE \\
\multirow{2}{*}{grep.2be0c659} & \multirow{2}{*}{78\%} & \multirow{2}{*}{29} & \multirow{2}{*}{Moderate (3)} & Gemini \\
& & & & MagiCoder \\
\rowcolor{myGray} grep.c96b0f2c & 80\% & 50 & Very Difficult (4) & GPT-3.5 \\
\multirow{2}{*}{grep.3220317a} & \multirow{2}{*}{100\%} & \multirow{2}{*}{42} & \multirow{2}{*}{Very Difficult (4)} & Code LLAMA \\
& & & & Mixtral-MoE \\
\rowcolor{myGray} & & & & Code LLAMA \\
\rowcolor{myGray} & & & & Gemini \\
\rowcolor{myGray} & & & & GPT-3.5 \\
\rowcolor{myGray} \multirow{-4}{*}{grep.5fa8c7c9} & \multirow{-4}{*}{100\%} & \multirow{-4}{*}{26} & \multirow{-4}{*}{Moderate (3)} & MagiCoder \\
grep.55cf7b6a & 100\% & 15 & Slight (2) & GPT-3.5 \\
%%%% AUTOGENERATED

%%%% AUTOGENERATED
% Reorder with difficult first, swap multirow
% Total 6 Bugs & \makecell[r]{Human\\Correct} & \makecell[r]{Diagnosis\\Time (m.)} & \makecell[r]{Difficulty\\Rating (1-5)} & Model \\
% \midrule
% \rowcolor{myGray} grep.55cf7b6a & 100\% & 15 & Slight (2) & GPT-3.5 \\
% \multirow{4}{*}{grep.5fa8c7c9} & \multirow{4}{*}{100\%} & \multirow{4}{*}{26} & \multirow{4}{*}{Moderate (3)} & Code LLAMA \\
% & & & & Gemini \\
% & & & & GPT-3.5 \\
% & & & & MagiCoder \\
% \rowcolor{myGray} \multirow{2}{*}{grep.3220317a} & \multirow{2}{*}{100\%} & \multirow{2}{*}{42} & \multirow{2}{*}{Very Difficult (4)} & Code LLAMA \\
% \rowcolor{myGray} & & & & Mixtral-MoE \\
% grep.c96b0f2c & 80\% & 50 & Very Difficult (4) & GPT-3.5 \\
% \rowcolor{myGray} \multirow{2}{*}{grep.3220317a} & \multirow{2}{*}{78\%} & \multirow{2}{*}{29} & \multirow{2}{*}{Moderate (3)} & Gemini \\
% \rowcolor{myGray} & & & & MagiCoder \\
% \multirow{2}{*}{find.24bf33c0} & \multirow{2}{*}{71\%} & \multirow{2}{*}{31} & \multirow{2}{*}{Moderate (3)} & GPT-3.5 \\
% & & & & Mixtral-MoE \\
%%%% AUTOGENERATED

% Wei's edits
% \midrule
% Total 6 Bugs & \makecell[r]{Difficulty\\Rating (1-5)} & \makecell[r]{Diagnosis\\Time (m)} & \makecell[r]{Human\\Correct} & Model \\
% \midrule
% \rowcolor{myGray} grep.3220317a & Very Difficult (4) & 42 & 100\% & Code LLAMA \\
% \rowcolor{myGray} grep.3220317a & Very (4) & 42 min. & 100\% & Mixtral-MoE \\
% grep.55cf7b6a & Slight (2) & 15 m. & 100\% & GPT-3.5 \\
% \rowcolor{myGray} grep.5fa8c7c9 & Moderate (3) & 26 min. & 100\% & Code LLAMA \\
% \rowcolor{myGray} grep.5fa8c7c9 & Moderate (3) & 26 min. & 100\% & Gemini \\
% \rowcolor{myGray} grep.5fa8c7c9 & Moderate (3) & 26 min. & 100\% & GPT-3.5 \\
% \rowcolor{myGray} grep.5fa8c7c9 & Moderate (3) & 26 min. & 100\% & MagiCoder \\
% find.24bf33c0 & Moderate (3) & 31 min. & 71\% & GPT-3.5 \\
% find.24bf33c0 & Moderate (3) & 31 min. & 71\% & Mixtral-MoE \\
% \rowcolor{myGray} grep.2be0c659 & Moderate (3) & 29 min. & 78\% & Gemini \\
% \rowcolor{myGray} grep.2be0c659 & Moderate (3) & 29 min. & 78\% & MagiCoder \\
% grep.c96b0f2c & Very (4) & 50 min. & 80\% & GPT-3.5 \\

% Initial data
% Bug & \makecell[l]{Difficulty\\Rating} & \makecell[l]{Diagnosis\\Time (min.)} & Match (\%) & Model \\
% \midrule
% \multirow{2}{*}{grep.5fa8c7c9} & \multirow{2}{*}{Moderate} & \multirow{2}{*}{26} & \multirow{2}{*}{100\%} & Code LLAMA \\
%  & & & & Mistral \\
% grep.3220317a & Moderate & 42 & 100\% & Code LLAMA \\
% find.6e4cecb6 & Moderate & 33 & 89\% & Mistral \\
% grep.7aa698d3 & Moderate & 31 & 80\% & Code LLAMA \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> _OldVersion.ICSE25/Figures/error-analysis/categories.tex <==
\begin{figure}[t]
    \centering
    \small{Does the response contain an error?\\
    \begin{tabular}{ll}
    \mbox{\cblock{58}{146}{58} No} &
    \mbox{\cblock{192}{61}{62} Yes}
    \end{tabular}}
    \centering
    \includegraphics[width=\linewidth]{Images/error-analysis/error_categories.pdf}
    \caption{Error categories observed in responses from all LLMs.
    Bar width shows the number of errors observed in each category. Bar labels show the percentage of responses containing each category of error. Responses can contain more than one error.}
    \label{fig:error-categories}
    % \end{subfigure}
\end{figure}


==> _OldVersion.ICSE25/Figures/error-analysis/dbgbench-old.tex <==

\begin{table}[htbp]
    \centering
    \caption{DBGBench results. \benjamin{WIP.
    TODO: Add summary of model performance, including models that didn't correctly predict any.
    % Most participants completed only up to 12 examples; \textit{Marks Location} should reflect how many examples the participants in each percentile completed.
    }}
    \label{tab:my_label}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llllr}
\toprule
Vulnerability & Model & Diagnosis Time & Difficulty & Human \\
\midrule
grep.3220317a & Code LLAMA & 50 - 60 min. & Moderate & 100\% \\
grep.5fa8c7c9 & Code LLAMA & 30 - 40 min. & Moderate & 100\% \\
grep.5fa8c7c9 & Mistral & 30 - 40 min. & Moderate & 100\% \\
grep.7aa698d3 & Code LLAMA & 40 - 50 min. & Moderate & 80\% \\
find.6e4cecb6 & Mistral & 40 - 50 min. & Moderate & 89\% \\
\bottomrule
\end{tabular}
\end{adjustbox}

\vspace*{0.25 cm}

% \caption{Human performance.}
% \begin{tabular}[t]{lr}
% \toprule
% Percentile & Human Match \% \\
% \midrule
% 25\% & 71\% \\
% 50\% & 82\% \\
% 75\% & 96\% \\
% 100\% & 100\% \\
% \bottomrule
% \end{tabular}

% \vspace*{0.25 cm}

% \caption{Perceived difficulty and diagnosis time of all bugs in DbgBench. \benjamin{TODO: histogram of perceived difficulty level, diagnosis time, and human match \%, with points for LLM detections.}}
% \begin{tabular}[t]{lr}
% \toprule

% Diagnosis Time & Count \\
% \midrule
% 10 - 20 minutes & 1 \\
% 20 - 30 minutes & 5 \\
% 30 - 40 minutes & 4 \\
% 40 - 50 minutes & 11 \\
% 50 - 60 minutes & 4 \\
% 60 minutes or more & 2 \\
% \bottomrule
% \end{tabular} \quad %
% % 
% \begin{tabular}[t]{lr}
% \toprule

% Perceived Difficulty & Count \\
% \midrule
% Slightly difficult & 5 \\
% Moderately difficult & 13 \\
% Very difficult & 8 \\
% Extremely difficult & 1 \\
% \bottomrule
% \end{tabular}

\end{table}

% \begin{table}[htbp]
%     \centering
%     \caption{DBGBench results. \benjamin{WIP. Most participants completed only up to 12 examples; \textit{Marks Location} should reflect how many examples the participants in each percentile completed.}}
%     \label{tab:my_label}
% \begin{tabular}{lrrr}
% \toprule
% LLM & Marks Location & \# Location & \# Match \\
% \midrule
% Code LLAMA & 100.0\% & 18.2 & 3.0 \\
% Mistral & 92.9\% & 29.2 & 2.0 \\
% GPT-4 & 42.9\% & 33.1 & 0.0 \\
% MagiCoder & 75.0\% & 30.7 & 0.0 \\
% Mixtral-MoE & 82.1\% & 9.1 & 0.0 \\
% \midrule Human Percentile \\
%  \midrule 90 & & 70.5 & 12.0 \\
% 80 & & 57.5 & 12.0 \\
% 70 & & 44.9 & 11.0 \\
% 60 & & 28.0 & 10.0 \\
% 50 & & 13.4 & 9.0 \\
% 40 & & 8.3 & 8.0 \\
% 30 & & 4.0 & 6.0 \\
% 20 & & 3.1 & 3.0 \\
% 10 & & 3.0 & 2.0 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> _OldVersion.ICSE25/Figures/error-analysis/fine-grained-errors.tex <==
\begin{table}[t]
\centering
    \centering
    \caption{Fine-grained errors across 287 responses to 100 programs.
    For select \textit{Code understanding} errors related to specific code structures, the total number of responses containing those structures and the percentage with an error are shown.
    % \wei{why control flow syntax datatype does not have a total?}
    }
    \label{tab:fine-grained}
\begin{tabular}{llr}
\toprule
Error category & Error & Count \\
\midrule
\multirow[t]{10}{*}{Code understanding} & Bounds/NULL check & 76/159 (48\%) \\
 & String operation & 3/29 (10\%) \\
 & Integer math & 8/96 \myspace(8\%) \\
 & Pointer operation & 9/147 \myspace(6\%) \\
 & Alloc/Free operation & 4/81 \myspace(5\%) \\
 & Index operation & 1/60 \myspace(2\%) \\
 & Control flow & 11 \\
 & Syntax & 5 \\
 & Data type & 1 \\
 \cmidrule{2-3}
 & Total & 118 \\
 \midrule
\multirow[t]{4}{*}{Hal/Mem/Rep} & Hallucination & 15 \\
 & Memorization & 11 \\
 & Repetition & 5 \\
 \cmidrule{2-3}
 & Total & 31 \\
 \midrule
\multirow[t]{3}{*}{Logic error} & Implication & 14 \\
 & Inconsistent & 13 \\
 \cmidrule{2-3}
 & Total & 27 \\
 \midrule
Common knowledge & Total & 8 \\
\bottomrule
\end{tabular}



    % \end{subfigure}
\end{table}


==> _OldVersion.ICSE25/Figures/error-analysis/fine-grained-predictions.tex <==
\begin{figure}[t]
    \centering
    \small{
    \begin{tabular}{ll}
    \mbox{\cblock{192}{61}{62} Prediction + Bug Type} & \mbox{\cblock{50}{116}{161} Prediction} \\
    \mbox{\cblock{169}{170}{53}  Prediction + Location} & \mbox{\cblock{147}{114}{178} Prediction + Cause} \\
    \mbox{\cblock{225}{129}{44}  Prediction + Bug Type + Location} &
    \end{tabular}
    }
    \includegraphics[width=0.9\linewidth]{Images/error-analysis/strict_performance.pdf}
    \caption{Performance of the best prompting method/seed.
    \textit{Prediction} displays binary prediction accuracy; bars with \textit{Bug Type}, \textit{Location}, and \textit{Cause} display correct predictions for explaining a vulnerability.
    GPT-3.5, GPT-4, and Gemini each produced fewer than 5 eligible explanations each and are excluded.
    % \benjamin{TODO: Check against Precision results in above figures.}
    }
    \label{fig:strict-performance}
\end{figure}


==> _OldVersion.ICSE25/Figures/error-examples/hmr-hallucination.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Hallucination}.} \label{fig:hallucination-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 30/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
static int __get_data_block(struct inode *inode, sector_t iblock, struct buffer_head *bh, int create, int flag, pgoff_t *next_pgofs)
{
  struct f2fs_map_blocks map;
  int err;
  map.m_lblk = iblock;
  map.m_len = bh->b_size >> inode->i_blkbits;
  map.m_next_pgofs = next_pgofs;
  err = f2fs_map_blocks(inode, &map, create, flag);
  if (!err) {
    map_bh(bh, inode->i_sb, map.m_pblk);
    bh->b_state = (bh->b_state & ~F2FS_MAP_FLAGS) | map.m_flags;
    bh->b_size = (u64)map.m_len << inode->i_blkbits;
  }
  return err;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
    % Sure! The function \texttt{\_\_get\_data\_block} takes a \texttt{sector\_t} parameter \texttt{iblock} and uses it to calculate the block number for the input \texttt{inode} and \texttt{bh} using the formula \texttt{iblock * (inode->i\_blkbits / 512)}
    
    \ldots
    \hl{if \texttt{iblock} is set to this maximum value, the calculation \texttt{iblock * (inode->i\_blkbits / 512)} will result in a large integer overflow}, causing the calculation to wrap around to a small value.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/hmr-repetition.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Repetition} (code not shown).} \label{fig:repetition-example}
%     \begin{tcolorbox}[title=\textbf{Source code} (Example 49/vulnerable),colframe=Periwinkle]
%     \begin{minted}
%     [
%     frame=lines,
%     numbersep=2mm,
%     breaklines=true,
%     fontsize=\footnotesize,
%     highlightlines={},
%     highlightcolor=yellow,
%     linenos,
%     tabsize=2,
%     ]
%     {c}
% void * CAPSTONE_API cs_winkernel_malloc(size_t size)
% {
%   // Disallow zero length allocation because they waste pool header space and,
%   // in many cases, indicate a potential validation issue in the calling code.
%   NT_ASSERT(size);

%   // FP; a use of NonPagedPool is required for Windows 7 support
% #pragma prefast(suppress : 30030)		// Allocating executable POOL_TYPE memory
%   CS_WINKERNEL_MEMBLOCK *block = (CS_WINKERNEL_MEMBLOCK *)ExAllocatePoolWithTag(
%     NonPagedPool, size + sizeof(CS_WINKERNEL_MEMBLOCK), CS_WINKERNEL_POOL_TAG);
%   if (!block) {
%     return NULL;
%   }
%   block->size = size;

%   return block->data;
% }
%     \end{minted}
%     \end{tcolorbox}
    \begin{tcolorbox}[title={\textbf{Model response} (StarCoder, Example 49/vulnerable)}]
1. The function is buggy because it is not checking for a null pointer.

2. The function is buggy because it is not checking for a null pointer.

\ldots

10. The function is buggy because it is not checking for a null pointer.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/logical-contradiction.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Logical Contradiction}.} \label{fig:contradiction-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 38/vulnerable),colframe=Periwinkle]
% int ecall_restore(const char *input, uint64_t input_len, char **output,
%                   uint64_t *output_len) {
%   if (!asylo::primitives::TrustedPrimitives::IsOutsideEnclave(input,
%                                                               input_len) ||
%       !asylo::primitives::TrustedPrimitives::IsOutsideEnclave(
%           output_len, sizeof(uint64_t))) {
%     asylo::primitives::TrustedPrimitives::BestEffortAbort(
%         "ecall_restore: input/output found to not be in untrusted memory.");
%   }
%   int result = 0;
%   size_t tmp_output_len;
%   try {
%     result = asylo::Restore(input, static_cast<size_t>(input_len), output,
%                             &tmp_output_len);
%   } catch (...) {
%     LOG(FATAL) << "Uncaught exception in enclave";
%   }

%   if (output_len) {
%     *output_len = static_cast<uint64_t>(tmp_output_len);
%   }
%   return result;
% }
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    breakanywhere=true,
    % breakanywheresymbolpre=\tiny\ensuremath{\hookleftarrow},
    % breakanywheresymbolpre=-,
    breakanywheresymbolpre={},
    fontsize=\footnotesize,
    highlightlines={3,9},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
int ecall_restore(const char *input, uint64_t input_len, char **output, uint64_t *output_len) {
  if (!IsOutsideEnclave(input, input_len) ||
      !IsOutsideEnclave(output_len, sizeof(uint64_t)))
    BestEffortAbort("ecall_restore: input/output found to not be in untrusted memory.");
  // ...
  result = Restore(input, static_cast<size_t>(input_len), output, &tmp_output_len);
  // ...
  if (output_len)
    *output_len = static_cast<uint64_t>(tmp_output_len);
  return result;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (Code LLAMA)]
    \ldots
    % 
    \hl{The function then checks if the \texttt{output\_len} pointer is located in untrusted memory}, and if it is not, it aborts the execution.

    \ldots
    % 
    The function is vulnerable to CWE-787: Out-of-bound Write because \hl{the \texttt{output\_len} pointer is not checked to ensure that it is located in untrusted memory} before it is used to store the restored enclave state.
    This could allow an attacker to write to the \texttt{output\_len} pointer, which could lead to a buffer overflow or other security vulnerabilities.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/logical-implication.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of \textbf{Faulty Logical Implication}.} \label{fig:logical-implication-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 11/non-vulnerable),colframe=Periwinkle]
% int avpriv_ac3_parse_header(AC3HeaderInfo **phdr, const uint8_t *buf,
%                             size_t size)
% {
%   GetBitContext gb;
%   AC3HeaderInfo *hdr;
%   int err;

%   if (!*phdr)
%     *phdr = av_mallocz(sizeof(AC3HeaderInfo));
%   if (!*phdr)
%     return AVERROR(ENOMEM);
%   hdr = *phdr;

%   err = init_get_bits8(&gb, buf, size);
%   if (err < 0)
%     return AVERROR_INVALIDDATA;
%   err = ff_ac3_parse_header(&gb, hdr);
%   if (err < 0)
%     return AVERROR_INVALIDDATA;

%   return get_bits_count(&gb);
% }
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={3,6},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
int avpriv_ac3_parse_header(AC3HeaderInfo **phdr, const uint8_t *buf, size_t size) {
  // ...
  err = init_get_bits8(&gb, buf, size);
  if (err < 0)
    return AVERROR_INVALIDDATA;
  err = ff_ac3_parse_header(&gb, hdr);
  if (err < 0)
    return AVERROR_INVALIDDATA;
  return get_bits_count(&gb);
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
    \ldots{}if the input \texttt{buf} is null, then \hl{the \texttt{init\_get\_bits8} call will return a negative value, and the \texttt{ff\_ac3\_parse\_header} call will attempt to access the null pointer \texttt{hdr}}, which will result in a null pointer dereference.
    
    Therefore, the function is vulnerable to a null pointer dereference if the input \texttt{buf} is null.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/understanding-control-flow.tex <==
\begin{figure}[htbp]
    \centering
    % \benjamin{Could be macro, not as typical as the other example. Make sure we know what list\_for\_each\_entry\_safe does. Have some discussion why the error might happen.}
    \caption{Example of \textbf{Incorrect Control-flow}.} \label{fig:control-flow-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 17/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={12,14},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
static void regulator_ena_gpio_free(struct regulator_dev *rdev)
{
	struct regulator_enable_gpio *pin, *n;
	if (!rdev->ena_pin) return;
	/* Free the GPIO only in case of no use */
	list_for_each_entry_safe(pin, n, &regulator_ena_gpio_list, list) {
		if (pin->gpiod == rdev->ena_pin->gpiod) {
			if (pin->request_count <= 1) {
				pin->request_count = 0;
				gpiod_put(pin->gpiod);
				list_del(&pin->list);
				kfree(pin);
				rdev->ena_pin = NULL;
				return;
			} else {
				pin->request_count--;
			}
		}
	}
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (StarChat-$\beta$)]
    The function \hl{dereferences \texttt{`rdev->ena\_pin`} after freeing it}, which is a use after free. This can lead to memory corruption or other unexpected behavior.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/understanding-integer-math-2.tex <==
% mixtral 41/nvul
% mixtral 21/nvul
% llama2 23/vul
% Finally, gpt-4 21/nvul

\begin{figure}[htbp]
    \centering
    \caption{Example of Incorrect Understanding of \textit{Integer Math}.} \label{fig:integer-math-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 21/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={9},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
void AllocateDataSet(cmsIT8* it8) {
  TABLE* t = GetTable(it8);
  if (t -> Data) return;  // Already allocated
  t-> nSamples = atoi(cmsIT8GetProperty(it8, "NUMBER_OF_FIELDS"));
  t-> nPatches = atoi(cmsIT8GetProperty(it8, "NUMBER_OF_SETS"));
  if (t -> nSamples < 0 || t->nSamples > 0x7ffe || t->nPatches < 0 || t->nPatches > 0x7ffe)
    SynError(it8, "AllocateDataSet: too much data");
  else {
    t->Data = (char**)AllocChunk(it8, ((cmsUInt32Number)t->nSamples + 1) * ((cmsUInt32Number)t->nPatches + 1) * sizeof(char*));
    if (t->Data == NULL) {
      SynError(it8, "AllocateDataSet: Unable to allocate data array");
    }
  }
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (GPT-4)]
\small{
Both \texttt{t->nSamples} and \texttt{t->nPatches} are user-controlled and can be large. When these values are incremented by 1 and then multiplied by each other and further multiplied by \texttt{sizeof(char*)}, \hl{the result can overflow a 32-bit integer if the values are sufficiently large}...
% This is especially true if \texttt{sizeof(char*)} is 4 or 8 bytes (depending on the architecture), which increases the multiplication factor.
}

\small{
Before performing the allocation, the function checks if \texttt{nSamples} and \texttt{nSamples} are within a certain range (\texttt{0} to \texttt{0x7ffe}). However, this check does not prevent overflow. For example, \hl{values close to the upper limit can still cause the multiplication result to wrap around}, leading to a smaller allocation than required.
}
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/understanding-integer-math.tex <==
\begin{figure}[htbp]
    \centering
    \caption{Example of Incorrect Understanding of \textit{Integer Math}.} \label{fig:integer-math-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 5/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={4},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
long WebPImage::getHeaderOffset(byte* data, long data_size, byte* header, long header_size) {
  if (data_size < header_size) { return -1; }
  long pos = -1;
  for (long i=0; i < data_size - header_size; i++) {
    if (memcmp(header, &data[i], header_size) == 0) {
      pos = i;
      break;
    }
  }
  return pos;
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (LLAMA 2)]
The issue is that the comparison loop can cause an integer overflow if the \texttt{data\_size} is large and the \texttt{header\_size} is small\ldots
% This can happen because the loop iterates \texttt{data\_size}-\texttt{header\_size} times, which can result in a large number of iterations if \texttt{data\_size} is large.

For example, \hl{if \texttt{data\_size} is 1000 and \texttt{header\_size} is 10, the loop will iterate 900 times (1000 - 10). This can cause an integer overflow} if the loop counter is not properly initialized or if it is not properly checked for overflow.
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/error-examples/understanding-missing-check.tex <==
\begin{figure}[t]
    \centering
    % \benjamin{Give more detail. Show what percentage of examples this shows up. Maybe more simple code. How many involves while or if statements?}
    \caption{Example of \textit{Missing Bounds/NULL Check}.} \label{fig:bounds-check-example}
    \begin{tcolorbox}[title=\textbf{Source code} (Example 4/non-vulnerable),colframe=Periwinkle]
    \begin{minted}
    [
    frame=lines,
    numbersep=2mm,
    breaklines=true,
    fontsize=\footnotesize,
    highlightlines={2,5},
    highlightcolor=yellow,
    linenos,
    tabsize=2,
    ]
    {c}
static int changedline (const Proto *p, int oldpc, int newpc) {
  if (p->lineinfo == NULL)  /* no debug information? */
    return 0;
  while (oldpc++ < newpc) {
    if (p->lineinfo[oldpc]!= 0)
      return (luaG_getfuncline(p, oldpc - 1)!= luaG_getfuncline(p, newpc));
  }
  return 0;  /* no line changes between positions */
}
    \end{minted}
    \end{tcolorbox}
    \begin{tcolorbox}[title=\textbf{Model response} (StarChat-$\beta$)]
    \small{The function \hl{dereferences the \texttt{`p->lineinfo`} pointer without checking if it is null}. This can cause a crash or other unexpected behavior if the pointer is null\ldots}
    \end{tcolorbox}
\end{figure}

==> _OldVersion.ICSE25/Figures/performance-eval/best-prompt-distribution.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.65\linewidth}
    \includegraphics[width=\linewidth]{Images/performance-eval/best-prompt-pie.png}
    \end{minipage}
    \begin{minipage}{0.3\linewidth}
        \centering
        \begin{tabular}[c]{l}
            \mbox{\cblock{31}{119}{180} Basic} \\
            \mbox{\cblock{255}{127}{14} In-context} \\
            \mbox{\cblock{148}{103}{189} CoT-SA} \\
            \mbox{\cblock{44}{160}{44} Embedding}
        \end{tabular}
    \end{minipage}
    \caption{Distribution of best-performing prompting methods.}
    \label{fig:best-prompts-distribution}
\end{figure}

==> _OldVersion.ICSE25/Figures/performance-eval/best-prompt-performance-unpaired.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tabular}{ccc}
        \mbox{\cblock{50}{116}{161} Balanced Accuracy} &
        \mbox{\cblock{225}{129}{44} Precision} &
        \mbox{\cblock{58}{146}{58} Recall}
    \end{tabular}
    \includegraphics[width=\linewidth]{Images/performance-eval/best-performance_unpaired.pdf}
    % \caption{\benjamin{TODO: Write up analysis of performance on unpaired data.
    % What if the conclusions (order of models, whether the models perform ``well'') are different?
    % Does this weaken our conclusions on the paired data?
    % }}
    \caption{Best-case performance of each model on the unpaired dataset. Bar length represents the mean of three random seeds, with error bars indicating one standard deviation. The prompt used for each model is displayed in parentheses.}
    \label{fig:model-performance-unpaired}
\end{figure}

==> _OldVersion.ICSE25/Figures/performance-eval/best-prompt-performance.tex <==
\begin{figure*}[t]
    \centering
    \small{
    Metric\\
    \begin{tabular}{cccc}
        \mbox{\cblock{50}{116}{161} Balanced Accuracy} &
        \mbox{\cblock{225}{129}{44} Precision} &
        \mbox{\cblock{58}{146}{58} Recall} &
        \mbox{\sampleline{} Random-guess baseline}
    \end{tabular}
    }
    \newlength{\sizea}
    \setlength{\sizea}{0.498\textwidth}
    \newlength{\sizeb}
    \setlength{\sizeb}{\textwidth-\sizea}
    \begin{subfigure}{\sizea}
    \centering
    \includegraphics[width=\linewidth]{Images/performance-eval/best-performance.pdf}
    \caption{Performance on the paired dataset.}
    \label{fig:model-performance}
    \end{subfigure}%
    \begin{subfigure}{\sizeb}
    \centering
    \includegraphics[width=\linewidth]{Images/performance-eval/best-performance_random25.pdf}
    \caption{Performance on the unpaired dataset.}
    \label{fig:model-performance-unpaired}
    \end{subfigure}
    \caption{Best-case performance of each model. Bar length represents the mean of three random seeds, with error bars indicating one standard deviation. The prompt used for each model is displayed in parentheses.
    % \benjamin{TODO: Reduce width, increase font size}
    }
\end{figure*}


==> _OldVersion.ICSE25/Figures/performance-eval/best-prompts-unpaired.tex <==
\begin{figure*}[t]
    \centering
    \small{
    Prompting method\\
    \begin{tabular}{llllll}
        \mbox{\cblock{50}{116}{161} Basic} &
        \mbox{\cblock{225}{129}{44} IC-Random} & 
        \mbox{\cblock{58}{146}{58} IC-Embedding} & 
        \mbox{\cblock{192}{61}{62} CoT-CVE} & 
        \mbox{\cblock{147}{114}{178} CoT-SA} & 
        \mbox{\sampleline{} Random-guess baseline} \\
        &\multicolumn{4}{c}{(Best out of the contrastive and non-contrastive versions)}
    \end{tabular}
    }
    \includegraphics[width=0.95\linewidth]{Images/performance-eval/best-prompt_random25.pdf}
    \caption{A comparison of different prompting methods for each model \newthree{on 50 \wei{unpaired} examples (unrelated in terms of bug fixes)}. Bar height shows the mean of three random seeds, with error bars indicating one standard deviation. %\wei{50 examples}
    % \benjamin{This is the unpaired dataset. TODO: write it up}
    }
    \label{fig:best-prompts-unpaired}
\end{figure*}

==> _OldVersion.ICSE25/Figures/performance-eval/best-prompts.tex <==
\begin{figure*}[b]
    \centering
    \small{
    Prompting method\\
    \begin{tabular}{llllll}
        \mbox{\cblock{50}{116}{161} Basic} & 
        % \multicolumn{4}{@{}l@{}}{$\underbrace{\mbox{\cblock{225}{129}{44} IC-Random} \mbox{\cblock{58}{146}{58} IC-Embedding} \mbox{\cblock{192}{61}{62} CoT-CVE} \mbox{\cblock{147}{114}{178} CoT-SA}}_{\text{Best out of the contrastive and non-contrastive versions}}$} &
        \mbox{\cblock{225}{129}{44} IC-Random} & 
        \mbox{\cblock{58}{146}{58} IC-Embedding} & 
        \mbox{\cblock{192}{61}{62} CoT-CVE} & 
        \mbox{\cblock{147}{114}{178} CoT-SA} & 
        \mbox{\sampleline{} Random-guess baseline} \\
        &\multicolumn{4}{c}{(Best out of the contrastive and non-contrastive versions)}
    \end{tabular}
    }
    \includegraphics[width=0.95\linewidth]{Images/performance-eval/best-prompt.pdf}
    % \includepdf[pages=1]{Images/performance-eval/best-prompt.pdf}

    % \begin{minipage}{0.72\linewidth}
    % \centering
    % \includegraphics[width=\linewidth]{Images/performance-eval/best-prompt.png}
    % \end{minipage}
    % % 
    % \begin{minipage}{0.25\linewidth}
    % \centering
    % \includegraphics[width=\linewidth]{Images/performance-eval/best-prompt-pie.png}
    % % Need vertical space...
    
    % \ 

    % \ 

    % \ 

    % \ 
    % \end{minipage}
    
    \caption{A comparison of different prompting methods for each model \newthree{on 50 buggy and fixed pairs \wei{(100 examples)}}. Bar height shows the mean of three random seeds, with error bars indicating one standard deviation. %\wei{50 pairs}
    % \benjamin{TODO:
    % Run remaining seeds for subpar GPT-4 prompts.
    % Add x axis grid lines.
    % Make random baseline easier to see.
    % }
    % \benjamin{We evaluated the contrastive and non-contrastive approach for each in-context example selection method.}
    }
    \label{fig:best-prompts}
\end{figure*}

==> _OldVersion.ICSE25/Figures/performance-eval/cot-reasoning.tex <==
\begin{table*}[htbp]
    \centering    
    
\caption{Without reasoning questions/answers: total 12 examples (6 vul and 6 nonvul)}
\label{tab:reasoning}
\begin{tabular}{lrrrrrr}
\toprule
Model       & Correct \\
\midrule
GPT-3.5     & 5 \\
Code LLAMA  & 8 \\
WizardCoder & 6 \\
% \midrule
% Total & 12 \\
\bottomrule
\end{tabular}

\begin{minipage}{0.5\linewidth}
\caption{Model reasoning without corrections.}
\label{tab:reasoning}
\begin{tabular}{lrrrrrr}
\toprule
       & \multicolumn{4}{c}{Reasoning queries} &  \\ \cmidrule{2-5}
Model       & R1 & R2 & R3 & R4 & \makecell[r]{Correct} \\
\midrule
GPT-3.5     &  4  & 5  & 7  & 10 & 9  \\
Code LLAMA  &  2  & 2  & 6  & 6  & 10\\
WizardCoder &  5  & 5  & 8  & 6  & 3  \\
\bottomrule
\end{tabular}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\caption{Model reasoning with corrections.}
\label{tab:reasoning-correction}
\begin{tabular}{lrrrrrr}
\toprule
            & \multicolumn{4}{c}{Reasoning queries} &  \\ \cmidrule{2-5}
Model       & R1 & R2 & R3 & R4 & \makecell[r]{Correct} \\
\midrule
GPT-3.5     & 7  & 9  & 7  & 6  & {11} \\
Code LLAMA  & 6  & 12 & 8  & 6  & 6  \\
WizardCoder & 8  & 10 & 9  & 5  & {8}  \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table*}

==> _OldVersion.ICSE25/Figures/performance-eval/shots.tex <==
\begin{figure}[htbp]
    \centering
    % \includegraphics[width=0.5\textwidth]{Images/example-shots.png}
    \includegraphics[width=0.3\linewidth]{Images/plot-shots-llama.png}
    \includegraphics[width=0.3\linewidth]{Images/plot-shots-starchat.png}
    \includegraphics[width=0.3\linewidth]{Images/plot-shots-wizardcoder.png}
    \caption{Performance of 0 to 6 in-context examples.
    % \todo[inline]{WIP: waiting on the results of random strategy and other models}
    }
    \benjamin{TODO: Update this plot. It doesn't include the best-performing models.}
    \label{fig:shots}
\end{figure}

==> _OldVersion.ICSE25/Figures/setup/metrics.tex <==
\begin{table*}[b]
    \centering
    \caption{Comparing three performance metrics in different scenarios. Some values highlighted in \colorbox{pink}{red} indicate that Accuracy and F1 behave unintuitively for severely imbalanced scenarios.
    For example, Accuracy is the same at 50\% class-Accuracy as when all predictions are positive; F1 score for the extremely-balanced classifier is substantially higher than 50\% class-Accuracy.
    }
    \label{tab:imbalance}
    \begin{tabular}{lccccrrr}
    \toprule
    & \multicolumn{4}{c}{Model predictions} & \multicolumn{3}{c}{Consequent performance metrics} \\
    \cmidrule(r){2-5}\cmidrule(l){6-8}
    Scenario                                        & TP & TN & FP & FN & Accuracy & F1     & $Accuracy_{mean}$ \\
    \midrule
    Perfect                                     & 50 & 50 & 0  & 0  & 1.00        & 1.00 & 1.00      \\
    Slightly worse than perfect                 & 45 & 45 & 5  & 5  & 0.90      & 0.90 & 0.90     \\
    50\% class-Accuracy                     & 25 & 25 & 25 & 25 & 0.50      & 0.50 & 0.50      \\
    Slightly better than 50\% class-Accuracy & 30 & 25 & 20 & 25 & 0.55     & 0.57 & 0.55      \\
    Extremely imbalanced                                  & 50 & 0  & 50 & 0 & 0.50      & \colorbox{pink}{0.67} & 0.50      \\
    Slightly less imbalanced but still bad                    & 45 & 5  & 50  & 0 & \colorbox{pink}{0.50}      & \colorbox{pink}{0.64} & 0.45     \\
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table*}

==> _OldVersion.ICSE25/Sections/10.intro-old.tex <==
% \section{\wip{} Introduction}

\subsection{\wip{} Introduction (OLD)}

\benjamin{TODO: I will rewrite and expand the introduction}

Large language models (LLMs) perform well on applications such as code generation and chat assistant, but have not been thoroughly explored for vulnerability detection.
% 
\benjamin{Some of this will move to related work}
Several recent works have evaluated ChatGPT and a few other prominent models and studied various prompt engineering techniques for LLMs.
However, these studies exclude several prominent models which have demonstrated high performance on software engineering tasks and often do not evaluate the models using consistent and state-of-the-art benchmarks. Additionally, these studies do not incorporate prominent prompting techniques, including chain-of-thought~\cite{cot} and retrieval-augmented generation~\cite{rag}.
Thus, it is not well-known what is the best way to use LLMs for vulnerability detection and what their capabilities for prediction and reasoning are.

\benjamin{TODO: What are LLMs, what are coding assistants}

\benjamin{TODO: What is prompting}

\wei{research questions proofread}

\wei{In static analysis and human inspection, vulnerability detection requires code understanding and reasoning on top of it, also can use rules, does LLM memorize, using rules or perform code understanding/reasoning?}

We ran experiments to answer the following research questions:
\begin{itemize}
    \item \textbf{RQ1:} What are the most successful and least successful prompt designs for LLM-based vulnerability detection?
    \item \textbf{RQ2:} How well do state-of-the-art LLMs perform on vulnerability detection?
    %Do LLMs memorize the open-source vulnerabilities in the vulnerability dataset?
    % \item \textbf{RQ3:} Can LLMs reason about root causes of vulnerabilities in a conversational setting? Furthermore, does this improve the model's predictions?
    \item \textbf{RQ3:} What kinds of errors do LLMs make when explaining the vulnerabilities?
    % On what kinds of programs are LLMs prone to errors?
    % \item \textbf{RQ5:} What error patterns commonly occur in LLM predictions? On what kinds of programs did LLMs commonly make errors?
    \item \textbf{RQ4:} How do LLMs compare to human developers for localizing vulnerabilities?
    % \item How well do the SOTA LLMs perform along other metrics than performance (robustness and out-of-distribution generalization)?
    %\item Do LLMs memorize the open-source vulnerabilities in vulnerability datasets? How does this impact the quality of their predictions on novel data?
    \item \benjamin{TODO: Add RQs for additional experiments: paired examples, dbgbench comparison, etc.}
\end{itemize}

We conducted thorough investigation on the research questions by developing \textcolor{red}{XX} prompts, including \textcolor{red}{XX} new prompting techniques, evaluating \textcolor{red}{11} SOTA LLMs, designing a comprehensive error categorization, and manually analyzing the outputs of \textcolor{red}{190} LLM outputs.

\wei{contributions proofread}

In this paper, we made the following contributions:
\begin{itemize}
    \item We designed new prompting methods for vulnerability detection. % Contrasting pairs, CoT-CVE, CoT-SA
    \item We conducted a comprehensive study to evaluate the capability of state-of-the-art LLMs for vulnerability detection.
    \item We designed experiments to further problem what models learned and did not learn, and provide insights and dataset for future vulnerability detection using LLMs.
        \begin{itemize}
        
        \item Do LLMs remember the vulnerabilities in the open source dataset? (memorize)
        \item Can LLM distinguish the buggy and patched pairs? (reasoning and code understanding)
        \item What types of errors LLM make when reasoning about vulnerabilities? (reasoning and code understanding)
        \item Do we observe them rules and templates of LLM when doing code understanding and vulnerability detection?
        \item How do LLMs compared to human developers when reasoning about vulnerabilities?
        \end{itemize}
    %\item We open sourced tool and dataset
  %  \item Analyzing the errors and fine-grained predictions contained in a large dataset of LLM-generated explanations.
  %  \item Evaluating LLMs' debugging abilities in comparison with humans on the DbgBench vulnerability benchmark.
\end{itemize}

There have been a few similar studies on LLM for vulnerability detection~\cite{}. To the best of our knowledge our work is different in that:

\begin{itemize}
\item we studied 100 bugs and 11 SOTA models, more than others
\item we studied the paired versions to show that the model cannot distinguish the two
\item we designed new prompting methods, some of the methods further pushed model performance
\item we positioned LLM performance in the context human diagnosis of vulnerability and compared dbgbench
\end{itemize}

% Old introduction from "writeup"
\begin{comment}
To explore the capabilities of these models, we studied the following research questions:
\begin{itemize}
\item How well can state-of-the-art LLMs perform on vulnerability detection?
\item What are the most successful and unsuccessful prompt designs for vulnerability detection?
% \item understanding and analysis of LLM capabilities 
\end{itemize}

\benjamin{TODO-NOW: Remove}
We also plan to study the following research questions in the future:
\begin{itemize}
\item Why do the LLMs sometimes fail to predict correctly? What error patterns occur in the LLM predictions?
\item Are large language models able to reason about vulnerabilities?
\item How well do the SOTA LLMs perform along other metrics than performance (robustness and out-of-distribution generalization)?
\item How do LLMs compare to human developers for prediction quality and reasoning? (using bug studies such as \citet{dbgbench})?
\end{itemize}

We expect to make the following contributions: 
\begin{enumerate}
\item Thoroughly evaluate the LLMs on vulnerability detection. Prior studies have not evaluated a \textbf{large set of LLMs} or evaluated them on \textbf{the same SOTA benchmarks}.
\item Explore the successful and unsuccessful prompting designs.
\item Compare the models with human predictions and reasoning.
\item Provide a benchmark suitable for integrating different prompts to evaluate and compare future large language models in a consistent way, evaluating not just performance, but also generalization and robustness.
\item Analyze errors and identify limitations of LLMs to inform future developments.
\end{enumerate}

We expect our study to have special impact and novelty because we evaluate a relatively large set of LLMs (prior studies evaluate ChatGPT alone or only a few popular chat assistants) and will evaluate them on  large benchmarks (rather than smaller, hand-gathered datasets).
\end{comment}

% Initial planning
\begin{comment}
\todo[inline]{TODO: Revise}

Links:

\begin{itemize}
    \item Code: \url{https://git.las.iastate.edu/llm-vuln/prompting}
\end{itemize}

We studied the following research questions:
\begin{itemize}
\item the capabilities of in-context learning (different prompting methods and their results)
\item understanding and analysis of LLM  capabilities 
\begin{itemize}
\item error patterns
\item successful and unsuccessful prompts
\item reasoning analysis
\end{itemize}
\end{itemize}

Expected contributions: 
\begin{enumerate}
\item What the best model can do (accuracy, generalization and robustness)? how it compare to human? is the LLM the SOTA for vulnerabilities? (static analysis, fuzzing, other models)
\item benchmarks 
\item future development of the model/short coming of the models: a list of errors and error analysis 
\item understand the reasoning behind LLM: why (somewhat) fails?
\end{enumerate}

Impact and novelty:
\begin{itemize}
\item large benchmark studies 
\item more comprehensive set of models 
\end{itemize}
\end{comment}


==> _OldVersion.ICSE25/Sections/10.intro.tex <==



\section{Introduction}
Contributions:
\begin{enumerate}
\item A comprehensive study
\item Prompt techniques that significantly improves the state of the art 
\end{enumerate}


Large Language Models (LLMs) have demonstrated impressive capabilities across various software engineering tasks, such as code generation~\cite{humaneval}, test generation~\cite{lemieux_testgen}, and code summarization~\cite{ahmed2024automatic}. Their versatile capabilities, along with their novel ability to explain their predictions in plain-text, make LLMs worthwhile subjects of investigation for detecting security vulnerabilities.
In static analysis and human inspection, vulnerability detection requires \wei{code understanding and reasoning}. Pattern-matching on code structures is insufficient to produce precise analyses~\cite{flawfinder,rats}, especially for real-world code. For example, to precisely detect a buffer overflow, we cannot only scan for {\tt strcpy} or {\tt malloc} statements. We need to identify the statements that update the strings and buffers, reason about the lengths of the strings after the changes at these statements, and also understand the bounds-check code to judge whether the protection is sufficient. 

LLMs have shown limited ability for complex reasoning~\cite{hooda_large_2024}\newtwo{, and a recent survey calls for more challenging tasks to evaluate their reasoning abilities~\cite{reasoning_survey}}; this calls into question whether LLMs possess the capabilities to perform effective vulnerability detection. This capability has profound implications for the potential applications of LLMs in other tasks \wei{\newthree{which require understanding and reasoning} about semantics of code, e.g., fault localization, program repairs, debugging and code generation for non-trival tasks}.  Studying LLMs for vulnerability detection also shed lights for the industry practitioners on whether LLMs can be considered as their software assurance tools. 

% \wei{need better summarize the SOTA}
Several studies have shown that LLMs struggle to attain high performance on vulnerability detection\newtwo{~\cite{fu2023chatgpt,ullah2023large,nong2024chainofthought,zhang2023prompt}}.
LLMs generally underperformed with basic prompts~\cite{fu2023chatgpt}, which motivated the use of in-context examples~\cite{ullah2023large}, chain-of-thoughts~\cite{nong2024chainofthought} and static analysis~\cite{zhang2023prompt}.
Prior studies primarily evaluate vulnerability detection performance. The very recent work (to the best of our knowledge, these papers are still in arXiv but not yet published) highlight broad errors in the models' vulnerability detection responses~\cite{yu2024security,nong2024chainofthought,sun2024llm4vuln,ullah2023large}, but do not comprehensively investigate the LLM errors from the perspective of detecting vulnerabilities.

Our studies, which are concurrently developed with these works, aim for (1) {\it comprehensiveness} --- \newtwo{we surveyed a wider variety of models and prompts in different scenarios of vulnerability detection, and analyzed more LLM responses with multiple raters, compared to prior work}; and
% (2) {\it usefulness} --- we not only studied whether models can report a ``Yes/No'' prediction, but also whether they can correctly report the types, locations and causes of a vulnerability, as such information is reported in static analysis-based vulnerability detectors used in industry~\cite{fbinfer,codeql,sonarqube}.
(2) {\it usefulness} --- \newthree{beyond evaluating ``Yes/No'' predictions, we studied whether LLMs can correctly report the types, locations and causes of a vulnerability, as done in industry-standard static analysis-based detectors~\cite{fbinfer,codeql,sonarqube}, and point out capabilities and code structures which LLMs struggled with, highlighting future research directions}.
In that regard, we also compared the capabilities of LLMs with human performance for understanding vulnerabilities.
% When analyzing errors of LLMs, we point out which capabilities of LLMs might be improved to help with vulnerability detection.
Specifically, we designed the following four questions to guide our research:
%Additionally, given the demonstrated errors, a comparison with humans on a complex debugging task~\cite{dbgbench} could also yield insights into LLM capabilities.

% Given that LLMs make predictions and elicit reasoning through a natural-language interface~\cite{cot,react}, a comparison with humans on a debugging task could yield insights into the strengths and weaknesses of LLMs.
%}

%We developed four research questions to guide our research on the capabilities of LLMs for vulnerability detection:

\begin{itemize}
    \item \textbf{RQ1:} What are the most successful and least successful prompt designs for LLM-based vulnerability detection?
    \item \textbf{RQ2:} How well do state-of-the-art LLMs perform on vulnerability detection?
    \item \textbf{RQ3:} What kinds of errors do LLMs make when explaining the vulnerabilities?
    \item \textbf{RQ4:} How do LLMs compare to human developers for localizing vulnerabilities?
\end{itemize}

To thoroughly investigate these RQs, we evaluated 11 SOTA LLMs using five distinct prompt templates, including developing three novel techniques for generating prompts. We systematically searched among the prompts to draw out the best performance from each model (\Cref{sec:rq1}). We investigated their empirical performance and their capability to distinguish buggy code from the corresponding fixed versions (\Cref{sec:rq2}).
% 
We rigorously analyzed 287 LLM responses explaining their vulnerability predictions and categorized them into 4 comprehensive error categories specifically tailored for vulnerability detection, revealing the ways in which the LLMs frequently failed and which code structures the models struggled with, as well as the effects of such errors on the models' explanation quality (\Cref{sec:rq3}).
% 
We evaluated the models' fault localization abilities on DbgBench, comparing their performance and difficulties with those of professional human software engineers to understand their similarities and differences (\Cref{sec:dbgbench}).

% \wei{you need to modify the sentences here or in the conclusions, so the two are different.}
\new{Our results show the following:
most models performed best with Basic and In-Context prompting. Our proposed CoT-SA and Contrastive Pairs, used with In-Context prompting, were beneficial for some models. 
LLMs performed within 0.5-0.63 Balanced Accuracy, close to a random-guess baseline, and failed to distinguish buggy and fixed versions of code in 76\% of cases on average.
57\% of LLM responses contained errors in \wei{{\it Code Understanding}, {\it Hallucination}, {\it Logic}, and/or {\it Commonsense Knowledge}, and among others,} LLMs especially struggled with correctly identifying bounds/null checks. Furthermore, LLMs frequently predicted erroneous location, type, or root cause of vulnerabilities, in spite of the correct binary label.
LLMs correctly located 6/27 bugs in DbgBench~\cite{dbgbench}, all of which were correctly diagnosed by at least one human. GPT-3 performed the best among all the models and correctly located 4/27 bugs.}

% \wei{
% (1) you need to summarize LLM studies at least for vulnerability detection with the proper citations,
% (2) typically we have a pargraph to summerize the results before listing the contributions,
% (3) clean up the pink}

% \begin{newenv}
% \benjamin{TODO: Finish writing after related work.}

\new{In summary, we make the following contributions:
\begin{itemize}
    \item We designed 3 new prompt templates for vulnerability detection, integrating information from bug-fixing patches, CVE descriptions, and static analyzers. % Contrasting pairs, CoT-CVE, CoT-SA
    \item We comprehensively evaluated the vulnerability detection capabilities of state-of-the-art LLMs, including testing them on pairs of buggy/fixed code.% and assessing their memorization of open source vulnerability data.
    % \begin{itemize}
    %     \item What types of errors LLM make when reasoning about vulnerabilities?
    %     \item Can LLM distinguish the buggy and patched pairs?
    %     % \item Do we observe them rules and templates of LLM when doing code understanding and vulnerability detection?
    %     % \item How do LLMs compared to human developers when reasoning about vulnerabilities?
    %     \item Do LLMs memorize the vulnerabilities in the open source dataset?
    % \end{itemize}
    \item We analyzed 287 LLM responses to break down the errors which LLMs made, and provide insights and a dataset for future research on vulnerability detection using LLMs.
   \item We evaluated LLMs' debugging abilities in comparison with humans on the DbgBench vulnerability benchmark.
\end{itemize}
}

\begin{comment}
\new{
\wei{we can remove the following and double check if any points missed in related work and in the paragraph before RQs in intro, added it there}
There have been a few similar studies on LLM for vulnerability detection~\cite{yu2024security,nong2024chainofthought,sun2024llm4vuln,ullah2023large}. To the best of our knowledge, our work is different from prior studies in that:
% 
\begin{itemize}
% \item We studied 100 bugs and 11 SOTA models, more than other studies~\cite{citation-needed}.
\item We studied the paired vulnerable and fixed versions of code to show that the model cannot distinguish the two.
\item We designed new in-context and CoT prompt templates tailored for vulnerability detection, some of which improved model performance.
% \item We analyze both incorrect and correct cases, looking for errors in reasoning.
\item We analyzed more models and used multiple raters to manually annotate a larger set of LLM responses.
\item We developed a more fine-grained error categorization and analyzed the code structures which LLMs had difficulty.
% \item We analyzed more responses with multiple humans than any other papers (287 compared to other papers: \cite{yu2024security} 82 responses, \cite{nong2024chainofthought} 100 responses, \cite{sun2024llm4vuln} 300 responses from one person then automatic using LLM, \cite{ullah2023large} fully-automatic handling).
% \item We analyzed more diverse models (11 compared to \cite{yu2024security} 3, \cite{nong2024chainofthought} 3, \cite{sun2024llm4vuln} 3, \cite{ullah2023large} 5).
% \item We analyzed code structures linked to problems, which is more detailed than other studies.
% \item We used more objective classification criteria, a more principled method to generate explanations, and a more rigorous agreement procedure, than other studies.
\item We positioned LLMs in a complex debugging context and compared them with human performance on DbgBench.
\end{itemize}
% \end{newenv}
}
\end{comment}

% First outline
\begin{comment}
\new{Large Language Models (LLMs) have shown novel capabilities for several tasks in software engineering, such as code generation, program repair, and code explanation.
This makes them worthwhile subjects of investigation for detecting security vulnerabilities.}

% strengthen our argument for the importance of this study by casting it as a concrete instance of the wider research into the reasoning capabilities of LLMs

% strengthen the importance of our work by making the case, here and in the introduction, that vulnerability detection is an important instance of a task that requires reasoning, not just pattern matching, so our finding have import for the wider question of whether and how well LLMs reason

\new{At the same time, it is not known whether they possess the capacity to reason about vulnerabilities.
In static analysis and human inspection, vulnerability detection requires code understanding and reasoning on top of it to logically prove vulnerabilities. It also can use rules. We want to know, do LLMs memorize, using rules, or perform code understanding/reasoning when doing vulnerability detection?
They have shown limited ability for complex reasoning in other tasks, cite...
The question of whether the models can reason about vulnerabilities is very important for applying LLMs to other tasks, such as localization, explaining vulnerabilities, repair, secure code generation...
It also is very important for understanding whether and how well LLMs reason when making predictions.}

\new{Previous studies have shown that LLMs struggle to attain good performance on LLMs.
However, these studies did not investigate prominent LLM prompting methods such as retrieval-augmented generation (embedding) and chain-of-thought with examples from real humans and static analyzer tools (emphasize that this is different from CFG/DFG since the explanations may be more directly useful to show the reasoning) \benjamin{@Rasel Can we claim these?} \rasel{ Are you talking about the explanation of vulnerability? Nong et al.\cite{nong2024chainofthought} makes an attempt I think. Could you please have a look at once on this paper?}
Additionally, these studies did not comprehensively investigate the reasons the models failed, thus are limited in terms of suggesting improvements for the model.
% 
Given that LLMs input and output through a natural-language text interface and their reasoning capabilities are generally elicited by speaking through this interface (cite cot, tot), it is also interesting to compare their performance with humans performing the same task, which is another thing previous studies have not done.}

\new{To investigate this open topic, we developed four research questions:
\begin{itemize}
    \item \textbf{RQ1:} What are the most successful and least successful prompt designs for LLM-based vulnerability detection?
    \item \textbf{RQ2:} How well do state-of-the-art LLMs perform on vulnerability detection?
    \item \textbf{RQ3:} What kinds of errors do LLMs make when explaining the vulnerabilities?
    \item \textbf{RQ4:} How do LLMs compare to human developers for localizing vulnerabilities?
\end{itemize}
}

\new{We conducted a thorough investigation on the research questions by developing 5 prompts, including 3 new prompting techniques and evaluating the performance of 11 SOTA LLMs, including evaluations on paired bugs and their fixes.
We rigorously analyzed 287 LLM responses explaining their vulnerability predictions and categorized them into 4 comprehensive error categories specifically tailored for vulnerability analysis, revealing the ways in which the LLMs frequently failed and which code structures the models struggled with, as well as the effects of such errors on the models' explanation quality.
We evaluated the models' fault localization abilities on DbgBench, comparing their results and performance with those of human software engineers to understand the similarities and differences.}

\begin{newenv}
\benjamin{Remove redundancy with RQs}
In this paper, we made the following contributions:
\begin{itemize}
    \item We designed 3 new prompt templates for vulnerability detection, integrating information from CVE descriptions, bug-fixing patches, and static analyzers. % Contrasting pairs, CoT-CVE, CoT-SA
    \item We conducted a comprehensive study to evaluate the capability of state-of-the-art LLMs for vulnerability detection.
    \item We designed experiments to further problem what models learned and did not learn, and provide insights and dataset for future vulnerability detection using LLMs.
    \begin{itemize}
        \item Do LLMs remember the vulnerabilities in the open source dataset? (memorize)
        \item Can LLM distinguish the buggy and patched pairs? (reasoning and code understanding)
        \item What types of errors LLM make when reasoning about vulnerabilities? (reasoning and code understanding)
        \item Do we observe them rules and templates of LLM when doing code understanding and vulnerability detection?
        \item How do LLMs compared to human developers when reasoning about vulnerabilities?
    \end{itemize}
   \item We evaluated LLMs' debugging abilities in comparison with humans on the DbgBench vulnerability benchmark.
    %\item We open sourced tool and dataset
  %  \item Analyzing the errors and fine-grained predictions contained in a large dataset of LLM-generated explanations.
\end{itemize}
\end{newenv}
\end{comment}


==> _OldVersion.ICSE25/Sections/20.study-setup.tex <==
\section{Study Setup}

\subsection{Dataset}
\label{sec:dataset}
% \begin{itemize}
% \item DiverseVul
% \item Synthetic vulnerabilities  
% \end{itemize}

We evaluated the models' vulnerability detection capabilities mainly using the SVEN dataset released by \citet{sven}. This dataset was collected from CVE records reporting real-world vulnerabilities from the CrossVul~\citep{crossvul}, BigVul~\citep{bigvul}, and VUDENC~\cite{vudenc} datasets.

% \input{Figures/setup/metrics}

SVEN is made of the source code of functions that were changed in vulnerability-fixing commits, where the version of the code before the commit is considered vulnerable and the version after the commit is considered non-vulnerable.
The authors curated the dataset by manually inspecting the commits based on their domain expertise to ensure that the data includes true security vulnerabilities/fixes and excludes data quality issues, including spurious commit message matches, tangled commits, and project-specific APIs.
Leveraging these labels, we focus on the \textit{binary classification} setting: given a prompt containing a function's source code, models predict whether the function belongs in the positive (vulnerable) or negative (non-vulnerable) class.


%Our pilot studies did not show any indication that the models had memorized the vulnerability labels (\S~\ref{sec:discussion}).}

% Previously 1,440??
The entire SVEN dataset comprises \new{846 C/C++} functions. We used 100 functions (50 pairs of a vulnerable function and its corresponding fixed version) to perform the study. This is because (1) many real-world functions are very long and do not fit the context window of the LLMs under study; (2) running LLM queries is very costly. It takes an average of 2 GPU-minutes per query, totaling 3.4 GPU-hours for 100 functions for each prompt method per model\newtwo{, and about \$180 of OpenAI credits in total}.  We studied a total of
11 models and for each model, we used 5 prompt methods
(§ III-A1). In addition, the models’ responses tended to vary when sampled multiple times. To address this variance, we ran the model inference 3 times with different random seeds and report the aggregated results. %We studied a total of 11 models and for each model, we used 5 prompt methods (\S~\ref{sec:prompt-design}). 

% \wei{we also used big vul and dbg, d2a (see details)}
% \benjamin{WIP}
\new{We also used the Big-Vul~\cite{bigvul} and D2A~\cite{d2a} datasets to source in-context examples and extra metadata to generate our prompts (see \Cref{sec:rq1}).
We used DbgBench~\cite{dbgbench} to compare the performances of LLMs and human for vulnerability detection (see  \Cref{sec:dbgbench}).}

%compared model performance with human performance on (see \S~\ref{sec:dbgbench}).}

%Conducting experiments on this dataset would incur higher costs, and many of the functions exceed the maximum context length of our chosen LLMs. In our experiments, we selected the shortest 50 examples, excluding a few examples with trivial or extremely-short code. Each example contains the vulnerable version of the function and its corresponding fixed version, totaling 100 functions.

% \todo{TODO: Add synthetic data}

\subsection{Models}
% \wei{Ben}

% \begin{itemize}
%     \item \url{https://docs.google.com/spreadsheets/d/1oImIIr-yWE0IqrqJe2Zv-zuoKelp0I\_DdYcCu02oUhU/edit?usp=sharing}
% \end{itemize}

We collected a list of large language models from two benchmark surveys~{\cite{zhao_survey_2023, liuAgentBenchEvaluatingLLMs2023}} as well as the highest-performing models from \citet{paperswithcode-humaneval}. We added several notable open-source models (e.g. StarCoder~\cite{starcoder}) and excluded the models for which inference was not available via API (e.g. Bard~\cite{bard}), not trained on source code (e.g. Pythia~\cite{pythia}), were trained only on distillations from ChatGPT (e.g. Vicuna~\cite{vicuna}), or were superseded by later iterations on the same project (e.g. LlaMA 1~\cite{llama1}).
% \rasel{As we are using both gpt3.5 and gpt 4, wont this line contradict?}
In \Cref{tab:humaneval}, we list 11 models used in our study, including the number of parameters (if it is an open source model), the length of the {\it context window}, i.e., the maximum number of input tokens, and HumanEval $Pass@1$ score~\cite{humaneval}, a metric that can somewhat reflect the models' capabilities in generating source code.  


% \benjamin{TODO: Link to extended page in data package \url{https://anonymous-llm-vulnerabilities.github.io/}}
% \url{https://docs.google.com/spreadsheets/d/1oImIIr-yWE0IqrqJe2Zv-zuoKelp0I\_DdYcCu02oUhU/edit?usp=sharing}




%The full list of models is available in our data package~\citep{data-package-figshare}.We evaluated the following prominent LLMs, which reported high code generation benchmark performance (see Table~\ref{tab:humaneval}). We list the name of each model along with the ID of the model checkpoint which we evaluated.
% \rasel{ When the reader reads the paper, what does he should understand from the right side of each of the contents? For example: "codellama/CodeLlama-34b-Instruct-hf". Those who works with the huggingface may know them very well, but those who does not work with api but only read papers, how do they know about these? Should we provide some information?}
% \begin{itemize}
%     \item Code LLAMA~\citep{codellama}: \texttt{codellama/CodeLlama-34b-Instruct-hf}
%     \item Gemini 1.0 Pro~\citep{gemini}: \texttt{gemini-pro}
%     \item GPT-3.5~\citep{gpt3.5}: \texttt{gpt-3.5-turbo-0613}
%     \item GPT-4~\citep{gpt4}: \texttt{gpt-4-0125-preview}
%     %\todo[inline]{TODO: Add \texttt{gpt-4} and \texttt{gpt-3.5-turbo}} \texttt{gpt-4-0613}
%     \item LLAMA 2~\citep{llama2}: \texttt{meta-llama/Llama-2-13b-chat-hf}
%     \item MagiCoder~\citep{magicoder}: \texttt{ise-uiuc/Magicoder-S-CL-7B}
%     \item Mistral~\citep{mistral}: \texttt{mistralai/Mistral-7B-Instruct-v0.1}
%     \item Mixtral of experts~\citep{mixtral} (to avoid confusion, we sometimes refer to Mixtral as Mixtral-MoE): \texttt{mistralai/Mixtral-8x7B-Instruct-v0.1}
%     \item StarChat-$\beta$~\citep{starchat} (a version of StarCoderBase~\citep{starcoder} which is fine-tuned for instruction-following): \texttt{HuggingFaceH4/starchat-beta}
%     \item StarCoder~\citep{starcoder} (with Anthropic's Tech Assistant prompt~\citep{starcoder-tech-assistant}): \texttt{bigcode/starcoder}
%     \item WizardCoder~\citep{wizardcoder}: \texttt{WizardLM/WizardCoder-15B-V1.0}
% \end{itemize}

\subsection{Implementation}
We wrote scripts to automatically query the models and parse the model output. For the open-source models, we used huggingface~\cite{huggingface_generation} local text generation APIs and wrote a custom prompting framework. For GPT-3.5, GPT-4, and Gemini, we used the APIs hosted by the corresponding organizations.
% \wei{We will open source these implementations for future reuse.}
\Cref{tab:parameters} shows the text generation parameters we used for the models.
We selected values of the models' hyperparameters intended to make their responses more deterministic, without sampling greedily (which can substantially reduce the performance).

\begin{table}[t]
\centering
\caption{11 models we studied, HumanEval $Pass@1$ is reported by \citet{paperswithcode-humaneval} or the source papers.}
% \benjamin{We ran LLAMA 2 13B since 70B doesn't fit. MagiCoder reported HumanEval+. Some others like Mixtral, MagiCoder and all parameter counts are reported outside ofthe leaderboard.}
% \benjamin{TODO: Note the model ID's we used.}
\label{tab:humaneval}
\begin{tabular}{lrrrrr}
\toprule
Model   & Parameters & Context Length& HumanEval              \\
\midrule
GPT-4~\citep{gpt4}       & - & 128k & 86.6 \\
Gemini 1.0 Pro~\citep{gemini} & - & 32k & 67.7 \\
WizardCoder~\citep{wizardcoder} & 15B & 2k                   & 57.3                 \\
Code LLAMA~\citep{codellama}  & 34B & 16k$\sim$100k                   & 48.8                    \\
GPT-3.5~\citep{gpt3.5}     & - & 4k & 48.1 \\
Mixtral-MoE~\citep{mixtral} & 45B & 8k$\sim$128k & 40.2 \\
Mistral~\citep{mistral} & 7B & 8k$\sim$128k & 30.5 \\
StarCoder~\citep{starcoder} & 15B & 8k & 30.4 \\
LLAMA 2~\citep{llama2} & 70B & 4k & 29.9 \\
StarChat-$\beta$~\citep{starchat} & 15B & 8k & - \\
MagiCoder~\citep{magicoder} & 7B & 16k$\sim$100k & - \\
% MagiCoder & 70B & 29.9 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
% \wei{missing starchat}
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{Text generation parameters we used.}
    \label{tab:parameters}
    \begin{tabular}{lccc}
    \toprule
         % & \multicolumn{3}{c}{API parameters} \\ \cmidrule{2-4}
        Parameter & HuggingFace & OpenAI & Google \\
    \midrule
        Top-$p$ & 0.9 & 1.0 & 1.0 \\
        Temperature & 0.1 & 0.1 & 0.1 \\
        Max. tokens generated & 512 & 512 & 512 \\
    \bottomrule
    \end{tabular}
\end{table}

% \new{StarCoder is the base model of StarChat-$\beta$.}
% For model survey Table
% \url{https://huggingface.co/blog/starcoder}
% \footnotetext[1]{StarCoder is the base model of StarChat-$\beta$ ~\cite{starchat}.}
% \footnotetext[2]{We used the next-largest 13B version of LLAMA 2 because we lacked the resources to run the 70B version.}
% % \footnotetext[2]{We used the next-largest 13B version of LLAMA 2 because we lacked the resources to run the 70B version.}
% % % For inference parameter table
% \footnotetext[3]{
% % \url{https://github.com/facebookresearch/codellama/blob/main/example\_completion.py\#L15}
% Code LLAMA's example scripts set \texttt{top\_p} to 0.9~\cite{codellama-temperature}. }
% \footnotetext[4]{OpenAI recommends to alter either temperature or 
% % \url{https://platform.openai.com/docs/api-reference/chat/create}
% \texttt{top\_p}, but not both, for their models~\cite{openai-temperature}.}
% \footnotetext[4]{OpenAI recommends to alter either temperature or \texttt{top\_p}, but not both, for their models. \url{https://platform.openai.com/docs/api-reference/chat/create}}
\new{The models generally replied with plain-text sentences. We developed a regular expression-based method to extract categorical yes/no responses; in cases where the models had no categorical response, we considered the prediction incorrect.
% Since the models replied in many different formats, some categorical responses can be extracted incorrectly;
In order to ensure the correctness of our extraction method, we selected 10\% of the responses for manual observation and found that our extraction procedure had an error rate of less than 0.5\%.}
\newthree{For future reuse, we open-source our code and document further implementation details in our data package~\citep{data-package-figshare}.}
% \wei{Make it clear the process is automatic and we parse using regex, point to data package.}
%The models' responses tended to vary greatly when sampled multiple times, due to non-determinism in both the sampling procedure and in the selection of examples for in-context learning. To address this variance, we ran the model inference 3 times with different random seeds and report the aggregated results.



\subsection{Metrics}
\label{sec:metrics}

% \benjamin{Need to figure out a way to present the metrics without rabbit trail}

We evaluated the models using the following four metrics: \textit{Accuracy}, the proportion of correct predictions on all examples, \textit{Precision}, the proportion of correct predictions out of the examples on which the model predicted positive (vulnerable), \textit{Recall}, the proportion of correct predictions out of the examples which are labeled positive (vulnerable), and \textit{Balanced Accuracy}, the mean of per-class accuracy for both positive and negative classes.

% \benjamin{Need to define accuracy, precision, recall somewhere}
 
\mycomment{
    \begin{equation*}
        \text{Accuracy} = \frac{correct}{examples} \quad
        \text{Precision} = \frac{correct_{positive}}{predicted_{positive}}
        \text{Recall} = \frac{correct_{positive}}{examples_{positive}} \quad
    \end{equation*}
}    
    \begin{equation*}     
        \text{BalancedAccuracy} = \frac{ \frac{correct_{negative}}{examples_{negative}} + \frac{correct_{positive}}{examples_{positive}} }{2}
    \end{equation*}
    
%\end{itemize}
% \rasel{As we are using MPCAccuracy in all the figures, can we use MPCAccuracy in the equation?}
\mycomment{
Much of the previous research on LLMs has used F1 score (a combination of Precision and Recall) to gauge overall model quality (e.g. \cite{fu2023chatgpt,nong2024chainofthought,zhang2023prompt}). However, 
}
\newtwo{We observed that LLMs often produce predictions that are highly imbalanced, such as labeling every example as ``vulnerable'' (see \wei{\Cref{sec:rq2}}), and that conventional metrics such as F1 and MCC tend to favor these severely-imbalanced classifiers (see our data package for details~\cite{data-package-figshare}).}
% 
% We observed that LLMs often produce predictions that are highly imbalanced, such as labeling every example as ``vulnerable'' (see \Cref{sec:rq2}).
% Accuracy and F1 tend to favor these severely-imbalanced classifiers.
% 
%\benjamin{Mention MCC, same result.}
% , including giving the same or higher score to a hypothetical model with a 90\% error rate on non-vulnerable examples, as to a model with 50\% error rate on both classes.
We argue that an imbalanced classifier that pathologically predicts only one class is less desirable than one that demonstrates some ability to differentiate between classes. In order to reflect this, {we primarily used Balanced Accuracy~\cite{brodersen_balanced_2010} to compare model performance}.

% \mycomment{
% \subsection{Research questions and experiment design}
% \wei{wei+ben+rasel+all}
% Reading study of LLM (SE)

% Thoughts for designing the study

% \begin{itemize}
%     \item threats should we avoid
%     \item research questions we can borrow
%     \item study methods and result presentation 
% \end{itemize}

% \benjamin{Wrote my thoughts about several papers in the related works section}

% \subsubsection{Initial probe}
% \wei{Ben, Roy, Sanjida, Rasel}
% Two types of data 
% \begin{enumerate}
% \item from existing benchmark
% \item newly generated data (synthetic)
% \end{enumerate}

% Two types of vulnerability 
% \begin{itemize}
% \item buffer overflow
% \item memory leak
% \end{itemize}

% Prompting engineering 
% \begin{itemize}
%  \item 0-zero shot 
%  \item 0-zero shot with NLP description
%  \item 3-shot
%  \item n-shot
%  \item n-shot chain of thoughts: examplar reasoning
%  \item step by step 
%  \item interactions
% \end{itemize}

% Prompt to understand the reasoning of the model, can the model understand the root cause of the memory leak

% delivery: summary results, interesting examples
% }


==> _OldVersion.ICSE25/Sections/30.performance-eval.tex <==
% \newpage

\section{Study Designs and Results of RQs}

\input{Figures/performance-eval/best-prompts}

\input{Figures/performance-eval/best-prompts-unpaired}

\subsection{RQ1: What are the most successful and least successful prompt designs for LLM-based vulnerability detection?}
\label{sec:rq1}

\input{Sections/31.prompting-methods}

\subsubsection{RQ1 Results} 
% \wei{need to clean up the messages, shorten the paragraph if needed}
\Cref{fig:best-prompts} shows the performance of all prompting methods over 3 random seeds, compared to a hypothetical random-guess baseline. The x-axis shows the models, and the y-axis reported the performance using the metric of Balanced Accuracy. Our results show that the Basic and IC-Random prompting methods achieve the best. As summarized on the pie chart on the right in \Cref{fig:best-prompts}, the two methods (the blue and the orange colored parts) each ranked the best for 4 out of 11 models.
% \wei{
We designed different approaches to select examples used for in-context learning; our results show no single approach fits all models.
% }
The IC-Embedding prompting ranked the best for 2 models and CoT-SA ranked the best for 1.

Q/A and CWE-list substantially improved the performance of Basic queries for 8 out of 11 models.
Additionally, IC-Embedding and CoT-SA techniques were beneficial for some models; IC-Embedding slightly outperformed IC-Random on LLAMA 2 and GPT-4, while CoT-SA substantially outperformed other approaches on average on MagiCoder.
\newthree{Contrastive Pairs performed better than non-contrastive settings in 45\% of cases.
% Surprisingly, CoT-CVE and Contrastive pairs did not perform very well, with CoT-CVE performing worse than the random baseline on 6 out of 11 models, and Contrastive Pairs underperforming standard prompts for 60\% of cases.
% Our results indicate that additional bug information can be useful but not always.
Surprisingly, CoT-CVE did not perform very well, with CoT-CVE performing worse than the random baseline on 6 out of 11 models.
Our results indicate that additional bug information can be useful but not always.}
\wei{This may be due to irrelevant context~\cite{distractibility} (e.g. the bug report contains information irrelevant to code like versions of programs) and is corroborated by \citet{sun2024llm4vuln}.}
Future work could explore alternative information such as bug reports and bug-fixing commits and different prompting methods that use the bug information.

\newthree{
We evaluated the models on a dataset containing pairs of vulnerable and fixed programs.
This represents a use-case such as using LLMs to detect vulnerabilities, and then checking again for the vulnerability after applying a bug-fixing patch.
While this aspect is shared with other benchmarks based on bug reports, like Big-Vul~\cite{bigvul} and CVEFixes~\cite{cvefixes}, it may not represent all settings of vulnerablity detection.
To represent an alternative scenario of scanning new procedures for vulnerabilities, we also plotted results on a random sample of 25 vulnerable and 25 non-vulnerable functions from our dataset that were unrelated in terms of bug fixes.
\Cref{fig:best-prompts-unpaired} shows that Basic, IC-Random and IC-Embedding were still the best prompting methods for the models, improving 5, 3, and 2 models respectively.
On these unpaired data, Contrastive Pairs performed better than non-contrastive settings 73\% of the time. 
The varying results across settings indicate that different scenarios may benefit from different prompts.
}
%and was the best prompt for 4 out of 6 models which performed best with in-context prompts.

\begin{summarybox}
\textbf{Summary for RQ1:}
\newthree{Across two vulnerability detection settings,}
% \wei{we need to revise this}
% The best-performing prompting methods varied by model; most models performed best with Basic, followed by In-context Random.
Basic or IC-Random prompts performed the best for 7-8 models.
%the majority of the 
% \new{Q/A and CWE-list were useful for improving model performance.
% IC-Embedding and CoT-SA \newtwo{performed best for 3  models}, while}
% \wei{change needed CoT-CVE and Contrastive Pairs were not as useful as we expected}.
\newthree{Integrating Q/A and CWE-list were useful for improving model performance.
IC-Embedding and CoT-SA performed best for 3-4 models. Contrastive Pairs were useful for predicting unpaired data.}
\end{summarybox}

\input{Figures/performance-eval/best-prompt-performance}

\subsection{RQ2: How well do state-of-the-art LLMs perform on vulnerability detection?}
\label{sec:rq2}
%Do LLMs memorize the open-source vulnerabilities in the vulnerability dataset?}

To explore the capabilities of LLMs for vulnerability detection, we compared the performance of the best prompting method for each model over 3 random seeds, shown in \Cref{fig:model-performance}. The best-performing model, StarChat-$\beta$, reported 0.56 Balanced Accuracy, showing that the current SOTA LLMs were not able to perform well for vulnerability detection. The performance of the models ranged from 0.56 to 0.50, close to that of random guessing. We observe that the model face challenges of distinguishing non-vulnerable and vulnerable versions, and 7 out of 11 models made 75\% or more predictions on the same class. Some models are severely biased towards one label, e.g., Mistral mostly predicts non-vulnerable\newtwo{, with only three exceptions}.
% \wei{we need an unbiased data plot?}
% \benjamin{TODO: Address \Cref{fig:model-performance-unpaired}}

% \input{Figures/performance-eval/best-prompt-performance-unpaired}


Compared to the HumanEval performance showed in \Cref{tab:humaneval},
we see that high code generation performance did not imply high vulnerability detection performance.
Despite their high code generation performance measured on HumanEval, WizardCoder, Code LLAMA, and Gemini performed poorly on vulnerability detection; while StarChat-$\beta$, StarCoder, and MagiCoder performed relatively better. These results indicate that effective vulnerability detection may require models to possess skills beyond code generation an it's not that the bigger models always perform better (StarChat-$\beta$, StarCoder, and MagiCoder only contain 7B parameters as shown in \Cref{tab:humaneval}).
GPT-4 and Mixtral-MoE maintained similar rankings in both tasks, displaying versatility across different contexts.


% \benjamin{WIP: discuss unpaired dataset.}
\mycomment{
We evaluated the models on a dataset containing pairs of vulnerable and fixed programs.
This represents a use-case such as using LLMs to detect vulnerabilities, then check again for the vulnerability after applying a bug-fixing patch.
% This may represent a specific use-case, such as using LLMs to detect bugs and check the fixes.
While this aspect is shared with other benchmarks based on bug reports, like Big-Vul~\cite{bigvul} and CVEFixes~\cite{cvefixes}, it may not represent all settings.
% To simulate a different setting of scanning a set of unrelated procedures for bugs,
To represent an alternative scenario, we also plotted results on a random sample of 25 vulnerable and 25 non-vulnerable functions from our dataset that were unrelated in terms of bug fixes.
This may simulate the use-case of scanning a set of unrelated procedures for vulnerabilities.
\Cref{fig:model-performance-unpaired} shows that in this scenario, the models' performance still ranged close to the random-guess baseline -- \wei{from 0.5 to 0.56 Balanced Accuracy.}
% Notably, more models performed better on the unpaired data with Basic prompts and with contrastive pairs.
These results underscore the conclusion that SOTA LLMs were not able to perform well for vulnerability detection.
% Several models, such as LLAMA 2 and Code LLAMA, performed better on the unpaired data, while other models, such as StarCoder and StarChat-$\beta$, performed worse.
}

% \wei{proofread
\Cref{tab:pair-performance} presents a further analysis on the models' capabilities of distinguishing pairs of vulnerable and nonvulnerable code. In the table, under Column {\it Can't Distinguish}, we show that on average, 76\% of pairs cannot be distinguished. Under {\it Both Correct} and {\it Both Wrong} columns, our results indicate that the models can predict both versions correctly in some instances (16\% of pairs), but there are also cases (8\% of pairs) where the models can predict both versions incorrectly. 
% }

\wei{Similar to the \newthree{scenario} in \Cref{fig:best-prompts-unpaired}, \Cref{fig:model-performance-unpaired} plots model performance on 50 unpaired examples. We see that performance improved slightly, but still ranged close to the random-guess baseline -- \wei{from 0.5 to 0.63} Balanced Accuracy. The models ranked differently for the two settings of vulnerability detection.
\newthree{In \Cref{fig:model-performance-unpaired}, the unpaired setting, GPT-4 performed the best.}}
% \benjamin{We can mention here that Contrastive performed best for 4/6 in-context methods in Figure 3b, which is surprising compared to 3a.}}


\newcommand{\myspace}{\hspace{4pt}}
\begin{table}[t]
    \centering
    \caption{Further analysis on 50 pairs of vulnerable and non-vulnerable examples. Cell values display the number and percentage of pairs in each category
    % \benjamin{TODO: Replace GPT-3.5 line.}
    }
    \label{tab:pair-performance}
    \begin{tabular}{lrrr}
    \toprule
        Model & Can't Distinguish & Both Correct & Both Wrong \\
       \midrule
        StarChat-Beta & 24 (48\%) & 18 (36\%) & 8 (16\%) \\
        GPT-4 & 36 (72\%) & 9 (18\%) & 5  (10\%)\\
        StarCoder & 35 (70\%) & 10 (20\%) & 5 (10\%) \\
        Mixtral-MoE & 36 (72\%) & 10 (20\%) & 4 \myspace(8\%) \\
        MagiCoder & 42 (84\%) & 6 (12\%) & 2 \myspace(4\%) \\
        GPT-3.5 & 40 (80\%) & 7 (14\%) & 3 \myspace(6\%) \\
        LLAMA 2 & 41 (82\%) & 6 (12\%) & 3 \myspace(6\%) \\
        WizardCoder & 21 (42\%) & 17 (34\%) & 12 (24\%) \\
        Code LLAMA & 44 (88\%) & 5 (10\%) & 1 \myspace(2\%) \\
        Mistral & 47 (94\%) & 3 \myspace(6\%) & 0 \myspace(0\%) \\
        Gemini & 49 (98\%) & 1 \myspace(2\%) & 0 \myspace(0\%)\\
        \midrule
        Average & 38 (76\%) & 8 (16\%) & 4 \myspace(8\%) \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{summarybox}
\textbf{Summary for RQ2:}
% \wei{add some numbers in this conclusion}
% The best model performance was only slightly above the random-guess baseline of 0.5 Balanced Accuracy.
\new{The SOTA LLMs performed poorly at vulnerability detection, with Balanced Accuracy ranging from \wei{0.5 to 0.63}.
% The best-performing models were StarChat-$\beta$, GPT-4, StarCoder, and Mixtral-MoE.
% 
All models frequently failed to distinguish the buggy and fixed versions of programs --- in 76\% of cases on average.
}
% and most models biased towards one class.
% Models did not tend to memorize the SVEN dataset.
\end{summarybox}


==> _OldVersion.ICSE25/Sections/31.prompting-methods.tex <==

% \benjamin{Changelog 09/03/2024:
% \begin{itemize}
% \item Moved to paragraph format.
% \item Renamed AccuracyMean to Balanced Accuracy.
% \item Moved contrasting pairs to a low-key paragraph.
% \item Renamed In-context to IC-Random and Embedding to IC-Embedding to show that they're both in-context approaches.
% \item Revised RQ1 and RQ2 to make the messages clear.
% \end{itemize}
% New text is pink.}

\subsubsection{Prompting methods}\label{sec:prompt-design}
We used three existing prompting methods~\cite{liu_pre-train_2021}, including
{\it Basic (zero-shot) prompting}, {\it In-context ($n$-shot) prompting}, and {\it In-context prompting based on embedding similarity}. 
We also designed three new prompting methods, namely \textit{In-context prompting based on contrastive pair}, \textit{Chain-of-Thought from CVE descriptions}, and {\it Chain-of-Thought from static analysis}.

% \wei{Ben, please change the bullet style to paragraphs}

% \wei{Contrastive pair is our idea, now it is mixed with in-context learning}

%We designed several varied methods for generating prompts with the goal of exploring which designs were most and least successful for vulnerability detection.Starting from the most basic zero-shot prompting method, we added features intended to improve the model's performance by influencing its completions towards a specific format, disambiguating the query, or giving examples for in-context learning.

\lstset{
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
breakatwhitespace=false,
% postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
escapeinside={<@}{@>},
rulecolor=\color{black},
frame=single,
}
\newcommand{\KeywordColor}{gray}
\newcommand{\HintColor}{RoyalBlue}
\newcommand{\CompletionColor}{ForestGreen}

% \begin{table*}[]
%     \centering
%     \caption{Variations of zero-shot prompting.}
%     Prompt template:\\
%     \texttt{Query \\ Code \\ \textcolor{green}{Hint} \\ Model completion}\\
%     \begin{tabular}{c|c|c|c}
%         Basic & Q/A & CWE List & Single-type analysis \\
%         Is the following code vulnerable, Yes or No?. & & & &
%     \end{tabular}
%     \label{tab:zero-shot}
% \end{table*}

% \benjamin{This list will be condensed to make space for more error analysis examples.}
%We use the prompting methods from the literature: % references for cwe and question/answer and system and incontext and embedding available after related work is written 

% \todo[inline]{TODO: Add more details and emphasize our methods}

% https://tex.stackexchange.com/a/461533
% https://tex.stackexchange.com/a/96298
\begin{description}[leftmargin=0pt,style=unboxed]
\item [Basic (zero-shot) prompting:] 
\new{We first designed a system prompt to set the context: ``I want you to act as a vulnerability detection system'', and we explored a variety of natural language descriptions:}
(1) \textit{Basic query}: ``Is the following function buggy? Please answer Yes or No.'' (We also tried ``Is the following function vulnerable?"; however, our pilot study shows that it did not perform as well.)
(2) \textit{CWE list}: This prompt starts with ``Does the following function contain one of the following bug types?'', followed by a fixed list of bug types, e.g., ``CWE-190: Integer Overflow'';
(3) \textit{Q/A}: \new{Begin the query with ``Question:'' and begin the model's response with ``Answer:''. This conditions the model to respond in a question-answering mode.}

\item[In-context ($n$-shot) prompting:] Here, we provide examples of inputs and responses for in-context learning~\citep{gpt3}.
The in-context examples condition the model to reply in the same format as the example responses. The selection of in-context examples can impact the performance. \wei{We studied three settings: (1) randomly selected examples, (2) the examples that had similar embeddings to the query example, and (3) the examples from {\it contrastive pairs} (see below for details).}

%The inputs and responses can be formatted as \textit{separate messages} (user message 1, assistant response 1, user message 2, assistant response 2, \ldots) or as a \textit{single message}, where the in-context examples condition a single query to the model.

%\new{The selection of in-context examples can impact the performance; by default, we select examples randomly, but alternatively the following methods can be used.}

\item[In-context prompting based on embedding similarity:] Choose the in-context examples which are most similar to the code in the query, where ``similar'' is approximated by the vector proximity between code embeddings.
Examples which are closer in embedding space can be more relevant to the query code~\cite{rag}.
We surveyed several embedding models~\cite{reimers2019sentencebert,openai_embeddings,codebert} and chose CodeBERT~\cite{codebert} because it
\newtwo{performed best.} \wei{We searched the SVEN dataset (the 100 examples we used) for similar examples.}
% elicited the best performance.

\item[In-context prompting based on contrastive pairs:] 
We used \textit{contrasting pairs} by providing the vulnerable version of the code (before the bug-fixing commit) and the fixed version (after the commit) as in-context examples in the same prompt. Since these two versions of the source code differ primarily in the portion related to the bug-fix, \newtwo{we hoped that this prompt template would highlight} the cause of the bug and instruct the model to learn that the small differences in code can lead to different labels.

\item[In-context prompting based on CoT from CVE descriptions:]
We designed ``chain-of-thought'' prompts by providing intermediate reasoning steps which lead to the answer, inspired by \citet{cot}. We use in-context examples from the Big-Vul dataset~\citep{bigvul}, which includes the CVE bug reports. For vulnerable examples,  we used the default in-context query and provide the chain-of-thought response. To produce such response, we adapt the descriptions in these bug reports to describe how the bug manifests.
% https://nvd.nist.gov/vuln/detail/CVE-2013-6051
For example, CVE-2017-9211~\cite{CVE-2017-9211} describes the vulnerability, including the symptoms, attack surface, and variable involved:

\begin{flushleft}
% \small{{\tt The {bgp\_attr\_unknown} function in bgp\_attr.c in {Quagga~0.99.21} {does not properly initialize the {total} variable}, which allows remote attackers to cause a {denial of service} (bgpd crash) via a {crafted BGP update}}}.
\small{\texttt{The crypto\_skcipher\_init\_tfm function in crypto/skcipher.c in the Linux kernel through 4.11.2 relies on a setkey function that lacks a key-size check, which allows local users to cause a denial of service (NULL pointer dereference) via a crafted application.}}
% A NULL pointer dereference vulnerability in the function nfc_genl_deactivate_target() in net/nfc/netlink.c in the Linux kernel before 5.1.13 can be triggered by a malicious user-mode program that omits certain NFC attributes, leading to denial of service.
% \small{\texttt{The matchCurrentInput function inside lou\_translateString.c of Liblouis prior to 3.7 does not check the input string's length, allowing attackers to cause a denial of service (application crash via out-of-bounds read) by crafting an input file with certain translation dictionaries.}}
\end{flushleft}

\new{We use this description as the CoT response and  append ``Therefore, the example is buggy'' to complete the response.
For non-vulnerable examples, we provide the default in-context example query/response.}

\item[In-context prompting based on CoT from static analysis:] We also used the output buggy paths reported by static analysis tools to prepare the chains of thought prompt. The buggy path consists of a list of statements that can lead to the bug. We use in-context examples from the D2A dataset~\citep{d2a}, which lists buggy paths from the Infer static analyzer~\cite{fbinfer} for several open-source C++ projects.
%Buggy paths are sequences of logical steps that indicate potential execution path which may lead to bugs. 
\new{We convert the buggy paths to natural language descriptions and use them as the response. This is an example COT response for a buffer overflow vulnerability:}

% \noindent
\begin{flushleft}
\small{\texttt{%
1. A buffer buf of size 10 is {allocated} at line 1.\\
2. An index i is {initialized to a value} in the range [0, 100] at line 2.\\
3. The index {i is used to access buf} at line 3. 
{This may exceed the bounds of buf.}\\
}}
\end{flushleft}

\new{We append ``Therefore, the example is buggy'' to complete the response.
For non-vulnerable examples, we provide the default response.}

\end{description}

% \wei{Add examples of CoT prompts}

% %%%%%%%
% \begin{itemize}
    % \item Foo
    % \begin{itemize}
    %     \item \textbf{Basic query}: ``Is the following function buggy? Please answer Yes or No.''
    %     \item \textbf{System prompt}: Set the context of the model's outputs before asking the query -- ``I want you to act as a vulnerability detection system.''
    %     \item \textbf{CWE list}: Provide a fixed list of bug types -- ``Does the following function contain one of the following bug types?''
    %     \item \textbf{Q/A}: Condition the model for question-answering by providing the marker tokens ``Question:'' before the question and ``Answer:'' before the model's answer.
    % \end{itemize}
    
    % \item \textbf{$n$-shot (in-context) prompting}: Provide examples of inputs and responses for in-context learning~\citep{gpt3}.
    % % For vulnerable examples, we give the example response ``Yes, the function is buggy''; for non-vulnerable examples, we give the response ``No, the function is not buggy''.
    % The in-context examples condition the model to reply in the same format as the example responses.
    % The inputs and responses can be formatted as \textit{separate messages} (user message 1, assistant response 1, user message 2, assistant response 2, \ldots) or as a \textit{single message}, where the in-context examples condition a single query to the model.
    % \new{The selection of in-context examples can impact the performance; by default, we select examples randomly, but alternatively the following methods can be used.}
    % In these prompt templates, we provide several examples for in-context learning~\citep{gpt3}, selected from some dataset of functions labeled as vulnerable or non-vulnerable. For vulnerable examples, we give the example response ``Yes, the function is buggy''; for non-vulnerable examples, we give the response ``No, the function is not buggy''. The in-context examples condition the model to reply in the same format as the example responses.
    
    % Following \citet{gpt3}, the model's response is conditioned on a set of $n$ ``good examples'' of queries and responses, then we give the unseen code and sample the model's completion. The model should follow the same behavior as the examples, and it can even learn from the in-context examples.

%     \item \textbf{Embedding similarity search}: Choose the in-context examples which are most similar to the code in the query, where ``similar'' is approximated by the vector proximity between code embeddings.
%     % \rasel{can we rewrite the following line.} Similar examples can provide the model with examples which are more relevant to the query code\cite{lewis2021retrievalaugmented}.
%     Examples which are closer in embedding space can be more relevant to the query code~\cite{rag}.
%     We surveyed several embedding models~\cite{reimers2019sentencebert,openai_embeddings,codebert} and chose CodeBERT~\cite{codebert} because it elicited the best performance.
%     % We used CodeBERT~\cite{codebert} to generate the embeddings; in our early experiments, it performed the best compared to SentenceTransformers~\cite{reimers2019sentencebert} and OpenAI Babbage embeddings~\cite{openai_embeddings}.
    
%     % In these prompt templates, we choose the in-context examples by looking up labeled source code examples which are similar to the code in the query, rather than choosing randomly~\citep{rag}. This can provide the model with examples which are relevant to the query, or provide examples of correct predictions in the same conditions and structures where a bug could manifest.
%     % 
%     % There are many methods available to determine the ``similar'' examples~\cite{liu_rag}; we used vector similarity scores measured using neural network embeddings like SentenceTransformers, CodeBERT, and OpenAI embeddings.
%     % In-context examples can be chosen by selecting randomly from the dataset, or similarity search using SentenceTransformers embedding, CodeBERT embedding, or OpenAI Babbage embedding~\cite{rag}.
% \end{itemize}

% We introduce the following new prompting methods:

% \begin{itemize}
    % \item \textbf{Contrasting pairs}:
    % Provide in-context examples consisting of the vulnerable version of some code (before the bug-fixing commit) and the fixed version (after the commit).
    % % In these prompt templates, we provide in-context examples consisting of buggy code and its corresponding fix. These are available because the SVEN dataset is constructed from bug-fixing commits; we can take the version before the commit as the buggy version and the version after the commit as the fixed version.
    % Since these two versions of the source code differ primarily in the portion related to the bug-fix (excluding any extraneous changes), we expect the small differences to highlight the cause of the bug.

%     \item \textbf{Chain-of-Thought from CVE descriptions}:
%     Provide in-context example responses in a ``chain-of-thought'' format -- intermediate reasoning steps which lead to the answer, inspired by \citet{cot}. We use in-context examples from the Big-Vul dataset~\citep{bigvul}, which includes the CVE bug reports. We adapt the descriptions in these bug reports to describe how the bug manifests.
%     % In these prompt templates, we provide the model with responses which include a ``chain-of-thought'' -- intermediate reasoning steps which lead to the answer, inspired by \citet{cot}.
%     \begin{itemize}
%         \item For vulnerable examples, we use the default in-context query and provide the chain-of-thought response.
%         % obtained natural-language reasoning steps by adapting the descriptions annotated by CVE bug reports. These descriptions describe how the bug manifests.
%         % \item For non-vulnerable examples, we used the commit messages of bug-fixing commits, which are annotated in the dataset. These messages explain what the bug was and how it was fixed.
%         \item For non-vulnerable examples, provide the default in-context example query/response.
%     \end{itemize}
%     % These extra metadata are annotated in the Big-Vul dataset~\citep{bigvul}.
%     % We condition the model on several pairs of queries and our constructed chain-of-thought responses, causing the model to generate completions in the same format.

%     % The bgp_attr_unknown function in bgp_attr.c in Quagga 0.99.21 does not properly initialize the total variable, which allows remote attackers to cause a denial of service (bgpd crash) via a crafted BGP update.
    
%     % The examples from the BigVul~\citep{bigvul} dataset are annotated with natural-language descriptions which are filed with the CVE report. These descriptions explain how and where the bug manifests.
%     % We propose to adapt the descriptions as an example of reasoning through the bug and prompt the model using a chain-of-thought template so that it follows the same process.

%     % We will use in-context learning to make the model generate a chain-of-thought. The model will be conditioned on several pairs of source code and our constructed responses (in \textcolor{\HintColor}{blue}) with chain-of-thought reasoning, then will make a prediction for the unseen source code. Because its behavior is conditioned the examples, the model should follow our constructed responses.

% % \begin{figure*}[htbp]
% %     \centering
% %     \includegraphics[width=\linewidth]{Images/performance-by-model.png}
% %     \caption{Performance of the prompting methods grouped by model.}
% %     \label{fig:prompting-by-model}
% % \end{figure*}
    

    
    % \item \textbf{Chain-of-Thought from Static Analysis}: Provide chains of thought derived from error traces reported by static analysis tools.
    % % In these prompt templates, we provide chains of thought derived from error traces reported by static analysis tools.
    
    % Many static analysis warnings include \textit{error traces} -- lists of locations in the code along with conditions at each location which imply the bug conditions.
    % % The traces are a minimal set of reasoning steps provided ``for free'' when the analyzer is run.
    % % Many analyzers are expensive to run, but we can use examples from the D2A dataset~\citep{d2a}, which lists thousands of traces from several open-source C++ projects.
    % We use in-context examples from the D2A dataset~\citep{d2a}, which lists error traces from the Infer static analyzer~\cite{infer} for several open-source C++ projects.
    % % \rasel{Can we explicitly mention that  only the in-context/shot examples are from D2A but the final test examples are from SVEN dataset? Can we do that also for Chain-of-Thought from CVE descriptions}
    % % We condition the model on several pairs of queries and chains of thought constructed from static analyzer traces.
    % % We propose to convert these error traces to natural-language reasoning steps and prompt the model using a chain-of-thought template so that it will emulate the same reasoning process.
    
    % % \item \todo[inline]{Implemented ideas above; future ideas are listed below}
    % % \item Tool use:
    % % \begin{itemize}
    % %     \item Retrieve definition of function
    % %     \item Retrieve similar code
    % %     \item Check control/data dependency, perform alias or value analysis
    % % \end{itemize}
    % % \item Ensemble multiple prompts or models

%     \item In combination with any method for selecting in-context examples, we can use \textbf{Contrasting Pairs}.
%     These consist of the vulnerable version of the code (before the bug-fixing commit) and the fixed version (after the commit).
%     % Provide in-context examples consisting of the vulnerable version of some code (before the bug-fixing commit) and the fixed version (after the commit).
%     % In these prompt templates, we provide in-context examples consisting of buggy code and its corresponding fix. These are available because the SVEN dataset is constructed from bug-fixing commits; we can take the version before the commit as the buggy version and the version after the commit as the fixed version.
%     Since these two versions of the source code differ primarily in the portion related to the bug-fix, we expect the small differences to highlight the cause of the bug.
%     % \new{This can be combined with any method to select the in-context examples.}
    
% \end{itemize}

% \benjamin{This can be pared down later}


%, and during development we observed that different prompts could boost different models' performance, for example ``CWE list'' + ``Q/A'' + ``$n$-shot with CodeBERT embeddings and contrasting pairs''; however, it is not economical for us to explore all the combinations of different prompts. 
% \wei{please shorten and clean it}
% The above prompting techniques can be combined to create many possible prompts. In order to find a high-performing prompting method while limiting the search space, we first evaluated the Basic query in four ``modes'':
% The above prompts can be combined in many ways.
Considering the numerous ways the above prompting techniques can be combined, we systematically searched for high-performing prompts for each model.
For the basic prompting method, we evaluated four ``modes'' ---
(1) basic query, (2) Q/A, (3) CWE list, and (4) both Q/A and CWE list --- and designated the best-performing mode as the \textbf{Basic} prompting approach.

% Similarly, we evaluated four possibilities for each in-context prompting method:
% Similarly, we enumerated four settings for formatting in-context examples:
% (1) sending in-context examples as separate messages, (2) single message, (3) contrasting pairs with separate messages, and (4) contrasting pairs with single message.
% We evaluated these settings for each of the four in-context prompting methods: random selection \textbf{(IC-Random)}, embedding similarity search \textbf{(IC-Embedding)}, chain-of-thought from CVE descriptions \textbf{(CoT-CVE)}, and chain-of-thought from static analysis \textbf{(CoT-SA)}.
% , exploring a total of 20 (4 basic + 16 in-context prompts for each model).
\new{For the in-context prompting methods, we evaluated random selection \textbf{(IC-Random)}, embedding similarity search \textbf{(IC-Embedding)}, chain-of-thought from CVE descriptions \textbf{(CoT-CVE)}, and chain-of-thought from static analysis \textbf{(CoT-SA)}.
% We did a pilot study and found that performance generally improved with more shots. Thus, we used 6 in-context examples for all prompts because that is the maximum number of examples that fit within most models' context sizes.
\newtwo{We did a pilot study (\S~\ref{sec:discussion}) and found that 6 shots performed the best for most models and was the maximum number of examples that fit within most models' context sizes. Thus, we used 6 shots for all in-context prompts.}
For each approach, we used two configurations: \newtwo{(1) 6 randomly-selected examples as well as (2) 3 contrastive pairs}. We then selected the best outcome for each model and prompting method.}
We list examples of the prompts and more details in our data package~\cite{data-package-figshare}.
% \benjamin{TODO: Look up previous results, do we have evidence that this is the best-performing setting?}

% \benjamin{TODO-NOW: Explain detailed settings of our prompting implementation: find the best basic prompt, then apply to all in-context prompts. Chose 6 in-context examples as the most that fits within most models' context size. Chose dataset from MSR for CoT-CVE, D2A for CoT-SA.}


==> _OldVersion.ICSE25/Sections/32.shots.tex <==
\section{$n$-shot prompting - moved to appendix}

\input{Figures/performance-eval/shots}

\paragraph{Results: $n$-shot prompting \benjamin{Consider removing this section; very detailed, calls attention to threats, and not very interesting.}}
Figure \ref{fig:shots} displays the performance of the $n$-shot random and CoT strategies with 1, 2, \ldots, up to 6 examples in the prompt.
We did not try more than 6 examples yet because more examples can exceed the context limit of some of the models.

Considering Code LLAMA, for the $n$-shot random approach, the optimal number of examples was 3 rather than 6. We consistently used 6 examples when comparing with different approaches, but note that future evaluations may tune this parameter.
For both CoT approaches, the model's mean performance drops below the baseline of 0.5 $Accuracy_{Mean}$ when we use 3-5 examples, but increases above the 0-, 1-, and 2-shot performance when we use 6 examples.
StarChat-$\beta$ and WizardCoder had similar performance characteristics, though the \textit{random} strategy peaked at 5 examples for StarChat-$\beta$ and 2 examples for WizardCoder. StarChat also improved rather consistently as more examples were added, though CoT underperformed compared to 0-shot.

These results indicate that more examples were not always better, but can improve the model if enough examples are given. The CoT approaches performed worse than the 0-shot baseline; however, their performance may be improved by using more than 6 examples.
We believe the cause of the improvement may be because the model's behavior is highly dependent on the examples, and a small set of examples may produce highly biased behavior or may not be informative to the model.
%Therefore, we used 6 examples when comparing our few-shot prompting approaches with other

\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:} The optimal number of in-context examples varied depending on the model and prompting method.
CoT prompting always performed worse than 0-shot.
\end{mdframed}

==> _OldVersion.ICSE25/Sections/33.reasoning.tex <==
\section{CoT-Reasoning - moved to appendix}

\subsection{Prompting}

\begin{itemize}
\item \textbf{Chain-of-Thought from Conversations}: In these prompt templates, we interact with the model in a conversation to query its reasoning about the bug.

    We implemented a human-in-the-loop prototype of this approach for null-pointer dereference bugs, by asking the following questions in a single session:

    \begin{itemize}
        % \item \textbf{Q1}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
        % \item After the initial query, we ask follow-up questions to question the model's reasoning:
        \item \textbf{R1}: \textit{At which line, the pointer can be a NULL?}
        \item \textbf{R2}: \textit{Which pointer can be a NULL?}
        \item \textbf{R3}: \textit{At which lines the pointer is dereferenced?}
        \item \textbf{R4}: \textit{Can a NULL pointer `X' be dereferenced?} (where `X' is a placeholder for the variable which can potentially be a NULL pointer)
        % \item After reasoning about the bug, we query the model again about the vulnerability:
        \item \textbf{Q}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
    \end{itemize}

    The \textbf{Q} (for Query) question asks the model for a prediction about the bug.
    The \textbf{R} (for Reasoning) questions force the model to reason about the root causes of the bug.
    
    As our prototype requires a human to reason about the answers to the intermediate questions, it is difficult to scale. We plan to automate this prompt technique or provide the model with examples of the manually-crafted conversations to condition its response to reason about the bug in a similar way before predicting an answer.
\end{itemize}

\subsection{Results}

\input{Figures/performance-eval/cot-reasoning}

\begin{figure}[htbp]
    \centering
    \benjamin{TODO: Make this format different from the `Summary' boxes.}
    \caption{Reasoning queries}
    \begin{mdframed}[roundcorner=10pt]
        \label{fig:reasoning-queries}
        \begin{itemize}
            % \item \textbf{Q1/Q2}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
            \item \textbf{R1}: \textit{At which line, the pointer can be a NULL?}
            \item \textbf{R2}: \textit{Which pointer can be a NULL?}
            \item \textbf{R3}: \textit{At which lines the pointer is dereferenced?}
            \item \textbf{R4}: \textit{Can a NULL pointer `X' be dereferenced?}
        \end{itemize}
    \end{mdframed}
\end{figure}

\paragraph{RQ3 results: Can LLMs reason about root causes of vulnerabilities in a conversational setting?}
We asked the models the questions from the method \textbf{Chain-of-Thought from Conversations}, in order (listed in Figure \ref{fig:reasoning-queries}).
We evaluated three models (GPT-3.5, Code LLAMA, and WizardCoder) on a small test set of 12 examples, 6 vulnerable and 6 non-vulnerable.
Table \ref{tab:reasoning} shows the results of asking the queries to the model and the effects on the models' accuracy.
Table \ref{tab:reasoning-correction} shows the same results, but after each reasoning query (R1, R2, R3, R4), if the model's answer is incorrect, the user corrects it before proceeding.

Considering Table \ref{tab:reasoning}, queries R1 and R2, all models predicted incorrectly for more than half of the programs, indicating that they are lacking in reasoning ability about detecting which pointers can be NULL.
However, all models predicted half or more of the examples correctly for R3 and R4, showing that they have better reasoning ability about whether pointers are dereferenced (generally an easier task than detecting NULL pointer assignments, since it requires only syntactic analysis rather than value-flow analysis).

Interestingly, the models sometimes predicted reasoning queries incorrectly, even when the answers are available within the conversation (Table \ref{tab:reasoning-correction}). For example, the correction to R1 implies the answer to R2, and the correction to R3 implies the answer to R4, but sometimes the models predicted R2 and R4 incorrectly. This shows that model reasoning can fail even when the answers are immediately available in the conversation.  In future work, we will more thoroughly investigate the models' reasoning capabilities

After adding reasoning to the model, 4/6 of the settings produced a greater number of correct answers (column Q2 across both tables). For GPT-3.5, the increase in correct predictions for Q2 was larger when corrections were given than without corrections.
These results indicate that forcing the model to reason in a conversational setting can potentially improve the model's vulnerability detection abilities, and that the model can perform better when it can access correct reasoning..

However, WizardCoder regressed without corrections and Code LLAMA regressed with corrections, indicating that even with correct reasoning, models can ignore the context and still predict incorrectly.

\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:}
Reasoning queries boosted the models' accuracy in 4/6 settings.
\end{mdframed}


==> _OldVersion.ICSE25/Sections/40.error-analysis.tex <==
% \section{Analyzing LLM Outputs}
\subsection{RQ3: What types of errors do LLMs make when explaining vulnerabilities?}
\label{sec:rq3}

%We prompted the models to explain the reasoning for the examples where they predicted the code was vulnerable. 

\subsubsection{Study setup} For a vulnerability detection tool to be useful, we hope it can present further vulnerability information such as its cause, types and locations. \new{We prompted the LLMs to explain all predictions that they identified as vulnerable and analyzed their responses.
%that provided valid explanations for those identified vulnerabilities\newtwo{We analyzed both incorrect and correct predictions, since we are interested in understanding the errors which occurred even when the LLM's vulnerable/non-vulnerable prediction is correct.}
The prompt consists of three parts:}
(1) the original prompt described in \Cref{sec:rq1}\newtwo{, applying the best-case prompt for each model noted in \Cref{fig:model-performance}},
(2) the model's original prediction, e.g., ``Yes/No'' for basic prompts or ``Yes, the vulnerability is \textit{CWE-XXX: Description}'' for prompts with CWE information, and
(3) ``Please explain the reasoning for this answer''. We manually inspected the results and found that the models generally make four types of errors:

% 
% \wei{we need to add examples for each category}

% \wei{Expand to include the ``reasoning'' about values and such. Consider re-adding the integer math example.}
% \paragraph{\textit{Code understanding errors}} LLMs produce incorrect assertions about programming language semantics, code structures, or effects of statements.
\paragraph{\textit{Code understanding errors}} LLMs produce incorrect assertions about programming language semantics or code structures\newtwo{, including inferences about the effects of statements}.
% \new{
For instance, sometimes an LLM incorrectly claims that a pointer is accessed without being checked, when the code contains the check\newtwo{; sometimes an LLM claims an integer operation will overflow when, considering the size of the integer and possible values of the operation \wei{implied by the prior code context}, an overflow is impossible}.
% }
% wizardcoder 22/vul, return value of -1 is OK
% codellama 1/nvul, lock for a data structure which is named according to convention
% mistral 15/nvul, && and != are not defined
% llama2 19/nvul, string processing function does not modify the input string
% starchat 20/nvul, the data do not have to be checked when we're bailing out
\paragraph{\textit{Common knowledge errors}} LLMs make incorrect assumptions about the applications, environment, or code conventions.
% \wei{need a better example}
% \new{For example, the LLM may claim that the function call \texttt{readBytesExact(client, buf, sizeof(buf));} can overflow if the client provides too many bytes, when it is reasonable to assume that the function will read at most \texttt{sizeof(buf)} bytes.}
% \newtwo{For example, an LLM claimed that the use of the \texttt{!=} operator would cause an error because the operator was not defined in the function; since != is built-into the C language, this claim is unreasonable.}
\newtwo{For example, an LLM may claim that if a variable \texttt{N\_FDC} is negative, an error will occur. However, a developer could reasonably interpret the all-capitalized \texttt{N\_FDC} as a configuration variable representing the number of a certain resource (floppy-disk controllers), and assume it to be a non-negative integer by definition.}
% \wei{This example is a bit unclear. We can instead talk about a hypothetical example, like global variables in all caps or string length operation returning nonzero values.}
% \newtwo{For example, an LLM claimed that a buffer overflow would occur if a string-processing operation \texttt{CASE\_FOLD(..., \&p, pend, buf)} modified the input string, but the string-processing function seems to copy the result to a new buffer rather than modifying the input.}
\paragraph{\textit{Logic errors}} LLMs produce statements that are logically contradictory or make incorrect logical implications when reaching the conclusions of vulnerability.
\newthree{For example, sometimes an LLM correctly claims that a variable \texttt{x} is checked, then later contradicts itself by stating, ``since \texttt{x} \textit{is not checked}, it will overflow...''.}
% \new{
% For example, sometimes an LLM incorrectly says that when {\tt a} is a large negative number, the statement \texttt{if(a<b)} is likely evaluated to {\tt false}; however, it is likely evaluated to {\tt true}.\wei{better example?}
% }
\paragraph{\textit{Hallucination/Memorization/Repetition errors}} LLMs produce {\it hallucination} (stating information that sounds correct but is not present in the prompt, such as pointing out a potential integer overflow in an arithmetic operation that doesn't appear in the code), {\it memorization} (memorizing information from the training data),
% \wei{find a better example}
% \new{, such as claiming that the code occurs inside a bug benchmark and as a result is not vulnerable}
% \newtwo{(),}
and {\it repetition} (infinitely repeating  certain text sequences, for instance: ``1. The function is buggy because it is not checking for a null pointer. 2. The function is buggy because it is not checking for a null pointer. 3\ldots'').

% \wei{we should reduce the empirical study setup and move some content to appendix}
\input{Figures/error-analysis/categories}

\input{Figures/error-analysis/fine-grained-errors}

% \new{
We collected quantitative data by analyzing  a total of 287 eligible LLM responses to understand how often LLMs make such mistakes.
To mitigate subjectivity, we used independent ratings from three authors, similar to \citet{empiricalstudy-deeplearningbugs}.
% The lead author designed the error categories and conducted a training session.
% Then,
The raters independently identified the errors in the LLM responses, meeting to refine the protocol after processing \sfrac{1}{3}, \sfrac{1}{2}, and all of the data.
We measured inter-rater agreement using \textit{Fleiss' kappa ($\kappa$)~\cite{fleiss}}, ranging from -1 to 1 with higher values indicating more agreement.
%Initially, $\kappa$ was 0.25 (fair agreement), with 30\% of responses classified identically by all three raters.
We resolved disagreements by siding with the majority when two raters differed from the third, resulting in $\kappa=0.75$ with 83\% of responses classified identically. We then discussed the remaining disagreements until reaching a final categorization for each response.
% }

% \setcodecaption


% \input{Figures/error-examples/understanding-control-flow}

% \input{Figures/error-examples/understanding-integer-math}


\subsubsection{RQ3 Results}

\input{Figures/error-examples/understanding-missing-check}

\input{Figures/error-examples/understanding-integer-math-2}

\input{Figures/error-analysis/fine-grained-predictions}

% \wei{proofread the following}
\Cref{fig:error-categories} reports how often each type of error occurred in LLM responses. We found that LLMs were somewhat useful for explaining vulnerabilities as 43\% responses contain no errors. Improving Code Understanding will help LLMs to better explain vulnerabilities, as 41\% responses contained code understanding errors. \wei{Our results also demonstrate that LLMs still cannot perfectly solve reasoning problems, as some of the incorrect code understanding is due to not being able to
reason about the values across several statements, and there are 9\% Logic errors and 3\% Common Knowledge errors, which can affect the reasoning.} We  observed that LLMs tended towards Hallucination, Memorization, and Repetition (11\% of errors) during vulnerability detection.

In \Cref{tab:fine-grained}, we show the specific code structures that affected the correctness of the explanations as well as the fine-grained classifications for Logic errors and Hallucination/Memorization/Repetition errors. For example, out of 159 responses explaining bounds checks, 76 are incorrect. \Cref{fig:bounds-check-example} shows an example of a model response which flags an unchecked null-pointer dereference, presumably at line 5 (\texttt{p->lineinfo[oldpc]}), even though \texttt{p->lineinfo} is checked at line 2.
This error can lead to false positives, especially after the bug is fixed by adding a check.

% \wei{1. Bounds check is in the code. 2. Still uncertain whether it's the definition problem.}
\wei{\Cref{fig:integer-math-example} shows an example of an \textit{integer math} error.  From the model response,  the LLM correctly identified that there is a bounds-check at line~6 (it was in fact added by the developers to prevent overflows~\cite{CVE-2018-16435}). Given the upper bound of \texttt{0x7fff} for \newthree{\texttt{nSamples+1} and \texttt{nPatches+1}}, even the maximum values would not cause an overflow in an unsigned integer ($\texttt{0x7fff} * \texttt{0x7fff} * \texttt{8} = \texttt{0xfff80008}$) at line~9; however, the LLM \newthree{was} not able to understand and reason about such math.}
% \wei{fix line for Figure 6}

%flagged a potential integer overflow close to the upper bound of \texttt{0x7fff}, even accounting for the range check in line 7;however, even the maximum values would not cause an overflow in an unsigned integer ($\texttt{0x7fff} * \texttt{0x7fff} * \texttt{8} = \texttt{0xfff80008}$). In fact, the check in line 7 was added by the developers to prevent overflows~\cite{CVE-2018-16435}.}
% \footnote{\texttt{0x7fff * 0x7fff * 8 = 0xfff80008}; see \url{https://github.com/mm2/Little-CMS/commit/768f70ca405cd3159d990e962d54456773bb8cf8}}.}
% however, considering the capacity of an unsigned integer is \texttt{4,294,967,295} and the maximum value of the multiplication is \texttt{4,294,443,016}, the operation would not cause an overflow.
% \wei{is it code understanding error or cannot understand what is integer overflow?}

%a breakdown of specific errors, listing the count of responses containing each fine-grained error and, where applicable, the count of responses with related code structures.LLMs frequently produced reasoning errors, with 57\% of model outputs containing at least one error.
% A substantial portion (41\%) of responses exhibited \textit{Code Understanding} errors, including incorrect handling of bounds/NULL checks, pointers, memory allocation, and type mismatches.\textit{Hal/Mem/Rep} occurred in 9\% of responses, followed by \textit{Logic} at 7\%. Finally, 3\% of responses contained \textit{Common Knowledge} errors.

%The \textit{Code Understanding} errors indicate syntactic structures that were difficult for LLMs.LLMs frequently made \textit{Bounds/NULL check} errors, incorrectly claiming that an index or pointer was not checked before use and could lead to a buffer overflow or null-pointer dereference, even though the code contained the check. This error occurred in nearly half (48\%) of the responses to programs containing a check operation and represents an important challenge for LLMs, since almost every program in our dataset contained a check operation. 

%, despite these occurring in about half and one-tenth of the programs, respectively

%LLMs also made errors on 8\% of integer operations and 10\% of string operations.

% 
%In contrast, LLMs made errors on only 6\% of \textit{pointer}, \textit{memory}, and \textit{index} operations seem to be more easily handled by the LLMs, perhaps because they do not require multiple steps of reasoning.

\mycomment{
\input{Figures/error-examples/hmr-hallucination}

% \input{Figures/error-examples/hmr-repetition}

% \setfigurecaption

\sethlcolor{yellow}
Out of the \textit{Hal/Mem/Rep} category, the most common case was hallucination, where the LLM produced reasoning based on code not represented in the prompt.
Figure \ref{fig:hallucination-example} shows an instance where the LLM explained a potential integer overflow in a formula which does not occur in the function.
Hallucinations can undermine the trustworthiness of the prediction since they require readers to verify the LLM's reasoning against the code.
}

\Cref{fig:strict-performance} presents the second part of the results of RQ3. Here, we provide a summary of the models' capability of reporting the type, the location and the root cause of a vulnerability. The results show that although most LLMs correctly predicted up to 79\% of vulnerable examples (blue bar), correctness dropped substantially when we consider the predicted location, bug type, and causes.
Considering both bug types and locations (orange bar), all models dropped in correctness, decreasing by 18-67\%, with Mistral failing on all examples.
Considering root-cause explanations (purple bar), model correctness decreased by 24-50\%.

\mycomment{
\textit{Prediction}: the model's binary prediction matches the label (vulnerable/non-vulnerable).
\textit{Bug Type}: the bug type predicted by the model matches the ground-truth bug type.
\textit{Location:} a location which the model mentioned as related to the vulnerability matches the locations changed in the bug-fixing patch.
\textit{Cause:} we observed no reasoning errors in the model's reasoning about the root cause.
We consider an example correctly labeled if all selected explanations are true.
}

\begin{summarybox}
\textbf{Summary for RQ3:}
57\% of LLM responses contained errors when explaining the cause of vulnerabilities.
The most common error categories were ``Code understanding'' (41\% of responses, especially missing Bounds/NULL Checks) and ``Hallucination/Memorization/Repetition'' (11\% of responses).
All LLMs experienced a substantial (18-100\%) drop in correctness when considering their predictions of bug location, type and causes.
\end{summarybox}


==> _OldVersion.ICSE25/Sections/45.dbgbench.tex <==
\subsection{RQ4: How do LLMs compare to human developers for localizing vulnerabilities?}
\label{sec:dbgbench}

% dbgbench includes one buffer overflow, https://dbgbench.github.io/find.c8491c11.diagnosis.txt
\subsubsection{Study setup} We are interested in how LLMs' performance compares to human's. To set up the experiments, we used DbgBench~\cite{dbgbench}, where the detailed human performance is reported. In their study~\cite{dbgbench}, 12 professional software engineers were given the source code, bug reports, and test cases related to 27 bugs in the \texttt{find} and \texttt{grep} utilities, such as null-pointer dereferences, buffer overflows, resource leaks, and infinite loops.  They reported a diagnosis with fault locations, rated their perception of the difficulty, and provided a patch. To match the human setting, we gave each LLM prompts containing the bug report, test case, the source code of the files containing the faults, and instructions ``Given the above bug report, test case which reproduces the bug, and source code, provide the line numbers of all fault locations in the code in the following format: \texttt{* file.c:line number}.''
% \benjamin{Other details will be addressed in threats to validity}
These prompts (averaging 19-25k tokens) exceeded the context length of 4 models, which we excluded.
We extracted fault locations from the outputs of the remaining 7 LLMs and compared them with the correct fault locations from DbgBench, considering a prediction correct if at least one fault location matched the ground truth.
% \benjamin{TODO: Run GPT3.5, Gemini, rerun GPT4 and add the results}

\input{Figures/dbgbench/performance-table}

\subsubsection{RQ4 Results}
% \benjamin{TODO: Discuss new results}
\Cref{tab:dbgbench-correct} shows that among the 7 models, 5 models produced correct output for 6 bugs and made a total of 11 correct predictions (some models predict correctly on the same bug). GPT-3.5 performed the best and correctly located 4 bugs. Interestingly, the newer model, GPT-4, did not match the ground-truth fault locations on any examples, and neither did Mistral. These bugs took humans 15 to 50 minutes to diagnose, with difficulty ratings ranging from slightly to very difficult (2-4 on a scale of 1 to 5).
\new{\Cref{fig:dbgbench-distribution} shows where these bugs located in the entire dataset in terms of perceived difficulty and diagnostic time given by DbgBench.}

%in the entire dataset the bugs which LLMs predicted correctly were clustered around the mean time and difficulty for the entire dataset.}
% 
%\wei{GPT-4 didn't provide any fault locations at first, saying "I don't have complete information, so it's difficult to provide the fault locations". So I added a clause to the prompt instructing it to provide fault locations even if the code is incomplete, but the fault locations provided were incorrect. we should report this as many people will be interested in gpt 4, to show that the model update can make certain functionality worse.}
% 
% \wei{fig 8 to be cleaned}

% Interestingly, both humans and LLMs tended to perform better on examples which were rated easier.
% These results suggest that LLMs and humans found similar examples easy or difficult.
% \benjamin{This claim needs to be strengthened with more evidence. We can show e.g. the human data on Fig 8.}

% \Cref{fig:dbgbench-distribution} plots the bugs where LLMs predicted correctly over the recorded time to diagnose and perceived difficulty from human developers.
% The correct LLM predictions were clustered around the mean of both time and difficulty rating.
% LLM correct predictions skewed right more than human predictions, meaning that they had a longer tail and LLMs tended to predict correctly on examples with an easy rating or shorter diagnosis time more often than humans.
% The bugs which LLMs predicted correctly were distributed the same as the difficulty and diagnosis time of the whole dataset. This is surprising since we expect predictions to be more likely correct on examples which with lower difficulty/time required, and indicates that the correct LLM predictions were likely not affected by the difficulty or diagnosis time. \benjamin{Need statistical test to show that they match, and show human-correct datapoints which should skew towards easier bugs.}
% The human participants noted missing documentation and incorrect hypotheses as an issue which caused bugs to be difficult; in our setting, the LLM only sees the code and so may not be affected by these issues.

\input{Figures/dbgbench/difficulty-time}

\input{Figures/dbgbench/performance-figure}

In \Cref{fig:dbgbench-performance}, we visualize individual bugs and rank them based on the ``easiness'' of diagnosis for humans. To do so, we first rank the bugs based on the correctness achieved among the developers who diagnosed the bug, and to break ties, we compared the diagnosis time. Here, we can see that LLMs failed to correctly predict the examples which were the hardest for humans (rightmost dots), \new{as well as many of the easiest examples (missing 4 out of 7 leftmost dots which were localized by 100\% of humans)}. Overall,  LLMs performed substantially worse than humans. Most of the correct predictions were among those already correctly diagnosed by 70-100\% of human study participants. These findings suggest that current LLMs still have significant limitations in localizing software bugs in a real-world setting.

\mycomment{
However, LLMs were far from human performance.
\Cref{fig:dbgbench-performance} compares the human and LLM performance on all the bugs in DbgBench. LLMs performed substantially worse than humans, with 21/27 examples lacking correct localizations by any model.

Furthermore, the bugs which were predicted correctly were already correctly diagnosed by 70-100\% of human study participants.
}

\begin{summarybox}
\textbf{Summary for RQ4:}
LLMs correctly located 6/27 bugs from \wei{DbgBench}, while at least one human correctly located 27/27 bugs. GPT-3.5 performed the best and correctly located 4 bugs. GPT-4 and Mistral failed to locate any bugs correctly.

%and both LLMs and humans found similar examples to be easy or difficult.
%However, LLM performance was far below human level on DbgBench, with all models failing on 21 out of 27 bugs, and 2 models failing to localize any bugs correctly.
\end{summarybox}


==> _OldVersion.ICSE25/Sections/46.threats.tex <==
\section{Threats to Validity}
Better prompts than those we evaluated may exist.
To draw out the best model performance, we systematically explored several prominent prompting techniques and introduced three \wei{new approaches} motivated by our domain knowledge (\Cref{sec:rq1}).
Model performance can be reduced by irrelevant context~\cite{distractibility}, or the order~\cite{incontext_order} and quality~\cite{incontext_number} of in-context examples. To alleviate these potential issues, we reported the best-case performance among various prompt orderings and varying amounts and sources of context\wei{, and tried different number of shots (\Cref{sec:discussion})}.

%Our dataset of 100 functions may seem limited or may not represent realistic vulnerability data.

We queried 100 functions due to the cost of LLMs (see \Cref{sec:dataset}), which may seem limited. However, we note that our dataset originates from 36 open-source projects with diverse applications, including databases, servers, and interpreters.
The vulnerabilities represent important issues, all featuring in the top-25 most dangerous CWEs for the past five years~\cite{cwe_stubborn}, and were manually curated to ensure quality~\cite{croft_quality} and focus on real-world use cases~\cite{sven}. \wei{We performed a pilot study which suggests that the models did not memorize the labels (\Cref{sec:discussion}).}


%These measures increase confidence in the results. %despite dataset size.

To mitigate potential biases from the experimental setup and metrics, we evaluated the LLMs in two distinct scenarios: ``paired'' and ``unpaired'' (\Cref{sec:rq2})\newtwo{, and aggregated results across 3 different random seeds}. We justify our choice of metrics in \Cref{sec:metrics}.
% discuss the precision/recall trade-offs and 
% We also report and discuss the precision and recall in order to reflect the relative importance of vulnerable and non-vulnerable predictions.
% We reported Balanced Accuracy rather than e.g. F1 score and Matthews Correlation Coefficient (MCC)~\cite{mcc} because F1 and MCC favored heavily biased classifiers (\Cref{sec:metrics}).
% \wei{mention the small possible set 100, why this is enough}
% \wei{Based on our pilot study (\Cref{sec:discussion}), we believe that the models had not  memorized the vulnerability labels.
% }

The analysis of the LLMs errors can involve subjective judgments. To ensure confident classifications, we rigorously designed the categories to be unambiguous and confirmed agreement among multiple raters (\Cref{sec:rq3}).

Our fault localization setting for DbgBench does not perfectly match the human debugging scenario, as the LLMs could not run tests or use debuggers. While such tools could aid LLMs in making a diagnosis, we focused on a direct use of LLMs in this study. Investigating long-context integration and interactive agent environments is an interesting direction for future work. %(\Cref{sec:dbgbench}).

%straightforward evaluation to establish a baseline

%%%%%%%%%%%%%%%%% FIRST REVIEW
% % \wei{I felt threats are too long.
% % 1. better prompt methods may exist.
% % 2. data may not sufficient 100 and not representative.
% % try to clean up the threads like this,
% % shorten it and provide a more crispy message}
% Our prompts may not produce the best vulnerability detection performance.
% We surveyed various state-of-the-art prompting techniques and introduced three of our own prompt templates, and systematically searched these prompt templates to find the best-case performance of each model (\Cref{sec:rq1}).
% Model performance can be reduced by irrelevant context~\cite{distraction} or the order~\cite{order-incontext} and number~\cite{number-incontext} of in-context examples. To mitigate these issues, we reported the best-case performance among various prompt orderings and amounts of context, and focused on relatively minimal prompts to avoid irrelevant information.
% % \benjamin{TODO: Thoroughly read the papers Earl suggested to see if we fully addressed the issue.} 
% % For vulnerability explanations, we experimented with several prompts and chose the final method because it allowed us to clearly and consistently generate explanations for analysis.

% % https://cwe.mitre.org/top25/archive/2023/2023_stubborn_weaknesses.html
% Our dataset of 100 functions may not be sufficiently large or may not represent realistic vulnerability data.
% The examples are sourced from and include five types of vulnerabilites which have appeared in the top-25 CWEs for the past five years~\cite{cwe_stubborn}, and were manually validated in a rigorous procedure~\cite{sven}.
% To mitigate bias, we evaluated the LLMs in two distinct settings: paired buggy/fixed examples and randomly sampled examples with no bug-fix relationship (\Cref{sec:rq2}). We also report and discuss the precision and recall in order to reflect the relative importance of vulnerable and non-vulnerable predictions.
% We primarily report Balanced Accuracy rather than some other popular metrics such as F1 score and Matthews Correlation Coefficient (MCC)~\cite{mcc}. We found that both F1 and MCC favored heavily biased classifiers (\Cref{sec:metrics}).
% % \wei{mention the small possible set 100, why this is enough}

% Our error categories are subjective. We mitigated subjectivity to produce confident classifications by rigorously designing the categories to remove ambiguity and by confirming the agreement among multiple raters (\Cref{sec:rq3}).

% The fault localization setting for DbgBench could not perfectly match the conditions of the human study.
% The LLMs could not read the entire program's source code due to context length limitations.
% % However, we believe that our setting is realistic if we assume that the bugs can be localized to an entire file based on the bug report.
% Additionally, while the humans had the ability to run tests and attach a debugger, the LLMs observed the code without running it. While the complete code, tests, and a debugger provide valuable information for diagnosis, we attempted to implement the most straightforward version of this evaluation and leave further investigation of long-context integration and agent environments to related work (\Cref{sec:dbgbench}).

%%%%%%%%%%%%%%%%%%%%%%%5 FIRST DRAFT
% \benjamin{TODO: revise after all experiments are done}

% \benjamin{TODO: Threat, our dataset has buggy/fixed pairs}

% Our design of the prompts might be flawed or incomplete. We explored the most common and SOTA methods for prompting in this new area.
% % 1.  It’s well-known that performance is extremely sensitive to the order of the shots in few-shooting:  https://arxiv.org/abs/2104.08786.  It’s probably too late to permute the shots in our few shot prompt or other components of our prompts, but we should cite this paper at least discuss this issue, rather than leave it to reviewers to point it out to us.
% % 2.  This interesting paper about LLM’s distractibility — https://arxiv.org/abs/2302.00093 — makes me wonder whether some of our prompts “distracted” the model.  We should cite and discuss this work.
% \benjamin{TODO: Address in-context example ordering, number, and distractibility.
% Note that when searching for the best prompts, we tried different prompt orderings and varying context amounts to avoid irrelevance. Feel free to suggest other ways to integrate these papers.}

% \benjamin{The LLMs could not read the entire program's source code since it would overrun their context length and provide irrelevant input, possibly confounding the model's response; however, we believe that our setting is realistic if we assume that the bugs can be reliably localized to a single file based on the bug report. Additionally, while the humans had the ability to run tests and attach a debugger, the LLMs observed the code without running it.}

% Balanced Accuracy vs. MCC and F1

% Parsing the responses might be done incorrectly. We checked it and found a low percentage of errors, instilling confidence in our implementation.

% Explanations are represented unevenly between models. But all models are represented with a baseline count of examples, and we observed that the distribution of error categories is similar among the different models.

% Our method of prompting the models may be imperfect or ``not causal''. We acknowledge that we analyze only explanations and these can fail to represent the model's ``thought process''~\cite{citation-needed} as well as other explanation methods. However, we argue that this still has value because the explanations should be correct in order to be used to boost any predictions, and the explanations are a valuable part of the predictions by themselves as they help explain the prediction to practitioners.

% Our error categories are subjective by necessity. We mitigated this with a rigorous design and agreement score verification.
% Our classifications may be coerced or influenced by one rater. We managed this by independently rating the examples, then majority/automatic ruling, and show that our final results for the disagreed examples did not favor one rater's original responses over another.

==> _OldVersion.ICSE25/Sections/49.discussion-short.tex <==
\section{Discussions}
\label{sec:discussion}

\newtwo{Because SVEN is open-source, the labels may be inside the training dataset of recent LLMs. To test if LLMs memorized vulnerability labels, we \wei{refactored} the code (using NatGen~\cite{chakraborty2022natgen}) while preserving the vulnerability labels and evaluated the models.
If the models simply memorized the vulnerability labels, we would expect performance to be substantially reduced on the \newthree{refactored code}. We saw both improvements and reductions in performance and only small differences in Balanced Accuracy (0.02-0.09), even with extensive \newthree{refactoring}.} %Although these results do not disqualify the possibility of memorization, they suggest that the models did not simply memorize the labels.}

%We used NatGen~\cite{chakraborty2022natgen}, to transform the source code's variables, operands, and control flow, with various amounts of transformation.

% The number and order of in-context examples can affect LLM performance~\cite{incontext_number,incontext_order}, including distracting the model~\cite{distractibility}.
\newtwo{As a pilot study, we tried using 2, 4, 6, or 8 in-context examples for the \newthree{models which performed best with in-context prompts} and found that 6-shots performed best for most models.
Extended results for both experiments can be found in our data package~\cite{data-package-figshare}.}


==> _OldVersion.ICSE25/Sections/49.discussion.tex <==
\section{\wip{} Discussions}

\benjamin{TODO: Cut content and figures to fit inside space.}

% Memorization/perturbation experiments

\paragraph{Memorization evaluation}

\begin{figure}
    \centering
    \begin{tabular}{lll}
\mbox{\colorline{31}{119}{180} StarChat-$\beta$}  &
\mbox{\colorline{214}{39}{40} MagiCoder}  &
\mbox{\colorline{227}{119}{194} Code LLAMA} \\
\mbox{\colorline{255}{127}{14} StarCoder}  &
\mbox{\colorline{148}{103}{189} LLAMA 2}  &
\mbox{\colorline{127}{127}{127} Mistral} \\
\mbox{\colorline{44}{160}{44} Mixtral-MoE}  &
\mbox{\colorline{140}{86}{75} WizardCoder}  &
\mbox{\colorline{188}{189}{34} Gemini} \\
    \end{tabular}
    \includegraphics[width=0.8\linewidth]{Images/performance-eval/memorization.pdf}
    \caption{Model performance under 0\%, 50\%, and 100\% perturbation. Lines represent the mean model performance on three random seeds.\benjamin{TODO: Add GPT3.5 and GPT4 results.}}
    \label{fig:memorization}
\end{figure}

\benjamin{This section can be pared down}
% 
Because the LLMs are pre-trained on huge corpora drawn from the Internet, the source code and labels in the open-source SVEN dataset may have been included in their pretraining data.
We conducted an experiment based on semantic-preserving transformations to evaluate whether and to what extent the models have memorized the training data. If the models' performance drops substantially when semantic-preserving transformations are applied, then the models' performance can be attributed to memorization rather than general vulnerability detection ability.

We used the NatGen tool provided by \citet{chakraborty2022natgen} to transform the source code of the functions while preserving the semantics of the source code, including the vulnerability label.
We applied the Var Renaming, Operand Swap, Block Swap, and Loop Transformation, each of which modifies different source code structures. We evaluated the models on settings of 50\% and 100\% perturbation; for 50\% perturbation, we randomly select 50\% of the possible locations for transformation, and for 100\% perturbation, we applied the transformations at all possible locations.
% As LLM models are trained on huge amount of data from the internet, it can happen that the models have also learnt the experiment functions with their vulnerability labels. Hence,  we conduct memorization tests to evaluate the extent the models have memorized the data. We conduct 50\% and 100\% semantically-equivalent perturbation of the data and hypothesize that the performance of perturbed data should deteriorate if the models have already seen the labels. We use Var Renaming, Operand Swap, Block Swap and Loop transformation techniques from NatGen \cite{NatGen} for the perturbation. For 50\% perturbations, we randomly select 50\%  of the variable names, binary logic operations, if else blocks, and for while loops for these operations.  For 100\% perturbations, we do these operations for all the occurences.

% \benjamin{We may tack this onto RQ2 (then add a summary of the results to the summary box) or a separate section.}
Figure \ref{fig:memorization} compares the models' mean performance over three random seeds on the non-perturbed data (0\%) with the 50\% and 100\% perturbation settings.
The difference in performance between different settings is relatively small (between \textcolor{red}{0.02 and 0.09} difference in Balanced Accuracy), indicating that the models' performance was not affected much by the perturbations.
Some models did gradually decrease in performance with added perturbation, such as MagiCoder (decreased from \textcolor{red}{0.53 to 0.45}), StarChat-$\beta$ (decreased from \textcolor{red}{0.56 to 0.54}), and Mixtral (decreased from \textcolor{red}{0.54 to 0.51}); this may indicate that part of these models' performance was due to memorization.
% Fig \ref{fig:memorization} compares the performance of perturbed data with the non-perturbed data. The performance of MagiCoder, StarChat-Beta, and Mixtral drops with the increase of perturbation. WizardCoder also shows lower performance with both perturbations than the no-perturbation performance. This indicates that these models (MagiCoder, StarChat-Beta, Mixtral, WizardCoder) may have seen the data with the vulnerability information to some extent. For the other models, there are fluctuations in the performance. CodeLLama has lower accuracy with 50\% perturbation but higher accuracy with 100\% perturbation. Other models (LLama 2, Mistral, StarCoder-TA) had higher accuracy with both perturbations than the no-perturbation. This indicates that these models (CodeLLama, LLama 2, Mistral, StarCoder-TA)  may not have seen the data with the vulnerability labels.
% \benjamin{Now is not the time to add to the scope of the paper! But, one interesting datapoint we could add here: we can train some SOTA vulnerability detection models like LineVul, DeepDFA on BigVul, then evaluate their MPCAccuracy on our SVEN dataset. This would allow us to compare the LLMs with SOTA vulnerability detection models.}

\wei{Shots vs performance in context learning}


==> _OldVersion.ICSE25/Sections/50.relatedwork-old.tex <==
\section{\wip{} Related Work}

\subsection{Large Language Models for Software Engineering}
% \benjamin{Outline, please use roughly one sentence per bullet point:
% 1. LLMs [cite] have been pretrained on massive corpora of code and are applied in a prompting setting for downstream tasks in SE.
% 2. List the downstream tasks they have been used for: code generation [citation], program repair [citation], etc. Leave vulnerability detection out to discuss in later section; however (now relate to our work), it's not understood whether they can detect vulnerabilities, reason about the code and vulnerabilities in the code.
% 3. Prompting section.
% Emphasize that they are pretrained, and prompting can make a big difference, and that the performance on vulnerability detection is unknown.}



\new{LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been applied in various software engineering tasks,}
such as code generation~{\cite{destefanis_2023_preliminary,dong_2023_self,wang_2023_enhancing}}, code completion~{\cite{code-completion_deng_2023,li_2023_cctest,wang_2023_codet5+}}, program repair~\cite{xia_apr}, and \new{code summarization}~\cite{chen_2023_gptutor, nam2024using, code_explanation_macneil_2023, li2023hitchhikers, maScopeChatGPTSoftware2023} through the use of \textit{prompting} -- providing formatted inputs to elicit a response which is applicable to a downstream task.
Effective prompts can condition the model for a specific task like Question/Answer~\cite{gpt3}, provide additional information through in-context examples~{\cite{rag}} and elicit step-by-step reasoning through chain-of-thought examples~{\cite{cot,kojima2022large}}.
\new{We have surveyed these state-of-the-art prompting methods and applied them to the vulnerability detection task.}


%%%%%%%%%%%%%%%%%%%%%%%% First version
\begin{comment}
% LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been pre-trained on massive corpora of code and natural language, and applied in many different down streaming tasks in software engineering,
\new{LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been applied in various software engineering tasks,}
such as code generation~{\cite{destefanis_2023_preliminary,dong_2023_self,wang_2023_enhancing}}, code completion~{\cite{code-completion_deng_2023,li_2023_cctest,wang_2023_codet5+}}, code repair~{\cite{automatedbugreplay-icse2024, chenTeachingLargeLanguage2023, repair_cao2023study, repair_wu_2023, repair_islam2024llmpowered, pearceExaminingZeroShotVulnerability2022}}, and \new{code summarization}~\cite{chen_2023_gptutor, nam2024using, code_explanation_macneil_2023, li2023hitchhikers, maScopeChatGPTSoftware2023} through the use of \textit{prompting} -- providing formatted inputs to elicit a response which is applicable to a downstream task.
% Automated Program Repair in the Era of Large Pre-trained Language Models
% 
% Prompt engineering is an integral part of LLM usage. It is the process of searching for the prompt template that results in the most effective performance for a downstream task~\cite{liu_pre-train_2021}.
% A well-structured and domain-guided prompt can significantly enhance performance in a down-streaming task ~\cite{structuredPrompt-1, structuredPrompt-2}.
% The format of the prompt can provide additional information to inform the model's predictions or allow the model to reason about its prediction in sequential steps.
% Several techniques have been proposed, including in-context learning~{\cite{lee2023incontext,rag}}, chain-of-thought~{\cite{cot,kojima2022large}}, tree-of-thoughts prompting~\cite{yao_tree_2024,long2023large} etc.
% 
% 
% 
Effective prompts can condition the model for a specific task like Question/Answer~\cite{gpt3}, provide additional information through in-context examples~{\cite{rag}} and elicit step-by-step reasoning through chain-of-thought examples~{\cite{cot,kojima2022large}}.
\new{We have surveyed these state-of-the-art prompting methods and applied them to the vulnerability detection task.}
% We systematically searched among existing prompting methods and introduced three novel prompting methods: the use of contrastive pairs to select in-context examples, as well as chain-of-thought using examples from CVE descriptions and Static Analysis.
% In this work, we evaluated three of the pre-existing prompting methods and introduced three new prompting methods incorporating domain knowledge,  such as In-context prompting based on contrastive pair, Chain-of-Thought from CVE descriptions, and Chain-of-Thought from static analysis.
% In spite of this progress, it is yet unknown to what extent LLMs can detect software vulnerabilities or reason about vulnerabilities in source code. 

% There are several LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} that are trained to generate code and natural language about the code from both natural language and code prompts.

% MagiCoder ~\cite{magicoder}, Code LLAMA~\cite{codellama}, Gemini-Pro~\cite{gemini}, GPT4 ~\cite{gpt4}, WizardCoder\cite{wizardcoder},  and GPT3.5 ~\cite{gpt3.5} achieved 70.7\%, 67.8\%, 67.7\%,  67.0\%, 57.3\% and 48.1\%  pass@1 score respectively on the code generation of the HumanEval benchmark. 
% Recent works have also used LLMs in many different software engineering down-streaming tasks.
% \benjamin{Too much detail, please summarize ``...different software engineering tasks, such as code generation [citation], program repair [citation], etc.''}
% \citet{xiaConversationalAutomatedProgram2023} propose a fully automated conversation-driven automated program repair tool using ChatGPT, which achieves new state-of-the-art performance on the Defects4j dataset. \citet{pearce2022examining} examine the ability of different LLM models on code repair tasks in zero-shot settings and found that the performance is promising in synthetic and hand-crafted scenarios but is not good enough for real-world examples. \citet{chenTeachingLargeLanguage2023} propose a self-debugging approach via few-shot demonstrations that teaches the LLM models to debug the predicted program. \citet{automatedbugreplay-icse2024} use LLM to automatically reproduce the bugs from the bug reports by leveraging few-shot learning and chain-of-thought reasoning. 
% % Survey prominent LLMs in general, focusing on novel contributions or mechanisms (ChatGPT first LLM, LLAMA open-source, Mixtral mixture of experts).
% % Survey LLMs specifically trained for code, and code generation as the most popular task.

% % \subsection{Prompt engineering for LLMs}

% \benjamin{Outline:
% 1. Define prompt engineering and say it's important because it can improve performance on down-stream tasks. Maybe just cite \citet{liu_pre-train_2021}
% 2. Several techniques have been proposed, including in-context learning~\cite{brown_language_2020,rag,others} and chain-of-thought~\cite{cot,others}.
% 3. Mention and differentiate our work by saying we designed new ways to incorporate in-context examples (contrastive pairs) and CoT (CVE and Static Analysis).}

% \benjamin{let's merge with prior section as this section will be short}
% An integral part of LLMs is prompt engineering, as a slight change in the prompting could have a significant impact on the performance \cite{learningPrompt}.\benjamin{This citation is not very applicable, as it's learning to prompt in vision domain.}
% A well-structured and domain-guided prompt can show a significant performance enhancement in a down-streaming task ~\cite{structuredPrompt-1, structuredPrompt-2}.
% Hence, research on designing different prompt designing paradigms is rapidly growing\cite{structuredPrompt-3}.
% \benjamin{Please merge these two into one short sentence -- see outline.}
% Though directly prompting the models to get the desired response shows promising results in some tasks by using the prior knowledge from the pre-training data, the models face challenges in providing desired output for the unseen contexts ~{\cite{brown_language_2020, fan2023automated}}. To overcome this, Brown et al. \cite{brown_language_2020} utilizes few-shot learning by adapting the context with the few sets of desired input and output. Though few-shot prompting shows efficient performance with some simple tasks, it faces difficulties with the multi-step arithmetic and logical reasoning benchmark ~\cite{rae2022scaling}. Wei el al.~\cite{wei_chain--thought_2023} propose Chain-of-thoughts reasoning, an instance of few-shot-prompting, which replaces the output of the shot examples with the intermediate reasoning steps.

% Survey existing work on developing prompts for LLMs.
% In-context learning, RAG, CoT.
\end{comment}

\subsection{LLMs for Vulnerability Detection}



Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as basic prompting ~{\cite{vulDetIssrew-2023, wang2023defecthunter, noeverCANLARGELANGUAGE, bakhshandeh2023using, fu2023chatgpt, cheshkov2023evaluation, hu2023large}}, in-context prompting~{\cite{gao2023far, zhou2024large, mathews2024llbezpeky, liuGptandIncontext2023,chan2023transformerbased, ma2024lms}}, and fine-tuning~{\cite{shestov2024finetuning, chen2023diversevul, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized CoT, such as zero-shot CoT~{\cite{li2023hitchhikers, du2024evaluation, automatedbugreplay-icse2024, chen2023chatgpt, sun2023gptscan} }, Few Shot CoT~{\cite{ullah2023large}}, CoT with Multi-Turn Conversation~{\cite{davidYouStillNeed2023}}, CoT with generic program information such as CFG, DFG, PDG and API call ~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.

\benjamin{Our summary of our work must focus on what is new. We can present most of the ``basic'' papers in a big group as you've done, then introduce how ours is different (contrastive, cot-sa, cot-cve. Then, for the others which are close to ours (CoT based on vulnerability report~{\cite{sun2024llm4vuln}}, CoT based on commit message~{\cite{yu2024security}}), dig into the differences.} 
\new{In this work, we propose three new prompting methods, such as in-context learning based on contrastive information from bug-fix commits,  CoT based on CVE descriptions(CoT-CVE, and CoT based on static analysis(CoT-SA). Yu et al.~{\cite{yu2024security}} introduce multi-turn conversational CoT, and in the first turn, they ask the LLMs to generate the supplementary code files based on the commit message. The original test code is analyzed for security defects in the second turn. \rasel{I am unsure how to differentiate this from our work. Which of our prompts is close to this one? Contrastive pair? We didn't use the commit message in that setting. Right?} Sun et al. ~{\cite{sun2024llm4vuln}} creates a database of the vulnerability report with its corresponding code. During prompting, they retrieve the bug report of the similar code and use the raw/summarized(by GPT 4) report with zero-shot CoT prompting. In our COT-CVE method, we include the CVE descriptions of the examples used along with their Chain-of-Thought responses.} 
CoT based on vulnerability report~{\cite{sun2024llm4vuln}}, CoT based on commit message~{\cite{yu2024security}},
% 


\new{
Nong et al. ~{\cite{nong2024chainofthought}} inspected the 100 random failure cases of three LLMs(GPT-3.5, LLama2, Falcon) and identified four common root causes - insufficient contexts, oblivion of CWE, incomplete control flow analysis, and incomplete data flow analysis. They found that LLMs miss the important control flow facts related to vulnerability during their reasoning and insufficient context of the code snippet is also another dominating reason for the failure cases. Sun et al. \cite{sun2024llm4vuln} analyzed all the false negative and false positive cases of three LLMs (GTP-4, Mistral, and CodeLLama) and found that the significant factor affecting LLMs' vulnerability detection capability is the lack of reasoning capabilities. }
% Sun et al. \cite{sun2024llm4vuln} \rasel{They only counted the number of wrong reasoning. No fine-grained analysis on the wrong reasoning}.
\new{Ullah et al. ~{\cite{ullah2023large}} investigated the quality of the LLMs(GPT-4, GPT-3.5, CodeLLama-34B, chat-bison, codechat-bison) reasoning\rasel{(for all the responses LLM generated, more than 700+. This number varies based on models as models don't response in many examples. They are not counted for that model.)} and found that LLMs responses are not backed by thorough and correct reasoning in many cases.}
% \rasel{ Ullah et al. ~{\cite{ullah2023large}} : The analysis is focusing on four aspects: (1) for how many cases
% does the LLM provide a reasoning for the presence of a vulnerability in a code snippet at all, (2) for how many correct
% answers the LLM also provides a correct reasoning, (3) for how many correct answers the LLM provides an incorrect reasoning, and (4) for how many answers does the LLM
% provide the wrong answer, but a correct reasoning.} 
\new{Yu et al.~{\cite{yu2024security}} analyzed the 82 responses of LLMs(Gemini-Pro, GPT-4, GPT-3.5) and identified 16 categories of errors across five themes. Their results indicate that the responses produced by LLMs often suffer from verbosity, vagueness, and incompleteness, highlighting the necessity to enhance their conciseness, understandability, and compliance to security defect detection. We deeply analyzed the errors which occurred in LLM responses from the perspective of vulnerability detection, producing findings reflecting on the fine-grained errors and the syntactic structures which beckoned improvement.}


\begin{itemize}
    \item Yu et al. ~{\cite{yu2024security}} I am unsure how to differentiate this from our work. Which of our prompts is close to this one? Contrastive pair? We didn't use the commit message in that setting. Right?
    \item Sun et al. \cite{sun2024llm4vuln} They only counted the number of wrong reasoning. No fine-grained analysis on the wrong reasoning.
    \item  Ullah et al. ~{\cite{ullah2023large}} : The analysis is focusing on four aspects: (1) for how many cases does the LLM provide a reasoning for the presence of a vulnerability in a code snippet at all, (2) for how many correct answers the LLM also provides a correct reasoning, (3) for how many correct answers the LLM provides an incorrect reasoning, and (4) for how many answers does the LLM provide the wrong answer, but a correct reasoning.
    \item Yu et al.~{\cite{yu2024security}}: the last line need to be praphrased.

\end{itemize}


% \benjamin{For these closely related error analysis studies, we need detail into the findings (their conclusions, not just how many categories), extent (did they analyze a lot of responses or just a few case studies, and how many models), and what kinds of errors they investigated in order to set apart our work.}
% \new{\sanjida{Zouh et al.~{\cite{zhou2024large}}  analyzed how effective ChatGPT (GPT3.5 and GPT 4) is with different prompt designs in vulnerability detection compared to baselines where they’ve used CodeBERT as a baseline model. However, in our paper, we are trying to determine the effectiveness of different prompt designs on 11 LLMs. Zhang et al.~{\cite{zhang2023prompt}} investigated the application of ChatGPT in identifying vulnerabilities. Their primary focus lies in improving prompts by incorporating additional information like API calls and data flow, and utilizing chain-of-thought prompting. In contrast, we have introduced a more diverse set of prompts, including Basic (Zero-shot) prompting,n-shot (In-context) prompting, Contrasting pairs, Chain-of-Thought from CVE descriptions, Chain-of-Thought from Static Analysis, which they didn’t consider in \cite{zhang2023prompt}. We have also analyzed the types of mistakes LLMs make when reasoning about vulnerability predictions that are not thoroughly examined in \cite{zhang2023prompt}.}
% }



%%%%%%%%%%%%%% Starting outline
% \new{Starting outline
% \begin{itemize}
%     % \item Several recent studies have initiated investigations into the usage of LLMs for vulnerability detection, using well-known techniques such as basic prompting~\cite{basic-approaches} fine-tuning~\cite{finetune-approaches}, and in-context examples~\cite{incontext-approaches}.
%     % \item Several papers have proposed CoT such as zero-shot CoT, or generic program information such as CFG, others...~\cite{cot-approaches}.
%     % We propose in-context learning based on contrastive information from bug-fix commits and CoT based on CVE descriptions and static analysis
%     \item \citet{LLM4Vuln: A Unified Evaluation Framework for Decoupling and Enhancing LLMs’ Vulnerability Reasoning} evaluated LLMs' reasoning capabilities by broad failure modes; \citet{Security Code Review by LLMs: A Deep Dive into Responses} analyzed responses of LLMs based on a taxonomy of common LLM errors. We deeply analyzed the errors which occurred in LLM responses from the perspective of vulnerability detection, producing findings reflecting on the fine-grained erros and the syntactic structures which beckoned improvement.
% \end{itemize}}


% There are also many works on Vulnerability Detection using LLMs. Some works use Basic prompting with a variety of natural language descriptions, such as ~{\cite{vulDetIssrew-2023, wang2023defecthunter, noeverCANLARGELANGUAGE, bakhshandeh2023using, fu2023chatgpt, cheshkov2023evaluation}}. However, these works didn't evaluate and compare the best natural language description for individual models, while we search for the best natural language for basic prompting for each individual model that help us to evaluate the best capabilities of these models.
% Some works also employ few-shot prompting for their study with different in-context example selection strategies, such as random Selection ~{\cite{gao2023far, zhou2024large}}, retrieved similar examples~{\cite{zhou2024large, mathews2024llbezpeky}. Unlike these works, we analyze the performance of different natural languages with each shot example and employ several retrieval strategies to find the best-performed retrieval method. CoT prompting is also used in a few works ~{\cite{zhangPromptEnhancedSoftwareVulnerability2023, sun2024llm4vuln, davidYouStillNeed2023}}. However, 

% Some works ~{\cite{shestov2024finetuning, chen2023diversevul, yusuf2024instructions}} also fine-tune the LLM models with the Vulnerability Detection data. As fine-tuning is a costly procedure and our research direction for this work is to search for the best prompting and evaluate them, we keep the fine-tuning direction for future work.


% Zhang et al. \cite{zhangPromptEnhancedSoftwareVulnerability2023} study the performance of vulnerability detecting using ChatGPT. They conduct extensive experiments with some basic and chain-of-thoughts prompting by leveraging structural and sequential auxiliary information. Purba et al. \cite{vulDetIssrew-2023} evaulate the performance of four different LLMs (CodeGen, Davinci, GPT-3.5-Turbo, GPT3.5-Turbo-0613) with a set of basic prompting. They found that LLMs don't perform well in vulnerability detection because of the high false positive rate but show promise in identifying subtle patterns commonly associated with different kinds of vulnerabilities. 


% Survey other papers which apply and study LLMs for vulnerability detection.
% Highlight very-closely-related ones and differentiate them from our work.


%%%%%%%%%%%%%% First draft of related work summary
% \benjamin{TODO: Expand related work. Emphasize our novelty.}

% There are several papers which study LLMs for vulnerability detection.
% Some parts of our planned study have been looked at before, though most benchmarks are rather small so some merit may come from running on a larger dataset (on the order of 100-1000 examples).
% However, several techniques/areas have not been studied yet, and most papers do not study LLMs besides ChatGPT or a few related models, so there is some opportunity for our study to bring novelty and impact by being more comprehensive.

% Below is a short list of the most closely related papers, categorized into the techniques which they studied. Keep in mind many of the techniques are studied only on one instance/implementation, but as we have seen, these techniques can be instantiated in diverse ways which affect the performance.
% \begin{itemize}
%     \item Zero-shot prompts~\citep{zhang2023prompt,cheshkovEvaluationChatGPTModel2023a,noeverCANLARGELANGUAGE,bakhshandehUsingChatGPTStatic2023,pearceExaminingZeroShotVulnerability2022}
%     \item $n$-shot prompts~\citep{li2023hitchhikers,fengPromptingAllYou2023}
%     \item Tool use~\citep{li2023hitchhikers,sunWhenGPTMeets2023,fengPromptingAllYou2023}
%     \item Multi-turn conversation~\citep{zhangPromptEnhancedSoftwareVulnerability2023,li2023hitchhikers}
%     \item Chain-of-thought prompting~\citep{li2023hitchhikers,zhang2023prompt,davidYouStillNeed2023a}
%     \item Model's understanding of loops, concurrency, unfamiliar functions~\citep{li2023hitchhikers} and AST, CFG, PDG, call graph, pointer analysis, taint analysis, mutant detection, flaky test detection~\cite{maScopeChatGPTSoftware2023}
% \end{itemize}



%%%%%%%% SECOND VERSION
\begin{comment}
% \benjamin{Outline, please use roughly one sentence per bullet point:
% 1. LLMs [cite] have been pretrained on massive corpora of code and are applied in a prompting setting for downstream tasks in SE.
% 2. List the downstream tasks they have been used for: code generation [citation], program repair [citation], etc. Leave vulnerability detection out to discuss in later section; however (now relate to our work), it's not understood whether they can detect vulnerabilities, reason about the code and vulnerabilities in the code.
% 3. Prompting section.
% Emphasize that they are pretrained, and prompting can make a big difference, and that the performance on vulnerability detection is unknown.}

% \benjamin{We will reiterate or move some of the above points to the end of the intro. List of novelty items which we should emphasize:
% \begin{itemize}
% \item We analyze incorrect and correct cases, looking for errors in reasoning.
% \item We analyzed more responses with multiple humans than any other papers (287 compared to other papers: \cite{yu2024security} 82 responses, \cite{nong2024chainofthought} 100 responses, \cite{sun2024llm4vuln} 300 responses from one person then automatic using LLM, \cite{ullah2023large} fully-automatic handling).
% \item We analyzed more diverse models (11 compared to \cite{yu2024security} 3, \cite{nong2024chainofthought} 3, \cite{sun2024llm4vuln} 3, \cite{ullah2023large} 5).
% \item We analyzed code structures linked to problems, which is more detailed than other studies.
% \item We used more objective classification criteria, a more principled method to generate explanations, and a more rigorous agreement procedure, than other studies.
% \end{itemize}
% }

% \new{
% In contrast, we developed a comprehensive categorization which separates the reasons for failure (difficult to determine) from the incorrect claims generated by the LLM.}
% \new{\citet{sun2024llm4vuln} inspected FP and FN cases and categorized into Wrong Reasoning, Need Detailed Analysis, Need Other Code, and Other. They analyzed 300 responses and used an LLM to annotate the rest.}

% \new{\citet{ullah2023large} evaluated GPT-4's summarization of models' reasoning on 228 scenarios by automatically comparing with human-generated reasoning using BLEU, ROUGE, and GPT-4.}
% \new{\citet{yu2024security} analyzed 82 responses, with three people agreeing on the initial codebook based on 20 responses, then one person doing the rest and the others checking. They identified problems based on two taxonomies of general GPT-3.5 issues and one taxonomy of stackoverflow-type code explanations.}
% Nong et al. ~{\cite{nong2024chainofthought}} inspected the 100 random failure cases of three LLMs(GPT-3.5, LLama2, Falcon) and identified four common root causes - insufficient contexts, oblivion of CWE, incomplete control flow analysis, and incomplete data flow analysis. They found that LLMs miss the important control flow facts related to vulnerability during their reasoning and insufficient context of the code snippet is also another dominating reason for the failure cases. Sun et al. \cite{sun2024llm4vuln} analyzed all the false negative and false positive cases of three LLMs (GTP-4, Mistral, and CodeLLama) and found that the significant factor affecting LLMs' vulnerability detection capability is the lack of reasoning capabilities. 
% Ullah et al. ~{\cite{ullah2023large}} investigated the quality of the LLMs(GPT-4, GPT-3.5, CodeLLama-34B, chat-bison, codechat-bison) reasoning and found that LLMs responses are not backed by thorough and correct reasoning in many cases.
% Yu et al.~{\cite{yu2024security}} analyzed the 82 responses of LLMs(Gemini-Pro, GPT-4, GPT-3.5) and identified 16 categories of errors across five themes. Their results indicate that the responses produced by LLMs often suffer from verbosity, vagueness, and incompleteness, highlighting the necessity to enhance their conciseness, understandability, and compliance to security defect detection. We deeply analyzed the errors which occurred in LLM responses from the perspective of vulnerability detection, producing findings reflecting on the fine-grained errors and the syntactic structures which beckoned improvement.

% \commentRelatedwork{
% Comment: 
% \begin{itemize}
%     \item Yu et al. ~{\cite{yu2024security}} I am unsure how to differentiate this from our work. Which of our prompts is close to this one? Contrastive pair? We didn't use the commit message in that setting. Right?
%     \item Sun et al. \cite{sun2024llm4vuln} They only counted the number of wrong reasoning. No fine-grained analysis on the wrong reasoning.
%     \item  Ullah et al. ~{\cite{ullah2023large}} : (for all the responses LLM generated, more than 700+. This number varies based on models as models don't response in many examples. They are not counted for that model.)The analysis is focusing on four aspects: (1) for how many cases does the LLM provide a reasoning for the presence of a vulnerability in a code snippet at all, (2) for how many correct answers the LLM also provides a correct reasoning, (3) for how many correct answers the LLM provides an incorrect reasoning, and (4) for how many answers does the LLM provide the wrong answer, but a correct reasoning.
%     \item Yu et al.~{\cite{yu2024security}}: the last line need to be praphrased.
% \end{itemize}}
\end{comment}

%%%%%%%%%%%%% First version
\begin{comment}
% LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been pre-trained on massive corpora of code and natural language, and applied in many different down streaming tasks in software engineering,
\new{LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been applied in various software engineering tasks,}
such as code generation~{\cite{destefanis_2023_preliminary,dong_2023_self,wang_2023_enhancing}}, code completion~{\cite{code-completion_deng_2023,li_2023_cctest,wang_2023_codet5+}}, code repair~{\cite{automatedbugreplay-icse2024, chenTeachingLargeLanguage2023, repair_cao2023study, repair_wu_2023, repair_islam2024llmpowered, pearceExaminingZeroShotVulnerability2022}}, and \new{code summarization}~\cite{chen_2023_gptutor, nam2024using, code_explanation_macneil_2023, li2023hitchhikers, maScopeChatGPTSoftware2023} through the use of \textit{prompting} -- providing formatted inputs to elicit a response which is applicable to a downstream task.
% Automated Program Repair in the Era of Large Pre-trained Language Models
% 
% Prompt engineering is an integral part of LLM usage. It is the process of searching for the prompt template that results in the most effective performance for a downstream task~\cite{liu_pre-train_2021}.
% A well-structured and domain-guided prompt can significantly enhance performance in a down-streaming task ~\cite{structuredPrompt-1, structuredPrompt-2}.
% The format of the prompt can provide additional information to inform the model's predictions or allow the model to reason about its prediction in sequential steps.
% Several techniques have been proposed, including in-context learning~{\cite{lee2023incontext,rag}}, chain-of-thought~{\cite{cot,kojima2022large}}, tree-of-thoughts prompting~\cite{yao_tree_2024,long2023large} etc.
% 
% 
% 
Effective prompts can condition the model for a specific task like Question/Answer~\cite{gpt3}, provide additional information through in-context examples~{\cite{rag}} and elicit step-by-step reasoning through chain-of-thought examples~{\cite{cot,kojima2022large}}.
\new{We have surveyed these state-of-the-art prompting methods and applied them to the vulnerability detection task.}
% We systematically searched among existing prompting methods and introduced three novel prompting methods: the use of contrastive pairs to select in-context examples, as well as chain-of-thought using examples from CVE descriptions and Static Analysis.
% In this work, we evaluated three of the pre-existing prompting methods and introduced three new prompting methods incorporating domain knowledge,  such as In-context prompting based on contrastive pair, Chain-of-Thought from CVE descriptions, and Chain-of-Thought from static analysis.
% In spite of this progress, it is yet unknown to what extent LLMs can detect software vulnerabilities or reason about vulnerabilities in source code. 

% There are several LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} that are trained to generate code and natural language about the code from both natural language and code prompts.

% MagiCoder ~\cite{magicoder}, Code LLAMA~\cite{codellama}, Gemini-Pro~\cite{gemini}, GPT4 ~\cite{gpt4}, WizardCoder\cite{wizardcoder},  and GPT3.5 ~\cite{gpt3.5} achieved 70.7\%, 67.8\%, 67.7\%,  67.0\%, 57.3\% and 48.1\%  pass@1 score respectively on the code generation of the HumanEval benchmark. 
% Recent works have also used LLMs in many different software engineering down-streaming tasks.
% \benjamin{Too much detail, please summarize ``...different software engineering tasks, such as code generation [citation], program repair [citation], etc.''}
% \citet{xiaConversationalAutomatedProgram2023} propose a fully automated conversation-driven automated program repair tool using ChatGPT, which achieves new state-of-the-art performance on the Defects4j dataset. \citet{pearce2022examining} examine the ability of different LLM models on code repair tasks in zero-shot settings and found that the performance is promising in synthetic and hand-crafted scenarios but is not good enough for real-world examples. \citet{chenTeachingLargeLanguage2023} propose a self-debugging approach via few-shot demonstrations that teaches the LLM models to debug the predicted program. \citet{automatedbugreplay-icse2024} use LLM to automatically reproduce the bugs from the bug reports by leveraging few-shot learning and chain-of-thought reasoning. 
% % Survey prominent LLMs in general, focusing on novel contributions or mechanisms (ChatGPT first LLM, LLAMA open-source, Mixtral mixture of experts).
% % Survey LLMs specifically trained for code, and code generation as the most popular task.

% % \subsection{Prompt engineering for LLMs}

% \benjamin{Outline:
% 1. Define prompt engineering and say it's important because it can improve performance on down-stream tasks. Maybe just cite \citet{liu_pre-train_2021}
% 2. Several techniques have been proposed, including in-context learning~\cite{brown_language_2020,rag,others} and chain-of-thought~\cite{cot,others}.
% 3. Mention and differentiate our work by saying we designed new ways to incorporate in-context examples (contrastive pairs) and CoT (CVE and Static Analysis).}

% \benjamin{let's merge with prior section as this section will be short}
% An integral part of LLMs is prompt engineering, as a slight change in the prompting could have a significant impact on the performance \cite{learningPrompt}.\benjamin{This citation is not very applicable, as it's learning to prompt in vision domain.}
% A well-structured and domain-guided prompt can show a significant performance enhancement in a down-streaming task ~\cite{structuredPrompt-1, structuredPrompt-2}.
% Hence, research on designing different prompt designing paradigms is rapidly growing\cite{structuredPrompt-3}.
% \benjamin{Please merge these two into one short sentence -- see outline.}
% Though directly prompting the models to get the desired response shows promising results in some tasks by using the prior knowledge from the pre-training data, the models face challenges in providing desired output for the unseen contexts ~{\cite{brown_language_2020, fan2023automated}}. To overcome this, Brown et al. \cite{brown_language_2020} utilizes few-shot learning by adapting the context with the few sets of desired input and output. Though few-shot prompting shows efficient performance with some simple tasks, it faces difficulties with the multi-step arithmetic and logical reasoning benchmark ~\cite{rae2022scaling}. Wei el al.~\cite{wei_chain--thought_2023} propose Chain-of-thoughts reasoning, an instance of few-shot-prompting, which replaces the output of the shot examples with the intermediate reasoning steps.

% Survey existing work on developing prompts for LLMs.
% In-context learning, RAG, CoT.

Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as \new{zero-shot} prompting ~{\cite{vulDetIssrew-2023, fu2023chatgpt, hu2023large}}, in-context prompting~{\cite{gao2023far, zhou2024large, liuGptandIncontext2023,chan2023transformerbased}}, and fine-tuning~{\cite{shestov2024finetuning, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized chain-of-thoughts (CoT), such as zero-shot CoT~{\cite{li2023hitchhikers, du2024evaluation, automatedbugreplay-icse2024, chen2023chatgpt, sun2023gptscan} }, Few Shot CoT~{\cite{ullah2023large}}, CoT with Multi-Turn Conversation~{\cite{davidYouStillNeed2023}}, CoT with generic program information such as CFG, DFG, PDG and API call ~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.
% 
% 
In this work, we propose three new prompting methods, such as in-context learning based on contrastive information from bug-fix commits, CoT based on CVE descriptions (CoT-CVE), and CoT based on static analysis (CoT-SA).
Yu et al.~{\cite{yu2024security}} introduce multi-turn conversational CoT, and in the first turn, they ask the LLMs to generate the supplementary code files based on the commit message. The original test code is analyzed for security defects in the second turn. 
Sun et al. ~{\cite{sun2024llm4vuln}} creates a database of the vulnerability report with its corresponding code. During prompting, they retrieve the bug report of the similar code and use the raw/summarized(by GPT 4) report with zero-shot CoT prompting. In our COT-CVE method, we include the CVE descriptions of the examples used along with their Chain-of-Thought responses.

Nong et al. ~{\cite{nong2024chainofthought}} inspected the 100 random failure cases of three LLMs(GPT-3.5, LLama2, Falcon) and identified four common root causes - insufficient contexts, oblivion of CWE, incomplete control flow analysis, and incomplete data flow analysis. They found that LLMs miss the important control flow facts related to vulnerability during their reasoning and insufficient context of the code snippet is also another dominating reason for the failure cases. Sun et al. \cite{sun2024llm4vuln} analyzed all the false negative and false positive cases of three LLMs (GTP-4, Mistral, and CodeLLama) and found that the significant factor affecting LLMs' vulnerability detection capability is the lack of reasoning capabilities. 
Ullah et al. ~{\cite{ullah2023large}} investigated the quality of the LLMs(GPT-4, GPT-3.5, CodeLLama-34B, chat-bison, codechat-bison) reasoning and found that LLMs responses are not backed by thorough and correct reasoning in many cases.
Yu et al.~{\cite{yu2024security}} analyzed the 82 responses of LLMs(Gemini-Pro, GPT-4, GPT-3.5) and identified 16 categories of errors across five themes. Their results indicate that the responses produced by LLMs often suffer from verbosity, vagueness, and incompleteness, highlighting the necessity to enhance their conciseness, understandability, and compliance to security defect detection. We deeply analyzed the errors which occurred in LLM responses from the perspective of vulnerability detection, producing findings reflecting on the fine-grained errors and the syntactic structures which beckoned improvement.

% \benjamin{For these closely related error analysis studies, we need detail into the findings (their conclusions, not just how many categories), extent (did they analyze a lot of responses or just a few case studies, and how many models), and what kinds of errors they investigated in order to set apart our work.}
% \new{\sanjida{Zouh et al.~{\cite{zhou2024large}}  analyzed how effective ChatGPT (GPT3.5 and GPT 4) is with different prompt designs in vulnerability detection compared to baselines where they’ve used CodeBERT as a baseline model. However, in our paper, we are trying to determine the effectiveness of different prompt designs on 11 LLMs. Zhang et al.~{\cite{zhang2023prompt}} investigated the application of ChatGPT in identifying vulnerabilities. Their primary focus lies in improving prompts by incorporating additional information like API calls and data flow, and utilizing chain-of-thought prompting. In contrast, we have introduced a more diverse set of prompts, including Basic (Zero-shot) prompting,n-shot (In-context) prompting, Contrasting pairs, Chain-of-Thought from CVE descriptions, Chain-of-Thought from Static Analysis, which they didn’t consider in \cite{zhang2023prompt}. We have also analyzed the types of mistakes LLMs make when reasoning about vulnerability predictions that are not thoroughly examined in \cite{zhang2023prompt}.}
% }
\end{comment}

%%%%%%%%%%%%%% Starting outline
\begin{comment}
% \new{Starting outline
% \begin{itemize}
%     % \item Several recent studies have initiated investigations into the usage of LLMs for vulnerability detection, using well-known techniques such as basic prompting~\cite{basic-approaches} fine-tuning~\cite{finetune-approaches}, and in-context examples~\cite{incontext-approaches}.
%     % \item Several papers have proposed CoT such as zero-shot CoT, or generic program information such as CFG, others...~\cite{cot-approaches}.
%     % We propose in-context learning based on contrastive information from bug-fix commits and CoT based on CVE descriptions and static analysis
%     \item \citet{LLM4Vuln: A Unified Evaluation Framework for Decoupling and Enhancing LLMs’ Vulnerability Reasoning} evaluated LLMs' reasoning capabilities by broad failure modes; \citet{Security Code Review by LLMs: A Deep Dive into Responses} analyzed responses of LLMs based on a taxonomy of common LLM errors. We deeply analyzed the errors which occurred in LLM responses from the perspective of vulnerability detection, producing findings reflecting on the fine-grained erros and the syntactic structures which beckoned improvement.
% \end{itemize}}


% There are also many works on Vulnerability Detection using LLMs. Some works use Basic prompting with a variety of natural language descriptions, such as ~{\cite{vulDetIssrew-2023, wang2023defecthunter, noeverCANLARGELANGUAGE, bakhshandeh2023using, fu2023chatgpt, cheshkov2023evaluation}}. However, these works didn't evaluate and compare the best natural language description for individual models, while we search for the best natural language for basic prompting for each individual model that help us to evaluate the best capabilities of these models.
% Some works also employ few-shot prompting for their study with different in-context example selection strategies, such as random Selection ~{\cite{gao2023far, zhou2024large}}, retrieved similar examples~{\cite{zhou2024large, mathews2024llbezpeky}. Unlike these works, we analyze the performance of different natural languages with each shot example and employ several retrieval strategies to find the best-performed retrieval method. CoT prompting is also used in a few works ~{\cite{zhangPromptEnhancedSoftwareVulnerability2023, sun2024llm4vuln, davidYouStillNeed2023}}. However, 

% Some works ~{\cite{shestov2024finetuning, chen2023diversevul, yusuf2024instructions}} also fine-tune the LLM models with the Vulnerability Detection data. As fine-tuning is a costly procedure and our research direction for this work is to search for the best prompting and evaluate them, we keep the fine-tuning direction for future work.


% Zhang et al. \cite{zhangPromptEnhancedSoftwareVulnerability2023} study the performance of vulnerability detecting using ChatGPT. They conduct extensive experiments with some basic and chain-of-thoughts prompting by leveraging structural and sequential auxiliary information. Purba et al. \cite{vulDetIssrew-2023} evaulate the performance of four different LLMs (CodeGen, Davinci, GPT-3.5-Turbo, GPT3.5-Turbo-0613) with a set of basic prompting. They found that LLMs don't perform well in vulnerability detection because of the high false positive rate but show promise in identifying subtle patterns commonly associated with different kinds of vulnerabilities. 


% Survey other papers which apply and study LLMs for vulnerability detection.
% Highlight very-closely-related ones and differentiate them from our work.


%%%%%%%%%%%%%% First draft of related work summary
% \benjamin{TODO: Expand related work. Emphasize our novelty.}

% There are several papers which study LLMs for vulnerability detection.
% Some parts of our planned study have been looked at before, though most benchmarks are rather small so some merit may come from running on a larger dataset (on the order of 100-1000 examples).
% However, several techniques/areas have not been studied yet, and most papers do not study LLMs besides ChatGPT or a few related models, so there is some opportunity for our study to bring novelty and impact by being more comprehensive.

% Below is a short list of the most closely related papers, categorized into the techniques which they studied. Keep in mind many of the techniques are studied only on one instance/implementation, but as we have seen, these techniques can be instantiated in diverse ways which affect the performance.
% \begin{itemize}
%     \item Zero-shot prompts~\citep{zhang2023prompt,cheshkovEvaluationChatGPTModel2023a,noeverCANLARGELANGUAGE,bakhshandehUsingChatGPTStatic2023,pearceExaminingZeroShotVulnerability2022}
%     \item $n$-shot prompts~\citep{li2023hitchhikers,fengPromptingAllYou2023}
%     \item Tool use~\citep{li2023hitchhikers,sunWhenGPTMeets2023,fengPromptingAllYou2023}
%     \item Multi-turn conversation~\citep{zhangPromptEnhancedSoftwareVulnerability2023,li2023hitchhikers}
%     \item Chain-of-thought prompting~\citep{li2023hitchhikers,zhang2023prompt,davidYouStillNeed2023a}
%     \item Model's understanding of loops, concurrency, unfamiliar functions~\citep{li2023hitchhikers} and AST, CFG, PDG, call graph, pointer analysis, taint analysis, mutant detection, flaky test detection~\cite{maScopeChatGPTSoftware2023}
% \end{itemize}
\end{comment}

%%%%%%%%% ORIGINAL - FULL CITATIONS
% Remove papers which are both (1) only in arxiv, i.e. unpublished and (2) about smart contract vulnerabilities, since these are pretty distinct from C++ vulnerabilities
\begin{comment}
Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as basic prompting ~{\cite{vulDetIssrew-2023, wang2023defecthunter, noeverCANLARGELANGUAGE, bakhshandeh2023using, fu2023chatgpt, cheshkov2023evaluation, hu2023large}}, in-context prompting~{\cite{gao2023far, zhou2024large, mathews2024llbezpeky, liuGptandIncontext2023,chan2023transformerbased, ma2024lms}}, and fine-tuning~{\cite{shestov2024finetuning, chen2023diversevul, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized CoT, such as zero-shot CoT~{\cite{li2023hitchhikers, du2024evaluation, automatedbugreplay-icse2024, chen2023chatgpt, sun2023gptscan} }, Few Shot CoT~{\cite{ullah2023large}}, CoT with Multi-Turn Conversation~{\cite{davidYouStillNeed2023}}, CoT with generic program information such as CFG, DFG, PDG and API call ~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.
\end{comment}
%%%%%%%%% ORIGINAL - RASEL REMOVED CITATIONS
% Rasel removed this list
% X Primarily trains a SLM, DefectHunter: wang2023defecthunter
% X Primarily PHP and JavaScript: noeverCANLARGELANGUAGE
% X Python only: bakhshandeh2023using
% X Technical report: cheshkov2023evaluation
% X Course project: mathews2024llbezpeky
% X Not vulnerability detection ma2024lms
% X Primarily DiverseVul dataset: chen2023diversevul
\begin{comment}
Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as zero-shot prompting ~{\cite{vulDetIssrew-2023, fu2023chatgpt, hu2023large}}, in-context learning~{\cite{gao2023far, zhou2024large, liuGptandIncontext2023,chan2023transformerbased}}, and fine-tuning~{\cite{shestov2024finetuning, yusuf2024instructions, yang_2024_large}}.
Several papers have proposed chain-of-thoughts (CoT), such as ``Let's think step-by-step''~{\cite{li2023hitchhikers, du2024evaluation, automatedbugreplay-icse2024, chen2023chatgpt, sun2023gptscan} }, multi-step prompts~{\cite{davidYouStillNeed2023,ullah2023large,yu2024security}}, and utilizing generic information such as CFG, DFG, PDG and API calls ~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.
\end{comment}
% 
% 
%Concurrent to our CoT-CVE, Sun et al. ~{\cite{sun2024llm4vuln}} also found that the original bug reports were not helpful. 

%In contrast, we developed error categories specifically tailored for vulnerability detection, analyzed the code structures which affected the correctness of LLMs, and analyzed explanations of both correct and incorrect predictions.


%To the best of our knowledge, our work represents the most comprehensive analysis of LLM errors in vulnerability detection.




==> _OldVersion.ICSE25/Sections/50.relatedwork.tex <==
\section{Related Work}
\label{sec:related-work}

% \subsection{Large Language Models for Software Engineering}
LLMs~\cite{gpt4, gemini, wizardcoder, gpt3.5, starchat, starcoder, mistral, mixtral, magicoder} have been applied in various software engineering tasks, such as code generation~\cite{humaneval}, test generation~\cite{lemieux_testgen}, and code summarization~\cite{ahmed2024automatic}
% , and program repair~\cite{xia_apr},
through the use of prompting.
Effective prompts can condition the model for a specific task like Question/Answer~\cite{gpt3}, provide additional information through in-context examples~{\cite{rag}} and elicit step-by-step reasoning through chain-of-thought examples~{\cite{cot,kojima2022large}}.
We have surveyed these state-of-the-art prompting methods and applied them to the vulnerability detection task.

% \subsection{LLMs for Vulnerability Detection}
Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as zero-shot prompting ~{\cite{vulDetIssrew-2023, fu2023chatgpt}}, in-context learning~{\cite{gao2023far,liuGptandIncontext2023,chan2023transformerbased}}, and fine-tuning~{\cite{shestov2024finetuning, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized chain-of-thoughts (CoT), such as ``Let's think step-by-step''~{\cite{li2023hitchhikers, automatedbugreplay-icse2024,sun2023gptscan}}, multi-step prompts~{\cite{ullah2023large,yu2024security}}, and generic information such as CFG, DFG, PDG, and API calls~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.
In this work, we propose three novel prompt approaches tailored for vulnerability detection, integrating information from bug-fix commits (contrastive pairs), CVE descriptions (CoT-CVE), and static analysis reports (CoT-SA). We reported the capabilities of LLMs to distinguish buggy and patched versions of code.

Several concurrent papers have taken initial steps to analyze errors in LLM-generated vulnerability detection responses (\wei{to the best of our knowledge}, the papers are in arXiv but not yet published).
\newtwo{\citet{yu2024security} analyzed 82 responses and identified problems based a taxonomy of errors in ChatGPT responses to StackOverflow and general-purpose queries}, corroborating our findings that the models struggled with  correctness, logic and consistency.
\citet{nong2024chainofthought} categorized 100 incorrect predictions from GPT-3.5 into {\it Insufficient Context}, {\it CWE Oblivion}, {\it Incomplete Control Flow/Data Flow}; similarly, \citet{sun2024llm4vuln} used an LLM guided by 300 human annotations to categorize incorrect predictions into  {\it Wrong Reasoning}, {\it Need Detailed Analysis}, {\it Need Other Code}, and {\it Other}.
\citet{ullah2023large} automatically compared GPT-4's summarization of LLM reasoning with human-generated reasoning based on BLEU, ROUGE, and GPT-4.

Our error classifications provide more fine-grained categories than prior work (see \Cref{tab:fine-grained}) \newtwo{and allow us to analyze the code structures which affected the correctness of explanations,} and thus potentially provide better guidance for future improvement of LLMs for vulnerability detection. We provide a quantitative comparison of LLMs and human's performance on locating bugs. To the best of our knowledge, our work is the most comprehensive: \newthree{compared to prior works, }we analyzed more models (11), and used multiple raters \newthree{with a rigorous agreement protocol based on Fleiss' $\kappa$} to manually annotate a larger set of 287 LLM responses.

==> _OldVersion.ICSE25/Sections/60.conclusion.tex <==
\section{Conclusions}
We comprehensively evaluated the vulnerability detection capabilities of LLMs from the standpoint of their performance as well as their errors.
We found that they performed only slightly better than random guessing (0.5-0.63 Balanced Accuracy), and that they struggled to differentiate buggy and fixed code versions, making the same prediction for 76\% of pairs.
We proposed CoT from Static Analysis and Contrastive pairs, which improved the performance of some models.
% We proposed several prompt templates based on Contrastive Pairs, CoT from CVE Descriptions, and CoT from Static Analysis, which improved the performance of some models compared to basic prompting.
LLMs frequently made Code Understanding, \wei{Common Knowledge}, Hallucination, and Logic errors when explaining vulnerabilities, with 57\% of responses containing errors.
On complex debugging tasks from DbgBench, LLMs performed far worse than humans, correctly localizing only 6/27 bugs.
These findings highlight LLMs' limitations in vulnerability detection and our dataset of LLM errors provides guidance for future improvement of LLM-based vulnerability detection.


==> _OldVersion.ICSE25/Sections/99.next-steps.tex <==
\section{Next steps}

Pursuant to these initial results, we hope to evaluate the models on a larger dataset, up to the entire SVEN dataset, and evaluate a larger set of models, using the prompting techniques we have explored.

There are several prompting techniques which we have not yet explored, broadly:
\begin{itemize}
    \item Tool use, i.e. providing chat models with tools to:
    \begin{itemize}
        \item Retrieve function definitions
        \item Retrieve similar code \& API usages
        \item Slice code
        \item Query control and data dependence relationships
        \item Run lightweight static analysis
    \end{itemize}
    \item Agentic behaviors, such as:
    \begin{itemize}
        \item Tree-of-thoughts~\cite{tot} and ReAct~\cite{react}.
        \item Ensembling~\cite{ensemble-llm} and Mixture-of-experts~\cite{moe}.
    \end{itemize}
\end{itemize}


==> _OldVersion.ICSE25/Sections/99.outline.tex <==
\section{Future section: Error Analysis and LLM Reasoning analysis}

Prediction (week 1)

\begin{itemize}
    \item What kind of examples in the prompt help most? On what types of programs does the model easily make mistakes?
    \begin{itemize}
        \item Short examples may be easier?
    \end{itemize}
    \item How often does the model reason?
    \item How often is the model's reasoning correct?
    \item What kinds of mistakes does the model frequently make in its reasoning?
    \begin{itemize}
        \item Is the question in the query ambiguous? Does the model answer a different meaning of ``bug''? \textbf{[Ben]}
        \item Is the model's reasoning self-consistent? \textbf{[Ben, Rasel]}
        \item Does the model give a clear answer to the question? \textbf{[Ben]}
        \item Does the model reason about the in-context examples rather than the query? \textbf{[Rasel]}
        \item Does the model reply ``I don't know''? Does it have sufficient information to make a decision?
        \item Are model predictions biased towards one class?
        Is it related to adding more examples on StarCoder as Roy presented? \textbf{[Roy]}
        \item Are the correct predictions of the examples actually "correct"? (Reasoning) \textbf{[Roy]}
    \end{itemize}
\end{itemize}

patterns of seeds 
\begin{itemize}
\item seeds disagree with the conclusions, \item there disagree with the different types
\item copy the prompt
\end{itemize}

=============

Obviously reasoning errors (week 2) 

\begin{itemize}
    \item What information was collected?
    Error classes
    bug localization/type
    \item Process of collecting the errors
    \begin{itemize}
        \item 3 raters
        \item agreement score
        \begin{itemize}
            \item Raw score: 0.2079, exact match: 26\%
            \item Applying majority rule changed 58\% of rows, but only 125/2184=5.7\% of ratings
            \item Agreement after majority rule is 0.7490, exact match: 83\%
        \end{itemize}
        \item resolve by majority, then discussion (how many were manually resolved?)
    \end{itemize}
    \item Prevalence of errors by model
    \begin{itemize}
        \item Show bar chart
    \end{itemize}
    \item Strict performance measurement: out of correct predictions, show extra bars on a bar chart for ``strict'' performance.
    \begin{itemize}
        \item How often does the type/location match?
        \item How often is there a reasoning error?
    \end{itemize}
    \item Discussions
\end{itemize}

\subsection{Patterns in error prediction: error analysis}

\subsection{LLMs versus humans for vulnerability detection task}


==> _OldVersion.ICSE25/Sections/complete-list-of-citation.tex <==
% Complete list of citations
Recent studies have initiated investigation into the usage of LLMs for vulnerability detection, using well-known techniques such as basic prompting ~{\cite{vulDetIssrew-2023, wang2023defecthunter, noeverCANLARGELANGUAGE, bakhshandeh2023using, fu2023chatgpt, cheshkov2023evaluation, hu2023large}}, in-context prompting~{\cite{gao2023far, zhou2024large, mathews2024llbezpeky, liuGptandIncontext2023,chan2023transformerbased, ma2024lms}}, and fine-tuning~{\cite{shestov2024finetuning, chen2023diversevul, yusuf2024instructions, yang_2024_large}}.
Several papers have utilized CoT, such as zero-shot CoT~{\cite{li2023hitchhikers, du2024evaluation, automatedbugreplay-icse2024, chen2023chatgpt, sun2023gptscan} }, Few Shot CoT~{\cite{ullah2023large}}, CoT with Multi-Turn Conversation~{\cite{davidYouStillNeed2023}}, CoT with generic program information such as CFG, DFG, PDG and API call ~{\cite{zhang2023prompt, nong2024chainofthought, khare2023understanding, ullah2023large}}.



==> _OldVersion.ICSE25/Sections/error-analysis-old.tex <==

% 
%We also extracted the bug type and locations identified by the model.

% we fed in exactly the same prompts as described in Section \ref{sec:rq1}, appending the categorical response given by the model and the message, ``Please explain the reasoning for this answer''.
%we fed in exactly the same prompts as described in Section \ref{sec:rq1}, followed by the model's categorical response, then ``Please explain the reasoning for this answer''.we further prompted using xxxx

%In order to understand what types of mistakes LLM makes to explain the vulnerabilities. We manually inspect the output and based on our initial inspection, and classified the answers 

% We propose as a next step to deeply investigate the predictions of these models to understand why they performed so badly.
% In order to understand LLM predictions more deeply than the surface-level performance metrics, we comprehensively and rigorously classified and analyzed errors and information occurring in the outputs of the LLMs.
%Next, we deeply investigated the predictions of these models to understand the reasons for their poor performance.
% We comprehensively classified the reasoning errors and fine-grained predictions which occurred in LLM responses.

% \paragraph{Prompting for reasoning and analyzing errors}

% We prompted the LLMs to explain the reasoning for their vulnerable predictions, then manually analyzed the model outputs to categorize the \textit{reasoning errors} and \textit{fine-grained predictions} produced by the model.
% \textit{Reasoning errors} refer to factual inaccuracies, faulty logic, or unreasonable assumptions which occur in LLM reasoning, which we define below.
% \textit{Fine-grained predictions} identify the bug type and location predicted by the model, beyond a binary classification as vulnerable or non-vulnerable.

% To generate reasoning, we fed in exactly the same prompts as described in Section \ref{sec:rq1}, appending the categorical response given by the model and the message, ``Please explain the reasoning for this answer''.
% We only generated reasoning for the examples where the LLM predicted vulnerable.
%We excluded non-vulnerable predictions, since the LLM did not detect the vulnerability, and any vulnerable examples where the LLM refused to produce a coherent explanation.
% In order to avoid confusion about the instructions, we rephrased the model's response to give the same vulnerability prediction in a fixed format similar to ``Yes, the function is vulnerable'' or ``No, the function is not vulnerable'', but removed further elaboration present in the original response.

% Based on our observations from the prior experiments, we defined a set of reasoning errors, with the goal that each intuitive ``mistake'' inside an LLM's response can be unambiguously assigned a category. A single response can contain multiple distinct errors.
% \textit{Code understanding} errors are incorrect assertions about programming language semantics, code structures, or effects of statements.
% \textit{Common knowledge} errors are assumptions which are unlikely when considering common knowledge about the application, environment, or conventions.
% \textit{Logic} errors are incorrect logical implications or logical contradictions between statements.
% \textit{Hallucination/Memorization/Repetition} errors are artifacts specific to LLM outputs, including hallucination (stating information that sounds correct but is not present in the prompt), memorization (memorizing information from the training data verbatim), and repetition (infinitely repeating text sequences).
% \benjamin{This can be pared down}
% \textit{Code understanding} errors are incorrect assertions about the programming language semantics, presence of code structures, or the effects of statements in the code, such as order of statement execution, check operations, memory allocations, or string operations.
% \textit{Common knowledge} errors are assertions which are the raters believe are rendered unlikely based on common knowledge about the application, execution environment, and common conventions, such as common assumptions on called functions, side-effects of standard library functions, or reasonable assumptions about configuration or global variables.
% \textit{Logic} errors are incorrect logical implications or contradictions between two statements in a single response. As an example, if the model says ``the statement is checked'', then later says ``the statement is not checked'', we consider it a logical contradiction; if the model says ``$P$ is true, therefore $Q$'' where $Q$ does not follow from $P$, we consider it a faulty logical implication.
% \textit{Hallucination/Memorization/Repetition} errors are common artifacts which are specific to LLM outputs. Hallucinations are statements which are not reflected in the code given to the model~\cite{citation-needed}. Memorization is a phenomenon where the model can recall specific information about the program under observation that occurs in its training data~\cite{citation-needed}. Repetition is a phenomenon where the LLM repeats some sequence of text infinitely (until it runs out of context budget)~\cite{citation-needed}.

 %\benjamin{Give some examples, such as bounds check, null check, overflow, control flow.}
% These errors included some describable patterns, such as the following:
% These errors can lead to misleading explanations, as shown in the following:

% \begin{itemize}
%     \item \textbf{Missing Check:}
%     % LLMs commonly claimed that an index or pointer was not checked before use, and could lead to a buffer overflow or null-pointer dereference, when in reality the code contained the check. This error occured in \textcolor{red}{23\%} of model responses.
%     Figure \ref{fig:bounds-check-example} shows an example of a model response which flags an unchecked null-pointer dereference, presumably at line 5 \texttt{p->lineinfo[oldpc]}, even though \texttt{p->lineinfo} is checked at line 2.
%     This error lead to false positives, especially after the bug is fixed by adding such a check.
%     % \benjamin{This also happens for checking buffer length and index range.}

%     % \item \textbf{Incorrect Control-flow:} LLMs commonly claimed that an error could occur when a program executes a statement $A$, then another statement $B$. However, in many cases, such control flow cannot occur; either $B$ always executes before $A$, or a jump occurs between $A$ and $B$ under the conditions which would cause the bug.
%     % This error occured in \textcolor{red}{4\%} of model responses.

%     % In Figure \ref{fig:integer-math-example}, the model flags a potential use-after-free inside a loop defined by the macro \texttt{list\_for\_each\_entry\_safe}, presumably referring to the dereference at line 10 \texttt{rdev->ena\_pin->gpiod} and the free of \texttt{pin} which is matched with \texttt{rdev->ena\_pin} at line 15, but since the function returns (line 17) after freeing \texttt{pin} (line 15), this dereference will not occur after \texttt{rdev->ena\_pin} is freed.
    
%     % This may occur due to the transformer architecture's limited ability to discern ordering of statements with the positional embedding, or the one-directional nature of causal language modeling. Our findings in the domain of vulnerability detection align with reports of similar shortcomings from \citet{allamanis-recent-paper,kexin-program-invariants,related-work-on-control-flow}.
    
%     \item \textbf{Incorrect reasoning about Integer Math:}
%     In Figure \ref{fig:integer-math-example}, 
% \end{itemize}

% StarChat-$\beta$ and StarCoder had more hallucination and repetition errors than other models.
% This may reflect on their pretraining regime, since they have the same base model.
% These errors included the following:
% 
% \begin{itemize}

% \textit{Hal/Mem/Rep} occurred in 8.7\% of responses.

% The models' responses contained reasoning errors more often than not, producing reasoning that was inconsistent at best (resulting in confusion for the user) and incorrect at worst (resulting in incorrect understanding for the user).

% \benjamin{
% Write up more about Fig 4.
% Write up fine-grained error types.
% }

% \wei{Focus on descriptive statistics, not just specific examples. Focus on the errors related to code features -- fine-grained errors under code understanding.
% What kinds of code features do LLMs struggle to understand correctly? Focus on the data under code understanding.
% Add a table with the percentages of each fine-grained error pattern, from the most confident rater's output.}

% \begin{figure}[htbp]
%     \centering
%     \caption{Example of \textbf{TYPE}.} \label{fig:XXX-example}
%     \begin{tcolorbox}[title=\textbf{Source code} (Example XX/non-vulnerable),colframe=Periwinkle]
%     \begin{minted}
%     [
%     frame=lines,
%     numbersep=2mm,
%     breaklines=true,
%     fontsize=\footnotesize,
%     highlightlines={2,5},
%     highlightcolor=yellow,
%     linenos,
%     tabsize=2,
%     ]
%     {c}

%     \end{minted}
%     \end{tcolorbox}
%     \begin{tcolorbox}[title=\textbf{Model response} (MODEL)]
    
%     \end{tcolorbox}
% \end{figure}

\sethlcolor{yellow}
Out of the \textit{Hal/Mem/Rep} category, the most common case was hallucination, where the LLM produced reasoning based on code not represented in the prompt.
Figure \ref{fig:hallucination-example} shows an instance where LLAMA 2 explains a potential integer overflow in a formula which does not occur in the function.
% The second most-frequent error in this category was \textit{Repetition}, where the LLM generates identical text which repeats infinitely. Figure \ref{fig:repetition-example} shows an example.

% \item \textbf{Hallucination:} The LLM's output refers to code that does not exist. This can occur because the discussion about the code would be statistically likely, even though it does not match the source material~\cite{need-citation}. This can mislead the developer trying to understand the reason for the vulnerable prediction.
% Figure \ref{fig:hallucination-example} shows an instance where LLAMA 2 explains a vulnerability prediction using a formula which does not occur in the function.
% \item \textbf{Repetition:} The LLM's output contains identical text which repeats infinitely. This can occur because the model gets ``stuck in a loop'', where the most likely next token is always the next token in the sentence or the repetition of the first token in the sentence~\cite{need-citation}. This can cause confusion for the developer trying to diagnose the detected vulnerability.
% Figure \ref{fig:repetition-example} shows an example where StarCoder repeats its prediction without limit until it generates the maximum amount of output.
% \end{itemize}

% \input{Figures/error-examples/logical-implication}

% \input{Figures/error-examples/logical-contradiction}

% Also occurring frequently was ``Logic error'', which occurred in \textcolor{red}{10\%} of responses.
% These errors included the following:

% \benjamin{Removed ``logic error'' examples in order to avoid showing too many examples, because they're not as frequent.}
% We also observed \textit{Logic} errors in 6.6\% and 3.5\% of responses, respectively.
% \begin{itemize}
%     \item \textbf{Faulty Logical Implication:} The LLM's stated reason for a vulnerable prediction contains an implication which does not follow. This error occured in \textcolor{red}{6\%} of model responses.
%     In Figure \ref{fig:logical-implication-example}, LLAMA 2's response states that \textit{if} \texttt{init\_get\_bits8} returns a negative value, \textit{then} \texttt{ff\_ac3\_parse\_header} will try to dereference a null pointer; however, this implication cannot follow because a negative return value will cause the function to return on line 6 before calling \texttt{ff\_ac3\_parse\_header}. This specific error occurred due to incorrect reasoning about the control flow of the program.
%     \item \textbf{Logical Contradiction:} The LLM's response contains two or more statements which cannot both be true.
%     This can cause confusion for the developer trying to utilize the LLM's reasoning. This error occured in \textcolor{red}{4\%} of model responses.
%     Figure \ref{fig:contradiction-example} shows WizardCoder's response which first states that \texttt{output\_len} is checked, then claims that \texttt{output\_len} is not checked and will cause a bug.
% \end{itemize}

% \benjamin{Given space, we may include others:
% Logical implication errors, Pattern matching errors,
% “Reading comments” errors,
% Repetition, Memorization, Anchoring errors.
%     % \item Control flow order errors, 
%     % \item “Missing the bounds check” errors,
% }
% \wei{Let's show more examples and strengthen this part, shortening the prompt methodology, to distinguish our work from many others reporting only the performance.}

%{RQ3 results: Revisiting model performance}

% \benjamin{Perhaps we will make an RQ for this analysis.}


% Because we have found that the LLM responses often contain errors, we want to understand the quality of the models with stricter requirements on the concept of ``correctness''. We can further investigate model correctness on vulnerable examples using the fine-grained prediction data from our error analysis. We consider the following four sets of constraints:

% \begin{itemize}
%     \item \textbf{Correct Prediction:} The binary prediction matches the label (vulnerable/non-vulnerable).
%     \item \textbf{Correct Bug Type:} One or more of the bug types flagged by the model matches the type documented in the ground-truth.
%     \item \textbf{Correct Location:} One or more of the locations flagged as related to the vulnerability match the locations changed in the bug-fixing patch.
%     \item \textbf{Correct Reasoning:} We observed no errors in the model's reasoning response.
% \end{itemize}

\input{Figures/error-analysis/fine-grained-predictions}

In Figure \ref{fig:strict-performance}, we present the the models' capability to further explain vulnerabilities by predicting the type of vulnerability, its location, and its root cause.
\textit{Prediction}: the model's binary prediction matches the label (vulnerable/non-vulnerable).
\textit{Bug Type}: the bug type predicted by the model matches the ground-truth bug type.
\textit{Location:} a location which the model mentioned as related to the vulnerability matches the locations changed in the bug-fixing patch.
\textit{Cause:} we observed no reasoning errors in the model's reasoning about the root cause.
We consider an example correctly labeled if all selected explanations are true.
% , and we report Accuracy instead of Balanced Accuracy since we only consider vulnerable predictions.
% ; for instance, the bar \textit{Prediction + Bug Type + Location} shows the proportion of examples where the model predicted the binary prediction, type, and the location correctly.
% 
Although most LLMs predicted correctly on up to 79\% of vulnerable examples (blue bar), correctness dropped substantially when the predicted location, bug type, and reasoning errors in the root cause were considered.
Considering both bug types and locations (orange bar), all models dropped in correctness, decreasing by 18-67\%, with Mistral failing on all examples.
Considering root-cause explanations with reasoning errors as incorrect (purple bar), model performance decreased by 24-50\%.

% Next, we evaluated the models with stricter requirements on the concept for correctness, using the fine-grained prediction data from our error analysis. We consider the following four sets of constraints.
% \textit{Correct Prediction:} The model's binary prediction matches the label (vulnerable/non-vulnerable).
% \textit{Correct Bug Type:} A bug type predicted by the model matches the ground-truth bug type.
% \textit{Correct Fix Location:} A location which the model mentioned as related to the vulnerability matches the locations changed in the bug-fixing patch.
% \textit{Correct Reasoning:} We observed no reasoning errors in the model's reasoning response.
% Most LLMs predicted with relatively high accuracy considering only the binary prediction and bug type, but the accuracy dropped substantially when three or all four constraints were considered.
% Additionally, some models which performed well regarding binary prediction only could not perform well when considering both prediction and bug type, such as MagiCoder and StarCoder; these models often flagged types of bugs which were unrelated to the ground-truth, such as functional or error-handling bugs.
% This indicates that while the models could flag vulnerable functions, they failed to isolate the precise lines containing the vulnerabilities and isolate the vulnerabilities labeled in the dataset. This limits their immediate applications for drop-in static analysis replacements and motivates future work to improve these areas.

==> _OldVersion.ICSE25/Sections/performance-eval-old.tex <==

% }
% }

% \benjamin{This section can be pared down}
% Zero-shot prompt modifications such as Q/A and CWE-list substantially changed the model's behavior;
% eight out of eleven models had higher performance with either Q/A or CWE modifications than on the basic query.
% Embedding search and chain-of-thought techniques were beneficial; on LLAMA 2 and GPT-4, Embedding performed better than In-context by a small margin, and on MagiCoder, CoT-SA performed substantially better than the other approaches on average; therefore, these approaches can indeed boost the overall best performance of some models.
% On the other hand, CoT-CVE consistently underperformed compared to the other prompting methods and performed worse than the random baseline on six out of eleven models, indicating that our implementation of this approach was not overall helpful; future work could explore the usage of other rich information available in bug reports.
% \benjamin{TODO-NOW: CoT outperformed incontext only in Magicoder, Mistral, and Mixtral and Embedding << incontext in 8 other models. How to explain this?}
% 
% \benjamin{WIP}
% \benjamin{Did contrasting pairs work? Did CoT work?}
% Contrasting pairs were rarely helpful in boosting model performance. Compared to naive selection approaches, contrasting pairs performed better in only 40\% of cases and only one model performed best with contrasting pairs. This suggests that naively including both vulnerable and non-vulnerable versions of examples is not helpful; we propose that perhaps future work can leverage bug-fixes in alternative ways, such as using the bug-fixes to highlight critical vulnerable regions of the in-context examples.


% \benjamin{TODO-NOW: Conclusions? Information or examples in CoT is important?}

% Commented out, redundant with the plot
% For all the models except for GPT-3.5, the zero-shot prompting method performed as well or better than a hypothetical baseline which randomly selects ``vulnerable'' or ``non-vulnerable'' (since the classes are balanced, we expect $\text{Balanced Accuracy} = 0.5$).
% Most models, such as StarChat-$\beta$, GPT-4, and LLAMA 2, performed consistently better when given in-context examples; however, the performance varied among different in-prompting approaches, showing that there was no one approach to fit all models (different models performed better with different types of information).
% Other models, such as Mixtral-MoE, WizardCoder, and Code LLAMA, performed better with basic prompts.
% These results show that in order to get the optimal performance, researchers applying LLMs for vulnerability detection should explore using in-context examples and various prompting methods.

% \input{Figures/performance-eval/best-prompt-distribution}

% The variance among three random seeds was large for some prompts.
% % \benjamin{TODO-NOW: Continue}
% This confirms the intuition that, to faithfully evaluate the LLMs, nondeterminism is a major factor




% Notably, more models performed better on the unpaired data with Basic prompts and with contrastive pairs.
%These results underscore the conclusion that SOTA LLMs were not able to perform well for vulnerability detection.
% Several models, such as LLAMA 2 and Code LLAMA, performed better on the unpaired data, while other models, such as StarCoder and StarChat-$\beta$, performed worse.


% Explain the bad performance
%The suboptimal performance could be attributed to prediction bias,


% \rasel{GPT-4, Mixtral-MoE, Mistral is missing in the following description. Make it clear that the point is to say humaneval score is reversed.}
% According to Balanced Accuracy, StarChat-$\beta$, StarCoder, and MagiCoder were among the best-performing models for vulnerability detection, while WizardCoder, Code LLAMA, and Gemini were among the worst-performing. These results reverse the models' HumanEval $Pass@1$ score and suggest that the models' high code generation performance is not necessarily linked to high vulnerability detection ability.

% \new{

% }

% \benjamin{This section can be cut}
% Gemini performed poorly, evidenced by performance near to the random baseline. Its predictions were severely biased towards always predicting either vulnerable or non-vulnerable predictions depending on which prompt was used, showing that it was not able to differentiate between vulnerable and non-vulnerable programs.

% \benjamin{This section can be cut}
% Several models (LLAMA 2, WizardCoder, Code LLAMA) earned Precision near to 0.5, indicating that their ``vulnerable'' predictions were no better than random guesses. This shows that these models had special difficulty in precisely detecting the vulnerable functions.
% Other models (StarCoder, Mixtral-MoE, MagiCoder, GPT3.5, Mistral) had higher Precision, but low Recall -- between 0.1 and 0.3. These models were biased towards non-vulnerable predictions, so while their vulnerable predictions were more often correct, they often missed the vulnerable functions.
% StarChat-$\beta$ was the only model with both Precision and Recall substantially above the random-choice baseline.

% \Roy{Writing up the paired analysis section}\\
%\subsubsection{Evaluation on Bug-fix Pairs}
% In this section, we will discuss the performance of LLMs on paired examples. By pair, we mean vulnerable and patched versions of an example code snippet. We aim to analyze how the models perform on each pair of examples. To analyze the performance of LLMs on paired examples, we categorize each pair into one of the following four categories:

%yes Investigating further, we analyzed the models' predictions on paired versions of code before and after the bug-fixing commits.
% The SVEN dataset is made of bug-fixing patches -- paired versions of the source code where the ``before'' version includes the vulnerability and the ``after'' version applies the changes which fix the vulnerability.
% yes The two versions differ primarily on the portions which were changed to fix the vulnerability.
\mycomment{
We aim to analyze whether the LLM can distinguish the vulnerable and non-vulnerable source code, given these precise differences.

Given the LLM's responses on each version, we categorize each pair into one of the following four categories:

\begin{enumerate}
    \item \textbf{Both Wrong}: The model incorrectly predicts both the vulnerable and buggy versions.
    
    \item \textbf{Both Correct}: The model correctly predicts both the vulnerable and buggy versions.
    
    \item \textbf{Can't Distinguish}: The model predicts the same label for both versions. This results in predicting one version correctly and one incorrectly.
    
    % \item \textbf{Both Correct (Strict)}: The model gives correct predictions on vulnerable and buggy examples and additionally predicts the correct bug type and location on the vulnerable code version.
\end{enumerate}
}




\mycomment{
The models generally failed to distinguish the buggy and fixed versions, with 
They predicted both ``before'' and ``after'' correctly in only 15\% of pairs (Both Correct) and predicted both versions incorrectly on 7\% of pairs (Both Wrong).
%, and the models' predictions matched the ground-truth bug-type and fault location on only 3\% of pairs which were predicted vulnerable.
% The models generally failed to differentiate between the ``before'' and ``after'' versions of a bug-fixing patch.
These findings highlight the limitations of the models' capabilities in making nuanced and precise vulnerability detection predictions.
StarChat-$\beta$, the highest-performing model by Balanced Accuracy, had the fewest ``Cant-Distinguish'' pairs.
In contrast, Mistral was severely biased towards predicting non-vulnerable and only predicted 3 examples as vulnerable.
}
% Table \ref{tab:pair-performance} presents the results of the best-performing prompts for each model.
% The models frequently predicted both versions with the same label, with 78\% of paired predictions resulting in Can't Distinguish.
% The models predicted both ``before'' and ``after'' correctly in only 15\% of pairs (Both Correct) and predicted both versions incorrectly on 7.2\% of pairs (Both Wrong).%, and the models' predictions matched the ground-truth bug-type and fault location on only 3\% of pairs which were predicted vulnerable.
% The models generally failed to differentiate between the ``before'' and ``after'' versions of a bug-fixing patch. These findings highlight the limitations of the models' capabilities in making nuanced and precise vulnerability detection predictions.
% StarChat-$\beta$, the highest-performing model, had fewer ``Cant-Distinguish'' pairs, showing that it differentiated between buggy and fixed versions.
% In contrast, Mistral was severely biased towards predicting non-vulnerable and only predicted 3 examples as vulnerable (but predicted these correctly), representing a highly-specific vulnerability classifier.
% \benjamin{TODO: Connect this to the performance plot above, showing why some models did not perform well on the dataset -- predicted Same a lot or got Both Wrong a lot.}
% Models frequently predict “Same”
% “Both correct strict” is difficult
% “Both wrong” is not uncommon

% Other than Both-SC, we could map each pair to the correct category automatically by parsing the model's output. However, to determine the capability of the models to figure out the bug type and location correctly, we have inspected the model's response manually by 3(three) different raters independently. Since, in many cases, models tend to generate responses without any reasoning, we collected the responses where the model gave predictions with reasoning. Models like GPT3.5 and Gemini didn't generate reasoning, hence, they were excluded from the raters' study.\\

% Table IV presents the results of the paired data analysis on the collated dataset.
% The table shows that the models exhibit various degrees of performance across the fine-grained categories. For instance, models like codellama, llama2, and starchat-beta wizardcoder indicate relatively high accuracy in predicting both examples correctly (Both-C).
% These models also show some capability in predicting the bug type and patch location (Both-SC), with starchat-beta topping the list for this category.
% Additionally, The most interesting observation is that the models tend to provide the same prediction for most of the pairs, which indicates the need for more understanding and differentiation between the two versions of the code by all of these models.

% Now, moving to Table V, which shows the results of the error analysis dataset. Error analysis dataset is a subset of the collated dataset, containing examples where the models outputted both prediction and reasoning. On these smaller sets of reasoning examples, we can see that, even when the models are giving predictions with reasoning, they still fail to differentiate between vulnerable and patched versions, consequently predicting the same thing for both versions. The other 3(three) category results are also similar in the error analysis dataset, from which we can conclude that, even if the LLM models generate responses with reasoning, the overall performance remains consistent across all the categories in the error analysis dataset.\\

% \Roy{End of paired analysis discussion}\\

% \input{Sections/32.shots}
% \input{Sections/33.reasoning}

% \paragraph{Results: Other findings and discussions}
% % Some other findings which we found in our experiments:

% \benjamin{This section will likely be moved to a ``discussion'' section grouping all the minor findings.}

% \begin{enumerate}
    % \item Zero-shot prompt modifications such as Q/A and CWE-list can change the model's behavior substantially, even with small modifications.
    % Seven out of eleven models had higher performance with either Q/A or CWE modifications.
    % \item CoT-CVE performed the worst out of all the prompting methods and performed worse than the random baseline on five out of ten models, indicating that this approach was not overall helpful; however, perhaps some future work could explore the usage of other rich information available in bug reports.
    % \item Contrasting pairs did not boost the performance. Compared to naive selection approaches, contrastive pairs performed better in only 40\% of cases. This suggests that naively including both vulnerable and non-vulnerable versions of examples is not helpful; we propose that perhaps bug-fixes can be leveraged in alternative ways, such as using the bug-fixes to highlight critical vulnerable regions in in-context examples.
%     \item Model predictions varied substantially among different random seeds, with a standard deviation of up to 0.05 among three random seeds, so it is important to account for this variability when comparing different settings.
% \end{enumerate}


==> _OldVersion.ICSE25/macros.tex <==
% \newcommand{\benjamin}[1]{\textcolor{Bittersweet}{[Ben]: #1}}
% \newcommand{\wei}[1]{{\color{red} #1}}
% \newcommand{\earl}[1]{\textcolor{JungleGreen}{[Earl]: #1}}
% \newcommand{\Roy}[1]{\textcolor{blue}{[Roy]: #1}}
% \definecolor{ddw}{cmyk}{0, 0.7808, 0.4429, 0.1412}
% \newcommand{\rasel}[1]{\textcolor{ddw}{[Rasel]: #1}}
% \newcommand{\sanjida}[1]{\textcolor{violet}{[Sanjida]: #1}}
% \newcommand{\new}[1]{\textcolor{RubineRed}{#1}}
% \newcommand{\newtwo}[1]{\textcolor{PineGreen}{#1}}
% \newcommand{\newthree}[1]{\textcolor{blue}{#1}}
% \newenvironment{newenv}{\color{RubineRed}}{\ignorespacesafterend}
% \newcommand{\wip}{\textcolor{red}{[WIP]}}
% \newcommand{\commentRelatedwork}[1]{\textcolor{blue}{#1}}

% Decolor all
\newcommand{\benjamin}[1]{\textcolor{black}{#1}}
\newcommand{\wei}[1]{\textcolor{black}{#1}}
\newcommand{\earl}[1]{\textcolor{black}{#1}}
\newcommand{\Roy}[1]{\textcolor{black}{#1}}
\newcommand{\rasel}[1]{\textcolor{black}{#1}}
\newcommand{\sanjida}[1]{\textcolor{black}{#1}}
\newcommand{\new}[1]{\textcolor{black}{#1}}
\newcommand{\newtwo}[1]{\textcolor{black}{#1}}
\newcommand{\newthree}[1]{\textcolor{black}{#1}}
\newcommand{\wip}{{}}
\newcommand{\commentRelatedwork}[1]{\textcolor{black}{#1}}

\newcommand{\mycomment}[1]{}

% https://www.overleaf.com/learn/latex/Environments
% White rounded frame
% \newenvironment{summarybox}
% {\noindent\begin{minipage}{\linewidth}
% \vspace{2pt}
% \begin{mdframed}[roundcorner=10pt]}%
% {\end{mdframed}
% \vspace{2pt}
% \end{minipage}}

% White frame
% \newenvironment{summarybox}
% {\noindent\begin{minipage}{\linewidth}
% \begin{mdframed}}%
% {\end{mdframed}
% \end{minipage}}

% Slim frame
\newenvironment{summarybox}
{\begin{tcolorbox}[boxsep=0pt]}%
{\end{tcolorbox}}

% Slim frame, breakable
% \newenvironment{summarybox}
% {\begin{tcolorbox}[enhanced jigsaw,boxsep=0pt,breakable,pad at break=1mm, break at=-\baselineskip/0pt]}%
% {\end{tcolorbox}}

% No frame
% \newenvironment{summarybox}
% {}%
% {}

% Gray
% \newenvironment{summarybox}%
% {\noindent\rule{\linewidth}{0.4pt}}%
% {\rule{\linewidth}{0.4pt}}

% https://www.natolambert.com/writing/grad-students-graphic-design
% \usepackage[dvipsnames]{xcolor}
\newcommand{\cblock}[3]{
 \hspace{-1.5mm}
 \begin{tikzpicture}
   [
   node/.style={square, minimum size=10mm, thick, line width=0pt},
   ]
   \node[fill={rgb,255:red,#1;green,#2;blue,#3}] () [] {};
 \end{tikzpicture}%
}
% https://tex.stackexchange.com/a/280736
\captionsetup{labelfont=sc,labelsep=period}
\definecolor{mygray}{RGB}{53,56,57}
\DeclareRobustCommand\sampleline[1]{%
  \tikz\draw[#1,dashed,mygray,line width=1.3pt,dash pattern=on 3pt off 1pt] (0,0) (0,\the\dimexpr\fontdimen22\textfont2\relax)
  -- (1.7em,\the\dimexpr\fontdimen22\textfont2\relax);%
}
% \definecolor{mygray}{RGB}{255,0,0}
% \DeclareRobustCommand\colorline[1]{%
%   \tikz\draw[#1,dashed,mygray,line width=1.3pt,dash pattern=on 3pt off 1pt] (0,0) (0,\the\dimexpr\fontdimen22\textfont2\relax)
%   -- (1.7em,\the\dimexpr\fontdimen22\textfont2\relax);%
% }
\newcommand{\cex}[3]{\tikz[baseline]{\definecolor{mycolor}{RGB}{#1,#2,#3};\draw[line width=2.5pt, color=mycolor] (-0.1,0) -- (0.1,0.2) (-0.1,0.2) -- (0.1,0);}}
\newcommand{\cplus}[3]{\tikz[baseline]{\definecolor{mycolor}{RGB}{#1,#2,#3};\draw[line width=2.25pt, color=mycolor] (-0.125,0.125) -- (0.125,0.125) (0,0) -- (0,0.25);}}
\newcommand{\ccircle}[3]{\tikz[baseline]{\definecolor{mycolor}{RGB}{#1,#2,#3};\draw[line width=2.5pt, color=mycolor, fill=mycolor] (0,0.1) circle (0.09);}}
\newcommand{\cbox}[3]{\tikz[baseline]{\definecolor{mycolor}{RGB}{#1,#2,#3};\draw[line width=1.5pt, color=mycolor] (0,0) rectangle ++(0.2,0.2);
% \draw[line width=1pt, color=mycolor] (0,0.1) -- (0.2,0.1);
}}
\newcommand{\cboxfill}[6]{\tikz[baseline]{\definecolor{mycolor}{RGB}{#1,#2,#3}; \definecolor{mycolor2}{RGB}{#4,#5,#6}; \draw[line width=1.5pt, color=mycolor, fill=mycolor2] (0,0) rectangle ++(0.2,0.2);
% \draw[line width=1pt, color=mycolor] (0,0.1) -- (0.2,0.1);
}}
\newcommand{\colorline}[3]{\raisebox{3pt}{\tikz{\definecolor{mycolor}{RGB}{#1,#2,#3}; \draw[mycolor, line width=0.5mm] (0,0) -- (0.5,0);}}}
% \DeclareRobustCommand\colorline[3]{%
%   \tikz{\definecolor{mycolor}{RGB}{#1,#2,#3};\draw[#1,dashed,color=mycolor,line width=1.3pt,dash pattern=on 3pt off 1pt] (0,0) (0,\the\dimexpr\fontdimen22\textfont2\relax)
%   -- (1.7em,\the\dimexpr\fontdimen22\textfont2\relax);%}
% }

% % https://claude.ai/chat/6e8e4b6c-2e9c-474b-81df-098eaae31088
% \newcounter{codectr}
% % \renewcommand{\thefigure}{\arabic{figure}}
% \newcommand{\setcodecaption}{%
%     % \addtocounter{codectr}{1}%
%     \stepcounter{codectr}% 
%     \renewcommand{\thefigure}{\textsc{Listing \arabic{codectr}}}%
% }
% \newcommand{\setfigurecaption}{%
%     \renewcommand{\thefigure}{\arabic{figure}}%
% }

\usepackage{lipsum}


==> _OldVersion.ICSE25/old-sections/application.tex <==
\mycomment{
%future work
\section{Application: other Reasoning Benchmarks}
Share commonality across other benchmarks:
Applied what we learned to other similar reasoning benchmarks
}

\section{Error Analysis and LLM Reasoning Capabilities}

Why fail?

Remember it or reasoning: old data in the Internet, new data compare with similar level of difficult
\begin{itemize}
\item feed wrong labels to see which results LLM predict -- does LLM remember or reason
\item can LLM get correct output when intemediate steps are wrong?
\end{itemize}

Robustness whether the model memorizes or uses the spurious features (not causal)

Chain of thoughts/explanations to understand which steps are difficult 

What capabilities LLM is lacking for reasoning about vulnerabilities? 

\mycomment{
%future work
\subsection{How to use LLM effectively: fine-tune or prompt}

\wei{Rasel and Roy}: novel fine-tuning

e.g., contrastive pairs 

Purpose:
\begin{itemize}
\item compare the effectiveness of fine-tune vs prompt
\item test the limit of current LLM 
\end{itemize}
}

\subsection{Patterns in error prediction: error analysis}

Hypothesize some error patterns based on the inital probe and confirm it 

Is there a particular type(s) more difficult to detect?

Collect examples that none of the models can predict correctly? 

What examples that none of the models can predict correctly?

\begin{itemize}
\item keyword "buggy" in NLP motivated LLM predict vulnerable all the time
\item always predict "buffer overflow"
\item cannot confirm non-vulnerable 
\end{itemize}

\section{LLMs Races Human for Vulnerability Detection Task}

Design the best approach for LLMs (like ensemble) to compare with human capabilities 

DBGBench (study methods): 



==> _OldVersion.ICSE25/old-sections/findings-early.tex <==
\textcolor{red}{EARLY NOTES BELOW}
\begin{itemize}
\item how sensitive is the format of prompt?
\end{itemize}


Survey the existing prompt methods
- Retrieval + LLM 
- Use CVE description in the prompt
- Contrasting: commits 

balanced labels, randomness for last examples

Chain of thoughts: 
- you can put together a paragraph
- interactively in chatgpt

automatically generate the need axilary information 

Prompt, generate responses with tool use 

Bug report with detailed explanations as chain of thoughts, stack traces 

Tool formers 

Inline the slice of PDG (from PVS)/CFG with code

Trace with random test input 

Propose new prompts 

Ensemble models:  scheduling or results, can we also select a fine-tune model

- soft consists 



Hypothesize some successful approach and confirm it. \benjamin{Get thoughts or ideas after completing the initial probe.}

\benjamin{Some resources on this topic:
\begin{itemize}
    \item Pretrain, prompt, and predict~\cite{train_2021}
    \item A Survey of Large Language Models~\cite{zhao_survey_2023}
    \item Lilian Weng's writeup on Prompt Engineering~\url{https://lilianweng.github.io/posts/2023-03-15-prompt-engineering/}
\end{itemize}
}

Proposed prompting approaches, ordered roughly from easy to difficult:

\begin{itemize}
    \item In-context learning with few-shot examples

        \textbf{Rationale}: The authors of the GPT-3 and GPT-2 papers~\cite{brown_language_2020,radford_language_2019} showed that providing a few exemplars in the prompt to a model can condition it to perform a task in an unsupervised fashion.
        Few-shot examples can be used for the goal of formatting the model's output or making the model ``think'' in intermediate steps ~\cite{zhao_survey_2023}.
        We will provide few-shot examples for vulnerability detection in order to condition the model to provide output in the format we desire.
        
        \textbf{Prior work}:
        Li et al.~\cite{li2023hitchhikers} used few-shot demonstrations to teach LLMs how to extract post-constraints that lead to the use of suspicious variables from the caller of a function.
        
        \textbf{Design}:
        There is much variation in the design, and therefore much experimentation is needed. All follow the same procedure: design a format of prompt/completion which the model should follow and show $n$ examples in this format derived from ground-truth labels. Some concrete designs:

        \begin{enumerate}
            \item \textbf{Simple}: prompt concatenated to completion. Given a fixed context length, the ``best'' examples can be chosen using several methods:
            \begin{itemize}
                \item Random sampling
                \item Random sampling stratified by labels
                \item Same project
                \item Semantically similar examples. We can measure this by vector similarity using KNN, CodeBERT embedding, OpenAI embedding, etc.
            \end{itemize}
            
            \item \textbf{CVE exemplar}: Use CVE descriptions as natural-language explanations for vulnerable examples. The model will attempt to generate a similar natural-language explanation for new vulnerabilities.
            This is motivated because the CVE is an actual explanation, sometimes step-by-step walking through the vulnerability.
            \begin{itemize}
                \item Take the CVE description from the CVE database (e.g. \url{https://www.cve.org/CVERecord?id=CVE-2017-11462}). Format the example as \textit{Prompt} + \textit{CVE description} + \textit{``Therefore, the example is vulnerable''}.
                \item In order to balance the labels, an equal number of non-vulnerable examples should be included with valid explanations, which can be generated by having the model (1) summarize the function's behavior without detecting vulnerabilities or (2) given the CVE description and the fixed version of the code, explain why the fix worked.
            \end{itemize}
            
            \item \textbf{Contrasting pairs}: Give positive and negative pairs of examples based on buggy/fixed versions from vulnerability datasets.
        \end{enumerate}

        The design must keep in mind some biases which have been identified, e.g.~\cite{zhao_calibrate_2021}:
        \begin{itemize}
            \item \textbf{Majority label bias}: the model tends to copy the majority label.
            \item \textbf{Recency bias}: the model tends to copy the latter examples.
            \item \textbf{Common token bias}: the model tends to generate tokens which are common in the prompt.
        \end{itemize}
    
    \item Chain of thoughts

        \textbf{Rationale}: LLMs have been shown to perform better on some tasks when they are prompted to use Chains of Thought (CoT)~\cite{wei_chain--thought_2023,kojima_large_2023}: series of intermediate reasoning steps, rather than immediately outputting the answer.
        
        \textbf{Prior work}: All prior works use basic versions of Chain-of-Thought which do not reveal the intermediate reasoning steps of vulnerability detection; our approach should surpass this basic implementation by forcing the model to reason through the steps similar to a proof output by a static analyzer.
        Li et al.~\cite{li2023hitchhikers} used ``simple CoT'' -- in other words, end the prompt with ``Let's think step-by-step''.
        Zhang et al.~\cite{zhang2023prompt} prompted the model to describe the program's intent, then predict whether it is vulnerable.
        David et al.~\cite{davidYouStillNeed2023} prompted the model to evaluate each function in a program individually.
    
        \textbf{Design}: Some candidate designs:
        \begin{enumerate}
            \item \textbf{Derive CoT from static analyzer trace}: Use static analyzer proofs to prompt the model to use chains of thought.
            Take the buggy traces from the D2A dataset; each example is a vulnerable program with $n$ trace steps. Transform each example into a ``trace-derived chain of thought''; list the code, then list the trace steps in plain English. Augment each example in a few-shot prompt with these CoT.
            \item \textbf{Zero-Shot CoT + self-consistency}: We can use an improved version of Zero-shot CoT compared to ~\cite{li2023hitchhikers}; generate exemplars of chains of thought using ``Let's think step-by-step'', filter exemplars to those which are correct and where the steps are consistent with the answer (by majority vote or by post-hoc evaluation by the LLM), and use them for in-context learning.
        \end{enumerate}

        We can also incorporate self-consistency -- see CoT-SC.
        
    \item Prompt augmentation with auxiliary information (static information, dynamic information)

        \textbf{Rationale}: The code inside is missing information which is used in compiler and static analysis, and may be difficult for the model to infer. We propose to augment the code in the prompt with static information in order to give more complete information for the model to make a decision.

        \textbf{Prior work}:
        Zhang et al. \cite{zhang2023prompt} enhanced prompts by appending text versions of AST, CFG, and PDG.

        \textbf{Design}: \cite{zhang2023prompt} has introduced the basic technique and shown that it has mixed results. We could improve on it by:
        \begin{itemize}
            \item Appending a subset of the ``most useful'' information, rather than the entire AST/CFG/PDG.
            \item Inserting the AST/CFG/PDG information inline rather than in a block separate from the text. E.g. by inserting a comment \texttt{if (x) // x depends on a, b, c}.
            \item Inserting additional static or dynamic information. Brainstorm: what information could be useful?
        \end{itemize}
        
    \item Program transformation using slicing

        \textbf{Rationale}: LLM have limited context length, so full programs might not fit inside the program. Also, . We propose to transform programs into slices of important variables in order to reduce their length and focus on the important code. 

        \textbf{Prior work}: No prior work known

        \textbf{Design}: Use a static slicing tool to reduce the program to the lines related to some set of important variables. Open question: how to decide which variables are important?

    \item Tool use
    
        \textbf{Rationale}: LLMs can struggle with basic functionality or functionality can be unavailable in a basic prompt. In ToolFormer, Schick et al.~\cite{schick_toolformer_2023} provide \textit{tools} to an LLM, which the model can access via APIs.
        
        \textbf{Prior work}: Li et al.~\cite{li2023hitchhikers} allow an LLM to access the body of a function by including a tool invocation in its output, e.g. \texttt{[{"type": "function\_def", "name": "foo"}]}. For each tool invocation, they provide the code inside the body of the function; this way, the model can request more context for the functions which are important/useful in reasoning about the program.

        \textbf{Design}: Provide API calls which the model can use to perform better on vulnerability detection and avoid ``I don't know'' responses. Li et al. have provided a basic API with one tool; our approach should surpass theirs by providing more in-depth tools, or tools to provide functionality which the model struggles to accurately fulfill by itself, such as static analysis.
        Tools could include:
        \begin{itemize}
            \item retrieve function body
            \item generate slice of function
            \item check control/data dependency
            \item alias analysis, value range analysis (many static analyses may be available off-the-shelf in LLVM or Joern)...
        For each tool, implement the tool using off-the-shelf static  analysis and either prompt or fine-tune the model to include API calls in its responses where appropriate as in ToolFormer.
        \end{itemize}

        We can also incorporate techniques for blending reasoning + acting -- see ReAct.
\end{itemize}

Try our new prompt methods

Baseline prompting
\benjamin{These are listed in the \textbf{Prior work} sections above and in a bullet list in the Related Work section.}

Baseline approaches:

\begin{itemize}
    \item \cite{li2023hitchhikers}:
    \begin{itemize}
        \item Few-shot examples
        \item Tool use
        \item Self-consistency
        \item Zero-shot CoT
        \item Model's understanding of loops, concurrency, and unfamiliar functions.
    \end{itemize}
    \item \cite{zhang2023prompt}:
    \begin{itemize}
        \item Basic prompting
        \item Augment with AST, CFG, PDG
        \item Chain-of-thought (but not a faithful implementation).
    \end{itemize}
    \item \cite{davidYouStillNeed2023}:
    \item \cite{maScopeChatGPTSoftware2023}:
    \begin{itemize}
        \item Model's understanding of CFG, call graph, PDG, taint analysis, pointer analysis, robustness
    \end{itemize}
\end{itemize}

\begin{itemize}
\item examples before NLP descriptions work better for predicting vulnerabilities 
\item order, token
\end{itemize}


==> _OldVersion.ICSE25/old-sections/performance-eval__old_.tex <==
% \newpage

\section{The Capabilities of LLMs for Detecting Software Vulnerabilities}

% \wei{more models, 1000 data points, synthetic data, sensitivity of the prompt}

\subsection{Prompting methods}

We've developed the following methods for generating prompts.
These prompt templates are meant to improve the model's performance by influencing its completions towards a specific format, disambiguating the query, or giving examples for in-context learning.
Some templates can be combined, such as ``CWE list'' + ``Q/A'' + ``$n$-shot with CodeBERT embeddings''.
Appendix \ref{sec:prompt-examples} lists examples of the prompts and more details.

\lstset{
basicstyle=\small\ttfamily,
columns=flexible,
breaklines=true,
breakatwhitespace=false,
% postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
escapeinside={<@}{@>},
rulecolor=\color{black},
frame=single,
}
\newcommand{\KeywordColor}{gray}
\newcommand{\HintColor}{RoyalBlue}
\newcommand{\CompletionColor}{ForestGreen}

% \begin{table*}[]
%     \centering
%     \caption{Variations of zero-shot prompting.}
%     Prompt template:\\
%     \texttt{Query \\ Code \\ \textcolor{green}{Hint} \\ Model completion}\\
%     \begin{tabular}{c|c|c|c}
%         Basic & Q/A & CWE List & Single-type analysis \\
%         Is the following code vulnerable, Yes or No?. & & & &
%     \end{tabular}
%     \label{tab:zero-shot}
% \end{table*}

The prompting methods:

% \todo[inline]{TODO: Add more details and emphasize our methods}

\begin{itemize}
    \item \textbf{Zero-shot prompting}: In these prompt templates, we prompt the model without giving examples for in-context learning.
    The prompt can be manipulated to disambiguate the request or improve the model's generations.
    % ``Let's think step-by-step'', Q/A, CWE list, system prompt, single-type analysis.

    % Several transformations can be applied to the query given to the model, which direct its completions and can improve the performance without the need for training or in-context learning.

    \begin{itemize}
        \item Basic query: ``Is the following function buggy? Please answer Yes or No.''
        \item System prompt: Give the model a system prompt to set the context of the model's outputs: ``I want you to act as a vulnerability detection system.''
        \item CWE list: Provide a list of bug types and, rather than asking if the function is ``buggy'', ask ``Does the following function contain \textbf{one of the following bug types}?''
        \item Q/A: Condition the model to work in a question-answering context by providing the marker tokens ``Question:'' before the question and ``Answer:'' before the model's answer.
    \end{itemize}
    
    \item \textbf{$n$-shot prompting}: In these prompt templates, we provide several examples for in-context learning~\citep{gpt3}, selected from some dataset of functions labeled as vulnerable or non-vulnerable. For vulnerable examples, we give the example response ``Yes, the function is buggy''; for non-vulnerable examples, we give the response ``No, the function is not buggy''. The in-context examples condition the model to reply in the same format as the example responses. More details are discussed in the Appendix.
    
    % Following \citet{gpt3}, the model's response is conditioned on a set of $n$ ``good examples'' of queries and responses, then we give the unseen code and sample the model's completion. The model should follow the same behavior as the examples, and it can even learn from the in-context examples.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{Images/performance.png}
    \caption{Performance of each prompting method.}
    \label{fig:performance}
\end{figure*}

    \item \textbf{Similarity search}: In these prompt templates, we choose the in-context examples by looking up labeled source code examples which are similar to the code in the query, rather than choosing randomly~\citep{rag}. This can provide the model with examples which are relevant to the query, or provide examples of correct predictions in the same conditions and structures where a bug could manifest.
    
    There are many methods available to determine the ``similar'' examples; we used vector similarity scores measured using neural network embeddings like SentenceTransformers, CodeBERT, and OpenAI embeddings.
    % In-context examples can be chosen by selecting randomly from the dataset, or similarity search using SentenceTransformers embedding, CodeBERT embedding, or OpenAI Babbage embedding~\cite{rag}.
    
    \item \textbf{Contrasting pairs}: In these prompt templates, we provide in-context examples consisting of buggy code and its corresponding fix. These are available because the SVEN dataset is constructed from bug-fixing commits; we can take the version before the commit as the buggy version and the version after the commit as the fixed version.
    Since these two versions of the source code differ primarily in the portion related to the bug-fix (excluding any extraneous changes), the small differences highlight the cause of the bug.

    \item \textbf{Chain-of-Thought (CoT) from CVE descriptions}: In these prompt templates, we provide the model with responses which include a ``chain-of-thought'' -- intermediate reasoning steps which lead to the answer, inspired by \citet{cot}.
    \begin{itemize}
        \item For vulnerable examples, we obtained natural-language reasoning steps by adapting the descriptions annotated by CVE bug reports. These descriptions describe how the bug manifests.
        \item For non-vulnerable examples, we used the commit messages of bug-fixing commits, which are annotated in the dataset. These messages explain what the bug was and how it was fixed.
    \end{itemize}
    These extra metadata are annotated in the Big-Vul dataset~\citep{bigvul}.
    We condition the model on several pairs of queries and our constructed chain-of-thought responses, causing the model to generate completions in the same format.

    % The bgp_attr_unknown function in bgp_attr.c in Quagga 0.99.21 does not properly initialize the total variable, which allows remote attackers to cause a denial of service (bgpd crash) via a crafted BGP update.
    
    % The examples from the BigVul~\citep{bigvul} dataset are annotated with natural-language descriptions which are filed with the CVE report. These descriptions explain how and where the bug manifests.
    % We propose to adapt the descriptions as an example of reasoning through the bug and prompt the model using a chain-of-thought template so that it follows the same process.

    % We will use in-context learning to make the model generate a chain-of-thought. The model will be conditioned on several pairs of source code and our constructed responses (in \textcolor{\HintColor}{blue}) with chain-of-thought reasoning, then will make a prediction for the unseen source code. Because its behavior is conditioned the examples, the model should follow our constructed responses.

% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{Images/performance-by-model.png}
%     \caption{Performance of the prompting methods grouped by model.}
%     \label{fig:prompting-by-model}
% \end{figure*}
    

    
    \item \textbf{Chain-of-Thought from Static Analysis}: In these prompt templates, we provide chains of thought derived from error traces reported by static analysis tools.
    
    Many static analyzers list as evidence for an alert \textit{error traces} -- lists of locations in the code along with conditions at each location which imply the bug.
    % The traces are a minimal set of reasoning steps provided ``for free'' when the analyzer is run.
    Many analyzers are expensive to run, but we can use examples from the D2A dataset~\citep{d2a}, which lists thousands of traces from several open-source C++ projects.
    We condition the model on several pairs of queries and chains of thought constructed from static analyzer traces.
    % We propose to convert these error traces to natural-language reasoning steps and prompt the model using a chain-of-thought template so that it will emulate the same reasoning process.
    
    % \item \todo[inline]{Implemented ideas above; future ideas are listed below}
    % \item Tool use:
    % \begin{itemize}
    %     \item Retrieve definition of function
    %     \item Retrieve similar code
    %     \item Check control/data dependency, perform alias or value analysis
    % \end{itemize}
    % \item Ensemble multiple prompts or models

    \item \textbf{Chain-of-Thought from Conversations}: In these prompt templates, we interact with the model in a conversation to query its reasoning about the bug.

    We implemented a human-in-the-loop prototype of this approach for null-pointer dereference bugs, by asking the following questions in a single session:

    \begin{itemize}
        % \item \textbf{Q1}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
        % \item After the initial query, we ask follow-up questions to question the model's reasoning:
        \item \textbf{R1}: \textit{At which line, the pointer can be a NULL?}
        \item \textbf{R2}: \textit{Which pointer can be a NULL?}
        \item \textbf{R3}: \textit{At which lines the pointer is dereferenced?}
        \item \textbf{R4}: \textit{Can a NULL pointer `X' be dereferenced?} (where `X' is a placeholder for the variable which can potentially be a NULL pointer)
        % \item After reasoning about the bug, we query the model again about the vulnerability:
        \item \textbf{Q}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
    \end{itemize}

    The \textbf{Q} (for Query) question asks the model for a prediction about the bug.
    The \textbf{R} (for Reasoning) questions force the model to reason about the root causes of the bug.
    
    As our prototype requires a human to reason about the answers to the intermediate questions, it is difficult to scale. We plan to automate this prompt technique or provide the model with examples of the manually-crafted conversations to condition its response to reason about the bug in a similar way before predicting an answer.
\end{itemize}

\subsection{Vulnerability detection capabilities}

We ran experiments to answer the following research questions:
\begin{itemize}
    \item What are the most successful and unsuccessful prompt designs for vulnerability detection?
    \item How well can state-of-the-art LLMs perform on vulnerability detection?
    \item Can the model reason about root causes of vulnerabilities in a conversational setting? Furthermore, does this improve the model's predictions?
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{Images/performance-by-model-vertical.png}
    % \includegraphics[width=\linewidth]{Images/performance-by-model-horizontal.png}
    \caption{Performance of the prompting methods for each model.}
    \label{fig:prompting-by-model}
\end{figure}

\paragraph{Results: prompting methods}
Figure \ref{fig:performance} shows the performance of all prompting methods for each model. Chain-of-thought prompt templates (CoT-CVE and CoT-SA) all performed worse than 0-shot prompts, which is the most basic baseline prompt; on the other hand, some 6-shot prompts performed better, especially using CodeBERT and contrasting pairs to select the examples.

The best approach for LLAMA and StarChat-$\beta$ (6-shot CodeBERT and contrasting pairs) did not perform well on WizardCoder or GPT-3.5; WizardCoder also performed relatively poorly using CoT-SA and Cot-CVE, and other $n$-shot prompt templates, suggesting that this model was not able to perform in-context learning as well as the other two models.

Figure \ref{fig:prompting-by-model} compares the performance of each prompting method for each model. On WizardCoder and StarChat-$\beta$, CoT approaches ranked among the lowest-performing approaches and often performed worse than their baselines, indicating that these more advanced approaches were not helpful in their current implementation, though they may improve if they are adjusted manually.

For all the models, the 0-shot prompting method performed about as well as a hypothetical baseline which randomly selects ``vulnerable'' or ``non-vulnerable'' (since the classes are balanced, we expect $Accuracy_{Mean}=0.5$).

\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:} The best-performing prompting methods were 6-shot prompts with either random selection or selection by CodeBERT retrieval + contrasting pairs.
\end{mdframed}

% CodeBERT embeddings + contrasting pairs performed the best for Code LLAMA and StarChat-$\beta$, while CodeBERT embeddings performed relatively poorly compared to random selection for WizardCoder.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{Images/model-performance.png}
    \caption{Best-case performance for each model.}
    \label{fig:best-model}
\end{figure}


\paragraph{Results: model performance}
Figure \ref{fig:best-model} compares the best-performing prompting methods for each model.
StarChat-$\beta$ outperformed CodeLLAMA, WizardCoder, and GPT-3.5, though these results reverse the models' performance on code generation $Pass@1$, shown in Table \ref{tab:humaneval}.
Additionally, all of the models performed at best slightly better than a random-selection baseline of $Accuracy_{Mean}=0.5$ (StarChat-$\beta$ earned 0.54 $Accuracy_{Mean}$).
Furthermore, WizardCoder earned less than 0.5 $Accuracy_{Mean}$ on average using its best setting.
These results suggest that the models' adequate vulnerability detection performance is not guaranteed by high code generation performance, though the models may be further improved by introducing better prompting methods or fine-tuning.
We propose as a next step to deeply investigate the predictions of these models to understand why they performed so badly.

\begin{minipage}{\linewidth}
\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:} The best-performing models were StarChat-$\beta$ followed by Code LLAMA.
The best performance was only slightly above the random-guess baseline of 0.5 $Accuracy_{Mean}$.%
\end{mdframed}
\end{minipage}


\begin{table}[t]
\centering
\caption{Code generation results on HumanEval, as reported by {\url{https://paperswithcode.com/sota/code-generation-on-humaneval}}}
\label{tab:humaneval}
\begin{tabular}{lcrrr}
\toprule
       &             & \multicolumn{3}{c}{$Pass@k$}              \\ \cmidrule{3-5}
Model       & Parameters            & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10}               & \multicolumn{1}{c}{100}              \\
\midrule
GPT-4       & \multicolumn{1}{c}{-} & 86.6   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
WizardCoder & 15B                   & 57.3   & 73.3                 & 90.5                 \\
Code LLAMA  & 34B                   & 48.8   & 76.8                  & 93                    \\
GPT-3.5     & \multicolumn{1}{c}{-} & 48.1   & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
StarCoderBase\footnotemark & 15B &	30.4 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
\bottomrule
\end{tabular}
\end{table}
\footnotetext{(base model of StarChat-$\beta$) \url{https://huggingface.co/blog/starcoder}}

\begin{figure}[htbp]
    \centering
    % \includegraphics[width=0.5\textwidth]{Images/example-shots.png}
    \includegraphics[width=0.8\linewidth]{Images/plot-shots-llama.png}
    \includegraphics[width=0.8\linewidth]{Images/plot-shots-starchat.png}
    \includegraphics[width=0.8\linewidth]{Images/plot-shots-wizardcoder.png}
    \caption{Performance of 0 to 6 in-context examples.
    % \todo[inline]{WIP: waiting on the results of random strategy and other models}
    }
    \label{fig:shots}
\end{figure}

\paragraph{Results: $n$-shot prompting}
Figure \ref{fig:shots} displays the performance of the $n$-shot random and CoT strategies with 1, 2, \ldots, up to 6 examples in the prompt.
We did not try more than 6 examples yet because more examples can exceed the context limit of some of the models.

Considering Code LLAMA, for the $n$-shot random approach, the optimal number of examples was 3 rather than 6. We consistently used 6 examples when comparing with different approaches, but note that future evaluations may tune this parameter.
For both CoT approaches, the model's mean performance drops below the baseline of 0.5 $Accuracy_{Mean}$ when we use 3-5 examples, but increases above the 0-, 1-, and 2-shot performance when we use 6 examples.
StarChat-$\beta$ and WizardCoder had similar performance characteristics, though the \textit{random} strategy peaked at 5 examples for StarChat-$\beta$ and 2 examples for WizardCoder. StarChat also improved rather consistently as more examples were added, though CoT underperformed compared to 0-shot.

These results indicate that more examples were not always better, but can improve the model if enough examples are given. The CoT approaches performed worse than the 0-shot baseline; however, their performance may be improved by using more than 6 examples.
We believe the cause of the improvement may be because the model's behavior is highly dependent on the examples, and a small set of examples may produce highly biased behavior or may not be informative to the model.
%Therefore, we used 6 examples when comparing our few-shot prompting approaches with other

\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:} The optimal number of in-context examples varied depending on the model and prompting method.
CoT prompting always performed worse than 0-shot.
\end{mdframed}

\begin{figure}[htbp]
    \centering
    \caption{Reasoning queries}
    \begin{mdframed}[roundcorner=10pt]
        \label{fig:reasoning-queries}
        \begin{itemize}
            % \item \textbf{Q1/Q2}: \textit{Does this program contain any vulnerabilities? Please answer ``Yes'' or ``No''.}
            \item \textbf{R1}: \textit{At which line, the pointer can be a NULL?}
            \item \textbf{R2}: \textit{Which pointer can be a NULL?}
            \item \textbf{R3}: \textit{At which lines the pointer is dereferenced?}
            \item \textbf{R4}: \textit{Can a NULL pointer `X' be dereferenced?}
        \end{itemize}
    \end{mdframed}
\end{figure}

% \begin{table*}[htbp]
% \centering
% \caption{Model performance with and without reasoning.}
% \begin{tabular}{lrrrrrrr}
% \toprule
%        &    & \multicolumn{4}{c}{Reasoning queries} &  \\ \cmidrule{3-6}
% Model       & No reasoning & R1 & R2 & R3 & R4 & \makecell[r]{Reasoning\\without corrections} & \makecell[r]{Reasoning\\with corrections} \\
% \midrule
% GPT-3.5     & 5  & 4  & 5  & 7  & 10 & \textbf{9} & \textbf{11}  \\
% Code LLAMA  & 8  & 2  & 2  & 6  & 6  & \textbf{10} & 6 \\
% WizardCoder & 6  & 5  & 5  & 8  & 6  & 3 & \textbf{8}  \\
% \midrule
% Total & 12  & 12  & 12  & 12  & 12  & 12 & 12 \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[htbp]
    \centering    
    
\caption{Without reasoning questions/answers: total 12 examples (6 vul and 6 nonvul)}
\label{tab:reasoning}
\begin{tabular}{lrrrrrr}
\toprule
Model       & Correct \\
\midrule
GPT-3.5     & 5 \\
Code LLAMA  & 8 \\
WizardCoder & 6 \\
% \midrule
% Total & 12 \\
\bottomrule
\end{tabular}

\begin{minipage}{0.5\linewidth}
\caption{Model reasoning without corrections.}
\label{tab:reasoning}
\begin{tabular}{lrrrrrr}
\toprule
       & \multicolumn{4}{c}{Reasoning queries} &  \\ \cmidrule{2-5}
Model       & R1 & R2 & R3 & R4 & \makecell[r]{Correct} \\
\midrule
GPT-3.5     &  4  & 5  & 7  & 10 & 9  \\
Code LLAMA  &  2  & 2  & 6  & 6  & 10\\
WizardCoder &  5  & 5  & 8  & 6  & 3  \\
% \midrule
% Total & 12  & 12  & 12  & 12  & 12  \\
\bottomrule
\end{tabular}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\caption{Model reasoning with corrections.}
\label{tab:reasoning-correction}
\begin{tabular}{lrrrrrr}
\toprule
            & \multicolumn{4}{c}{Reasoning queries} &  \\ \cmidrule{2-5}
Model       & R1 & R2 & R3 & R4 & \makecell[r]{Correct} \\
\midrule
GPT-3.5     & 7  & 9  & 7  & 6  & {11} \\
Code LLAMA  & 6  & 12 & 8  & 6  & 6  \\
WizardCoder & 8  & 10 & 9  & 5  & {8}  \\
% \midrule
% Total & 12  & 12  & 12  & 12  & 12  & 12  \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table*}

\paragraph{Results: Chain-of-Thought from Conversations}
We asked the models the questions from the method \textbf{Chain-of-Thought from Conversations}, in order (listed in Figure \ref{fig:reasoning-queries}).
We evaluated three models (GPT-3.5, Code LLAMA, and WizardCoder) on a small test set of 12 examples, 6 vulnerable and 6 non-vulnerable.
Table \ref{tab:reasoning} shows the results of asking the queries to the model and the effects on the models' accuracy.
Table \ref{tab:reasoning-correction} shows the same results, but after each reasoning query (R1, R2, R3, R4), if the model's answer is incorrect, the user corrects it before proceeding.

Considering Table \ref{tab:reasoning}, queries R1 and R2, all models predicted incorrectly for more than half of the programs, indicating that they are lacking in reasoning ability about detecting which pointers can be NULL.
However, all models predicted half or more of the examples correctly for R3 and R4, showing that they have better reasoning ability about whether pointers are dereferenced (generally an easier task than detecting NULL pointer assignments, since it requires only syntactic analysis rather than value-flow analysis).

Interestingly, the models sometimes predicted reasoning queries incorrectly, even when the answers are available within the conversation (Table \ref{tab:reasoning-correction}). For example, the correction to R1 implies the answer to R2, and the correction to R3 implies the answer to R4, but sometimes the models predicted R2 and R4 incorrectly. This shows that model reasoning can fail even when the answers are immediately available in the conversation.  In future work, we will more thoroughly investigate the models' reasoning capabilities

After adding reasoning to the model, 4/6 of the settings produced a greater number of correct answers (column Q2 across both tables). For GPT-3.5, the increase in correct predictions for Q2 was larger when corrections were given than without corrections.
These results indicate that forcing the model to reason in a conversational setting can potentially improve the model's vulnerability detection abilities, and that the model can perform better when it can access correct reasoning..

However, WizardCoder regressed without corrections and Code LLAMA regressed with corrections, indicating that even with correct reasoning, models can ignore the context and still predict incorrectly.

\begin{mdframed}[roundcorner=10pt]
\textbf{Summary:}
% The models failed to reason about NULL pointer values, but performed better at reasoning about pointer dereferences.
% The models sometimes failed to reason even when the answers were given in the conversation.
Reasoning queries boosted the models' accuracy in 4/6 settings.
\end{mdframed}

\paragraph{Results: Other findings}
Some other findings which we found in our experiments:

\begin{enumerate}
    \item Zero-shot prompt modifications such as Q/A can change the model's behavior substantially, even with small modifications. For example, the Q/A prompt template produced predictions which were correct for vulnerable and non-vulnerable code, while the most basic prompt nearly always predicted ``vulnerable''.
    \item Contrasting pairs performed especially well for selecting few-shot examples. We believe this may be because contrasting pairs show examples with small differences which produce a changed label, and these differences highlight the most critical regions of source code which cause the vulnerability.
    \item Model predictions can vary substantially among different random seeds, so it is important to evaluate the models multiple times when comparing different settings.
    \item The models commonly followed the chain-of-thought format when it was given. However, as shown by the reduced performance, the chains of thought did not help the model produce more correct answers. We've observed that the reasoning was often incorrect or irrelevant, and we believe that this might be the cause of lower performance.
    % \item Bigger models are not necessarily better; for example, Code LLAMA 34b performed worse than WizardCoder 15B.
    % \item Code LLAMA compared to WizardCoder-15B which outperformed Claude and CodeT5+ on code generation HumanEval but not ChatGPT-3.5, against which LLAMA should be on par
\end{enumerate}


% \todo[inline]{TODO: Add these things:%
% \begin{itemize}
% % \item What is the best prompting method?
% % \item What is the best model?
% \item COT results from sanjida?
% % \item Roy's data on the best number of few-shot examples?
% % \item A list of summary findings
% % \begin{itemize}
% %     \item Zero-shot prompt modifications such as Q/A can boost the performance substantially, for free. For example, Q/A boosted performance by XXX, ...
% %     \item Contrasting pairs performed especially well for selecting few-shot examples.
% %     \item Model predictions can vary substantially among different random seeds, so it is important to evaluate the models multiple times.
% %     \item The models commonly followed chain-of-thought examples derived from natural-language CVE descriptions and static analysis traces.
% %     \item Bigger model is not necessarily better (Code LLAMA 34b vs. WizardCoder 15B)
% %     \item Code LLAMA is newest but not the highest-performing, compared to WizardCoder-15B which outperformed Claude and CodeT5+ on code generation HumanEval but not ChatGPT-3.5, against which LLAMA should be on par
% % \end{itemize}
% \end{itemize}}


==> _OldVersion.ICSE25/old-sections/relatedwork.tex <==
\section{Related Work}

{\bf LLM studies and model studies in SE}: \wei{Sanjida}
\begin{enumerate}

 \item \textit{ \textbf{Automated Program Repair in the Era of Large Pre-trained Language Models}}:
 
Current state-of-the-art traditional and learning-based APR techniques face the problem of limited patch variety, failing to fix complicated bugs. In order to solve this issue, they directly applied LLMs (9) for APR.
 
They designed 3 different repair settings to evaluate the different ways to use LLMs to generate patches: 1) generate the entire patch function, 2) fill in a chunk of code given the prefix and suffix 3) output a single line fix.

Under this repair settings, directly application of the state-ofthe-art LLMs can outperform all existing APR techniques on all their datasets.

From their experiment, they observed that larger models tend to achieve better performance.

Besides patch generation, the LLMs consider correct patches to be more natural than other ones, and can even be leveraged for effective patch ranking or patch correctness checking.

\item \textit{ \textbf{Large Language Models are Few-shot Testers: Exploring LLM-based General Bug Reproduction}}:

This study focuses on the automation of test generation from general bug reports, In order to execute that they proposed LIBRO, a framework that uses Large Language Models (LLMs), which has been shown to be capable of performing code-related tasks. 

It can generate failure reproducing test cases for 33 of all studied cases (251 out of 750) and it can  successfully identify when the bug is reproduced by which test.


\item \textit{ \textbf{Conversational Automated Program Repair}}:

In this paper, they proposed conversational APR, a new paradigm for program repair that alternates between patch generation and validation in a conversational manner. 
In conversational APR, they iteratively build the input to the model by combining previously generated patches with validation feedback. 
They use the larger context window of Language Models (LLMs) to prevent repeating past mistakes and to integrate feedback for the model to better understand the semantic meaning of the code being tested.
By implementing this conversational APR, they were able to improve the number of correct and plausible patches for all unsupervisedly trained LLM across all model sizes.


\item \textit{ \textbf{Technical Report: Evaluation of ChatGPT Model for Vulnerability Detection}}:

In this paper, authors evaluated the performance of the ChatGPT and GPT-3 models for the task of vulnerability detection in code as these models has shown good performance on other code-based tasks, such as solving programming challenges and understanding code at a high level.

They found that the ChatGPT model performed no better than a dummy classifier for both binary and multi-label classification tasks for code vulnerability detection. 

By providing a few chain-of-thought demonstrations as epitomes in prompting, we might be able improve the models’ ability to detect vulnerabilities more accurately. 

We can explore the effectiveness of GPT-4, in addressing this task and to identify ways to enhance their performance in this specific domain.


\end{enumerate}

{\bf LLM studies in all domains}: ICML, NeurIPS, ICLR, references (archive)
\begin{enumerate}
    \item \textit { \textbf{Making Pre-trained Language Models Better Few-shot Learnerss
    Description Mappings}}: This paper  focuses on few-shot learning, a crucial aspect of natural language understanding where models need to excel with limited training data. The authors introduce a training method called "Prompt Engineering," which involves carefully crafting example-based prompts during fine-tuning to enhance model performance. Through this approach, they achieve significant improvements in few-shot learning tasks. The study highlights the importance of diverse prompts and explores different strategies to boost overall model performance. Ultimately, this research contributes to the adaptability of pre-trained language models in scenarios with minimal training data. \cite{DBLP:journals/corr/abs-2012-15723}
    \item \textit{ \textbf{Improving In-Context Few-Shot Learning via Self-Supervised Training
    Description Mappings}}: The paper  focuses on enhancing in-context few-shot learning through self-supervised training techniques. The research aims to improve the ability of models to make accurate predictions with minimal examples in a specific context. They introduce a self-supervised training approach to refine the model's understanding of context and boost its few-shot learning capabilities. The study involves experimenting with self-supervised training on various tasks and evaluating its impact on the model's performance. Ultimately, the paper provides insights into the effectiveness of self-supervised learning in improving in-context few-shot learning, which is essential for natural language understanding and related applications. \cite{chen2022improving}
    \item \textit{ \textbf{How Close is ChatGPT to Human Experts? Comparison Corpus, Evaluation, and Detection
    Description Mappings}}: This paper focuses on assessing the performance of ChatGPT in comparison to human experts. The research introduces a comparison corpus and evaluation framework to measure ChatGPT's ability to mimic human-level responses. They conduct a detailed analysis to examine the similarities and differences between ChatGPT's generated responses and those from human experts. The paper also explores techniques for detecting when ChatGPT provides answers that deviate from expert responses. Essentially, the study aims to provide insights into the gap between ChatGPT's performance and human expertise in various domains of knowledge and communication. \cite{guo2023close}
    \item \textit{ \textbf{In-Context Decision-Making from Supervised Pretraining
    Description Mappings}}: The paper focuses on the task of in-context decision-making using supervised pretraining. In this research, the authors investigate methods for improving decision-making capabilities within specific contexts. The study likely involves exploring how pretraining models with supervised data can enhance decision-making skills when applied to real-world scenarios. The paper likely discusses the methodology, experiments, and results related to in-context decision-making, ultimately contributing to advancements in reinforcement learning and decision-making systems.  \cite{lee2023incontext}
    \item \textit{ \textbf{Pretrained Language Models to Solve Graph Tasks in Natural Language
    Description Mappings}}: This paper, explores the use of pretrained language models to address graph-related tasks through natural language. In this research, the authors investigate the application of language models that have been pretrained on text data to tackle problems associated with graphs, typically requiring structured data representations. The study likely involves experiments and evaluations to assess the effectiveness of pretrained language models in solving graph-related tasks using natural language input. The paper likely discusses the methodology, findings, and potential implications of leveraging language models for graph-related problem-solving, which can have diverse applications in fields such as information retrieval, knowledge representation, and network analysis. \cite{wenkel2023pretrained}
\end{enumerate}




{\bf Vulnerability detection}: \wei{Roy} \\
\begin{enumerate}
    \item \textit{ \textbf{Not The End of Story: An Evaluation of ChatGPT-Driven Vulnerability
    Description Mappings}}: This study employs ChatGPT, a closed-source LLM model, for vulnerability mappings to CWE and ATT\&CK Techniques. ChatGPT's performance falls short compared to classical ML or DL models, possibly due to the absence of task-oriented fine-tuning, unlike fined-tuned GPT-2 which demonstrated better results. \cite{liu-etal-2023-end} 
    
    \item \textit{\textbf{Evaluation of ChatGPT Model for Vulnerability Detection}}: This study is on vulnerability detection, employing GPT-3.5(turbo, da-vinci) and ChatGPT models. The research involves experiments in two classification scenarios: binary classification (Yes/No) and multi-class classification (CWE-types/negative). In binary classification, a notable issue is a high false positive rate, whereas in multi-class classification, the LLM models exhibit a bias toward the negative class (non-vulnerable). \cite{cheshkov2023evaluation}

    \item \textit{\textbf{Prompt-Enhanced Software Vulnerability Detection Using ChatGPT}}: This project focuses on designing prompts for vulnerability detection with the assistance of ChatGPT. The enhancement process involves integrating auxilary information, such as Data Flow Graphs, Control Flow Graphs, API calls and employing a chain-of-thought approach to effectively memorize dialogues. Notably, distinct prompt strategies yielded varying results when applied to two distinct sets of C/C++ and Java vulnerability datasets. \cite{zhang2023prompt}

    \item \textit{\textbf{ Examining Zero-Shot Vulnerability Repair with Large Language Models}}: This study focuses on the limit of large language models as a buggy program repair tool. In the experiments, three types of vulnerable programs (synthetic, Hand-crafted and real-world examples) were used on both remote open-source LLMs and two local LLM models (Polycoder and gpt2-csrc). \cite{pearce2022examining}

    \item \textit{\textbf{ The Hitchhiker’s Guide to Program Analysis: A Journey with Large Language Models}}: This study addresses the enhancement of the static analysis tool UBITect, aiming to overcome inherent challenges, including knowledge limitations and exhaustive path exploration. This is achieved by leveraging Language Model Models (LLMs) due to their inherent domain knowledge recognition and code summarization capabilities. The proposed approach, known as LLift, introduces static analysis with LLM models. LLift successfully addresses design challenges associated with LLM models and demonstrates its effectiveness in identifying Use Before Initialization (UBI) bugs.\cite{li2023hitchhikers}

\benjamin{
\begin{itemize}
    \item Presentation: they have a good motivating example to step through their work.
    \item Presentation: they work from known limitations of LLMs, from previous studies or initial pilot studies, to research questions and method design.
    \item Idea: the authors allowed the model to query function bodies on-demand. We can provide the same ability as a tool to the LLM, and when the LLM points out that it has incomplete understanding of a function, it can query its code.
    \item Idea: the authors had the models generate natural-language answers, then summarize the answers as JSON. This avoids a limitation that the model may not perform well when it is asked to immediately provide JSON.
    \item This paper studies:
    \begin{itemize}
        \item Few-shot examples
        \item Tool use (on-demand context query)
		\item Multi-turn conversations with self-validation
		\item Combine LLM with static analyzer
		\item Simple chain-of-thought with "think step by step"
		\item Compare ChatGPT 3.5/4 with Claude and Bard
		\item Case study on the models' understanding of loops, concurrency, and unfamiliar functions
    \end{itemize}
\end{itemize}
}    
    
\end{enumerate}


{\bf Others} \wei{all} 

{\bf Ben}

Overall, there are several papers which study ChatGPT for vulnerability detection.
Some parts of our planned study have been looked at before, though most benchmarks are rather small so some merit may come from running on a larger dataset (on the order of 100-1000 examples).
However, several techniques/areas have not been studied yet, and most papers do not study LLMs besides ChatGPT, so there is some opportunity for us to study something useful.

Notable techniques which have been studied. Keep in mind many of the techniques are studied only in one simple implementation, so could be improved.
\begin{itemize}
    \item Simple and role-based prompts~\cite{zhangPromptEnhancedSoftwareVulnerability2023}
    \item Few-shot examples~\cite{li2023hitchhikers}
    \item Tool use (on-demant context query)~\cite{li2023hitchhikers}
    \item Multi-turn conversation~\cite{zhangPromptEnhancedSoftwareVulnerability2023,li2023hitchhikers}
    \item Chain-of-thought prompting~\cite{li2023hitchhikers,zhangPromptEnhancedSoftwareVulnerability2023,davidYouStillNeed2023a}
    \item Model's understanding of loops, concurrency, unfamiliar functions~\cite{li2023hitchhikers} and AST, CFG, PDG, call graph, pointer analysis, taint analysis, mutant detection, flaky test detection~\cite{maScopeChatGPTSoftware2023}
\end{itemize}

Comments on papers:

\begin{enumerate}
    \item Prompt-Enhanced Software Vulnerability Detection Using ChatGPT~\cite{zhangPromptEnhancedSoftwareVulnerability2023}

    In this study, the authors enhance prompts for vulnerability detection by adding AST, CFG, and Data dependency information.
    \begin{itemize}
        \item Methodology: There is room for improvement on chain-of-thought; their chain-of-thought prompting does not reason about solving the problem; it is 1. ``intent'', 2. ``classification''.
        \item Study design: They used multiple master's students to rate the explanations. I think it would be good for us to similarly quantify the quality of the explanations, but this method could be inconsistent or biased, or limited in scope due to the cost.
        
    \end{itemize}
    They studied:
    \begin{itemize}
        \item Instruct-style and Role-based prompts.
        \item Augmenting prompt with extra information from AST, CFG, Data dependency.
        \item Chain-of-thought (claimed, but I think it's incorrect/not useful).
    \end{itemize}
    
    \item Evaluation of ChatGPT Model for Vulnerability Detection~\cite{cheshkovEvaluationChatGPTModel2023a}

    In my opinion, this study is sloppy and we should not follow its example.
    For example, the main performance evaluation evaluates the ROC-AUC metric, but the model doesn't use a performance threshold - how was this calculated?
    The authors don't give enough detail about e.g. data collection or performance of different prompting methods to be useful.
    In our paper, we should be careful to avoid the mistakes by clearly explaining the rationale for our design decisions, such as data collection and prompting.
    
    \item Can Large Language Models Find And Fix Vulnerable Software?~\cite{noeverCANLARGELANGUAGE}

    The authors studied basic and role-based prompts for ChatGPT 4. They may reference some datasets which will be useful for us.

    \item Using ChatGPT as a Static Application Security Testing Tool~\cite{bakhshandehUsingChatGPTStatic2023}

\begin{itemize}
    \item Threat: Prompt context order, such as few-shot examples, can affect model performance, so they randomize it.
	\item Presentation: compare ChatGPT with SAST tools along several different dimensions to show the benefits/limitations of each approach. We can do the same, but also compare to other LLMs.
\end{itemize}

    \item When GPT Meets Program Analysis: Towards Intelligent Detection of Smart Contract Logic Vulnerabilities in GPTScan~\cite{sunWhenGPTMeets2023}

\begin{itemize}
    \item Idea: adding basic static analysis to GPT models can improve the approach. We are interested in evaluating the models' capabilities -- but could frame it as "tool use" or "consistency checking".
	\item Research question: Evaluate financial costs compared to performance of using ChatGPT.
	\item Threat: Analyze the model explanations to see why the model predicted incorrectly. This is what they did.
	\item Threat: Should mention how they get the categorical response - either they get perfect categorical responses or are leaving out important detail.
    We should just have one sentence to explain this and this will make our approach more concrete.
	\item Threat: selection bias due to any dataset filtering steps
\end{itemize}

    \item The Hitchhiker's Guide to Program Analysis: A Journey with Large Language Models~\cite{liHitchhikerGuideProgram2023}

    Comments attached to Roy's writeup.
    
    \item The Scope of ChatGPT in Software Engineering~\cite{maScopeChatGPTSoftware2023}

    The authors studied ChatGPT's understanding of syntax, static behavior (CFG, Call Graph, Data dependencies, taint and pointer analysis), and dynamic behavior (equivalent mutant detection, flaky test detection).

\begin{itemize}
    \item Presentation: break down categories of quality metrics, then analyze the reasons for all errors. See Figure 9.
    \item This paper studies:
    \begin{itemize}
        \item Control Flow Graph (CFG) generation
        \item Call Graph generation
        \item data dependency analysis
        \item taint analysis
        \item pointer analysis
        \item robustness to mutations, adversarial attacks
    \end{itemize}
\end{itemize}

    \item Do you still need a manual smart contract audit?~\cite{davidYouStillNeed2023a}

    The authors evaluated Claude and ChatGPT-4 for detecting and identifying vulnerabilities in smart contracts.

    \begin{itemize}
        \item Methodology: The authors noted several practical issues such as categorical answer and context length. We can follow their solutions where reasonable.
        \item Study design: The authors used mutation testing to test the LLMs.
        \item Study design: The authors varied parameters which are most important for generation and showed the effects.
        \item Study design: The authors studied chain-of-thought prompting.
    \end{itemize}

    \item Examining Zero-Shot Vulnerability Repair with Large Language Models~\cite{pearceExaminingZeroShotVulnerability2022}

    The authors used several, now outdated, models to fix vulnerabilities. They have a good discussion of prompt design which we can learn from and cite. Their focus is primarily on vulnerability repair, not detection.

    \item Prompting Is All You Need: Automated Android Bug Replay with Large Language Models~\cite{fengPromptingAllYou2023}

    The authors used ChatGPT to generate instructions to replay bugs on Android apps. This is different from vulnerability detection. However, we can learn from their prompt design, especially providing the model with an API, in-context learning via few-shot examples, and chain-of-thought reasoning.

%%Recent research [58, 65] demonstrates that prompting techniques have a major impact on LLM performance.






    
\end{enumerate}


==> _OldVersion.ICSE25/old-sections/threats.tex <==
\section{Threats to Validity}
Use labels as ground truth

==> _OldVersion.ICSE25/packages.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2022} with \usepackage[nohyperref]{icml2022} above.
\usepackage[hyphens]{url}
\usepackage{hyperref}
\usepackage[noabbrev,nameinlink]{cleveref}
% \usepackage[capitalise,noabbrev]{cleveref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2022}

% If accepted, instead use the following line for the camera-ready submission:https://www.overleaf.com/project/64e08ba18f21d5df8ac80186
% \usepackage[accepted]{icml2022}

% if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}

\usepackage{listings}

\usepackage{todonotes}
\usepackage{makecell}
\usepackage{footnote}
\makesavenoteenv{tabular}

\usepackage{dblfloatfix}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{multirow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}



% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage{todonotes}


\usepackage{comment}

% \usepackage[framemethod=TikZ]{mdframed}

\usepackage[numbers]{natbib}
% \usepackage[natbib=true,backend=bibtex,style=ieee,mincitenames=1,maxcitenames=2,minbibnames=3,maxbibnames=6]{biblatex}
% \usepackage{appendix}

% https://tex.stackexchange.com/a/280736
\usepackage{mathtools,tikz,caption}
\usepackage{subcaption}

% https://chat.openai.com/share/028bb52a-202b-475a-bedd-50d62e0b382d
\usepackage{adjustbox}

% https://tex.stackexchange.com/a/543
\usepackage[htt]{hyphenat}

% https://www.overleaf.com/learn/latex/Code_Highlighting_with_minted
% https://tex.stackexchange.com/a/517907
\usepackage{minted}
% \usepackage[finalizecache=true,frozencache=false,cachedir=minted-cache]{minted}
% \usepackage[frozencache=true,cachedir=minted-cache]{minted}
\usepackage[minted,most]{tcolorbox}

\usepackage{soul}

\usepackage{enumitem}

% https://texblog.org/2012/02/08/adding-line-numbers-to-documents/
% \usepackage[switch]{lineno}

% https://tex.stackexchange.com/a/163250
\usepackage{adjustbox}

% https://tex.stackexchange.com/a/3374
\usepackage{xfrac}

% Row colors
% https://tex.stackexchange.com/a/563022
\usepackage{colortbl}
% \addtolength{\extrarowheight}{\belowrulesep}
% \aboverulesep=0pt
% \belowrulesep=0pt
\usepackage[final]{pdfpages}

==> authors.tex <==

\author{\IEEEauthorblockN{Benjamin Steenhoek}
\IEEEauthorblockA{Iowa State University\\
Ames, Iowa, USA\\
benjis@iastate.edu}
\\
\IEEEauthorblockN{Mirza Sanjida Alam}
\IEEEauthorblockA{Iowa State University\\
Ames, Iowa, USA\\
sanjida@iastate.edu}
\and
\IEEEauthorblockN{Md Mahbubur Rahman}
\IEEEauthorblockA{Iowa State University\\
Ames, Iowa, USA\\
mdrahman@iastate.edu}
\\
\IEEEauthorblockN{Earl T. Barr}
\IEEEauthorblockA{University College London\\
London, UK\\
e.barr@ucl.ac.uk}
\and
\IEEEauthorblockN{Monoshi Kumar Roy}
\IEEEauthorblockA{Iowa State University\\
Ames, Iowa, USA\\
monoshi@iastate.edu}
\\
\IEEEauthorblockN{Wei Le}
\IEEEauthorblockA{Iowa State University\\
Ames, Iowa, USA\\
weile@iastate.edu}
}

==> conclusion.tex <==
\section{Conclusions}
This paper presented a thorough study of the challenges of vulnerability detection. Our results indicate that current autoregressive pretraining may not be directly useful for vulnerability detection type of problem

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> prompt-figure.tex <==

\begin{mdframed}[roundcorner=5pt,frametitle={Prompt format for queries and\\in-context examples},
% innerrightmargin=5,innerleftmargin=5
]
\begin{tinyenv}
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=30mm,center]
\centering (a) System prompt
\end{tcolorbox}
I want you to act as a vulnerability detection system.
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=30mm,center]
\centering (b) Instruction
\end{tcolorbox}
Question: Is the following function buggy? Please answer Yes or No.\\
- CWE-190: Integer Overflow\\
- CWE-XXX: \ldots\\
\texttt{<function source code>}
% \makebox[50mm]{\dotfill}

\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=40mm,center]
\centering (c) Example response\\(for in-context examples)
\end{tcolorbox}
Answer: The function contains CWE-190. Therefore, yes, the function is vulnerable.
\end{tinyenv}
\end{mdframed}
%%%%%
\begin{figure}[b]
\centering
\caption{CoT-explanation prompt which uses static analysis to provide information to the model and provides reasoning example responses to encourage reasoning.}
\label{fig:cot-explanation-prompt}\begin{mdframed}[roundcorner=5pt]
\begin{tinyenv}
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=65mm,center]
\centering (d) CoT-Explanation prompt and example response
\end{tcolorbox}
\begin{ttenv}
% Code Explanation: The pointers "['rs', 'rm', 'cmsg']" are passed as parameters in this function, which could be null.\\
% In line "struct page *page = NULL;", the pointer "page" is assigned to NULL.\\
% In lines "if (cmsg-\textgreater{}cmsg\_len \textless{} CMSG\_LEN(sizeof(struct rds\_atomic\_args)) || rm-\textgreater{}atomic.op\_active)", "rm-\textgreater{}atomic.op\_recverr = rs-\textgreater{}rs\_recverr;", the pointers "cmsg, rm, rs" are dereferenced.\\
Code Explanation: The pointer "['p']" is passed as parameters in this function, which could be null.
No pointer has been assigned to NULL in the given code.
In line "if (p-\textgreater{}lineinfo[oldpc] != 0)", the pointer "p" is dereferenced.
There is no NULL pointer check in the function.\\
\ldots\\
Reasoning: The function dereferences the pointer "p" without checking if it is NULL. If "p" is NULL, the function will crash when it tries to access the "lineinfo" field.\\
Answer: Yes, the function is buggy.

% Instructions: For the Query Function only, think step-by-step using these steps, then give an answer based on the Code Explanation. Assume pointers which are passed in will not cause a null-pointer dereference.\\
% 1. identify which locations pointers are likely to be null.\\
% 2. identify which of these are dereferenced.\\
% 3. identify which of these dereferences of potentially-null pointers are checked and handled. Filter these out.\\
% 4. if any unchecked dereferences remain, then the function is vulnerable. Otherwise, the function is not vulnerable.\\
\end{ttenv}
\end{tinyenv}
\end{mdframed}
\end{figure}
%%%%%%%
\begin{figure}
    \centering
    \caption{Prompts we evaluated.}
    \begin{mdframed}[frametitle={Basic/In-context prompts},frametitlealignment=\center]
\begin{mdframed}[frametitle={System prompt},frametitlerule=true,frametitlebackgroundcolor=yellow!70!white,roundcorner=5pt,frametitlealignment=\raggedright]
I want you to act as a vulnerability detection system.
\end{mdframed}

$n$ examples in the same format, selected with random selection or similar to the query example

\begin{mdframed}[frametitle={In-context example},frametitlerule=true,frametitlebackgroundcolor=blue!30!white,roundcorner=5pt,frametitlealignment=\raggedright]
Question: Does the following function contain one of these vulnerability types? Please answer Yes or No.

\ldots

Answer: The function contains CWE-190: Integer Overflow. Therefore, Yes, the function is vulnerable.
\end{mdframed}

\begin{mdframed}[frametitle={Query example},frametitlerule=true,frametitlebackgroundcolor=red!30!white,roundcorner=5pt,frametitlealignment=\raggedright]
Question: Does the following function contain one of these vulnerability types? Please answer Yes or No.\\
- CWE-190: Integer Overflow\\
- CWE-476: Null Pointer Dereference\\
- CWE-125: Out-of-bound Read\\
- CWE-787: Out-of-bound Write\\
- CWE-416: Use After Free

```\\
\texttt{<code>}\\
```

Answer: \texttt{<model completes>}
\end{mdframed}

    \end{mdframed}
    \caption{Prompting methods we evaluated.}
\end{figure}

%%%%%

% \begin{wrapfigure}{r}{0.6\textwidth}
\begin{figure}
\mdfsetup{frametitlealignment=\center}
\caption{CoT prompts which integrate vulnerability metadata to encourage reasoning.\label{fig:cot-prompts}}

\begin{mdframed}
% [roundcorner=5pt,frametitle={Example selection}, innerrightmargin=0,innerleftmargin=0]
[roundcorner=5pt,innerrightmargin=0,innerleftmargin=0]
\begin{tinyenv}
\centering
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=50mm,center]
\centering (a) In-context example selection
\end{tcolorbox}
\begin{tabular}{ccc}
\makecell{Random\\\cite{liuGptandIncontext2023}} & \makecell{Embedding\\\cite{zhou2024large}} & \makecell{Contrastive\\pairs}\\
\includegraphics[width=0.15\textwidth]{Images/random.png} &
\includegraphics[width=0.15\textwidth]{Images/embedding.png} &
\includegraphics[width=0.15\textwidth]{Images/diff.png}
\end{tabular}
\end{tinyenv}
\end{mdframed}
\vspace{-1.5em}
\begin{mdframed}[roundcorner=5pt]
\begin{tinyenv}
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=50mm,center]
\centering (b) CoT-CVE example response
\end{tcolorbox}
\texttt{The crypto\_skcipher\_init\_tfm function in crypto/skcipher.c in the Linux kernel through 4.11.2 relies on a setkey function that lacks a key-size check, which allows local users to cause a denial of service (NULL pointer dereference) via a crafted application. Therefore, the example is buggy.}
\end{tinyenv}
\end{mdframed}
\vspace{-1.5em}
\begin{mdframed}[roundcorner=5pt]
\begin{tinyenv}
\begin{tcolorbox}[boxsep=1pt,left=1pt,right=1pt,top=1pt,bottom=1pt,width=50mm,center]
\centering (c) CoT-SA example response
\end{tcolorbox}
\texttt{1. A buffer buf of size 10 is {allocated} at line 1.\\
2. An index i is {initialized to a value} in the range [0, 100] at line 2.\\
3. i is used to access buf at line 3. 
{This may exceed the bounds of buf.}\\
4. Therefore, the example is buggy.\\}
\end{tinyenv}
\end{mdframed}

\end{figure}

